On the Soundness of Coroutines with Snapshots

Coroutines are a general control flow construct that can eliminate control flow fragmentation inherent in event-driven programs, and are still missing in many popular languages. Coroutines with snapshots are a first-class, type-safe, stackful coroutine model, which unifies many variants of suspendable computing, and is sufficiently general to express iterators, single-assignment variables, async-await, actors, event streams, backtracking, symmetric coroutines and continuations. In this paper, we develop a formal model called $\lambda_{\rightsquigarrow}$ (lambda-squiggly) that captures the essence of type-safe, stackful, delimited coroutines with snapshots. We prove the standard progress and preservation safety properties. Finally, we show a formal transformation from the $\lambda_{\rightsquigarrow}$ calculus to the simply-typed lambda calculus with references.

==> abstract.tex <==
%!TEX root = coroutines-ecoop.tex

While event-driven programming is
a widespread model for asynchronous computing,
its inherent control flow fragmentation makes
event-driven programs notoriously difficult to understand and maintain.
\emph{Coroutines} are a general control flow construct
that can eliminate control flow fragmentation.
However, coroutines are still missing in many popular languages.
This gap is partly caused by the difficulties
of supporting suspendable computations in the language runtime.

We introduce first-class, type-safe, stackful coroutines with snapshots,
which unify many variants of suspendable computing.
Our design relies solely on the static metaprogramming support of the host language,
without modifying the language implementation or the runtime.
We also develop a formal model for type-safe, stackful and delimited coroutines,
and we prove the respective safety properties.
We show that the model is sufficiently general to express
iterators, single-assignment variables, async-await,
actors, event streams,
backtracking, symmetric coroutines and continuations.
Performance evaluations reveal that
the proposed metaprogramming-based approach has a decent performance,
with workload-dependent overheads of $1.03-2.11\times$ compared
to equivalent manually written code,
and improvements of up to $6\times$ compared to other approaches.


==> conclusion.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Conclusion}\label{sec:conclusion}

We described a programming model
for first-class typed stackful coroutines with snapshots,
along with a formalization.
Our implementation
relies on metaprogramming facilities of the host language.
We identified the critical optimizations
that need to accompany the implementation,
and showed their performance impact.
%The model achieves composability and
%generality with first-class coroutine definitions and direct nested calls.
%Composability is further strengthened through separation of yield and return types.
%We validate this by implementing a range of alternative primitives:
We identified a range of use cases
such as iterators, Async-Await, Oz-style dataflow variables,
Erlang-style actors, backtracking,
and direct-style event streams,
and we showed that they can be expressed in our model.
%Equivalence with delimited continuations is achieved
%by augmenting coroutines with the snapshot operation.
Experimental evaluation shows that our coroutine implementation
is almost as efficient as these other primitives,
and in some cases has an even better performance.

%The presented transformation technique canonicalizes the AST,
%and converts it to a control-flow graph,
%used to emit multiple entry points.

Our implementation is available online \cite{coroutines},
as an independent module that relies on metaprogramming capabilities in Scala,
and works with the official language releases.
%As a sidenote,
%this indicates a broader need for metaprogramming support
%in general-purpose languages --
%our approach requires no changes to the runtime or the language internals.
This work may indicate a wider need for metaprogramming support
in general purpose languages,
which may be easier to provide than continuation support in the runtime.
Moreover,
runtime support and JIT optimizations \cite{Prokopec:2017:MCO:3136000.3136002}
could improve the performance of our implementation even further,
and we plan to investigate this in the future.


==> evaluation.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Performance Evaluation}\label{sec:eval}

\begin{figure*}
\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  ybar=5pt,
  bar width=12pt,
  x=2.6cm,
  ymin=0,
  axis on top,
  ymax=32,
  xtick=data,
  enlarge x limits=0.24,
  symbolic x coords={TreeFindMax, TreeToArray, TreeSameFringe},
  restrict y to domain*=0:36,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=-1,
    at={(0.05, 1.45)},
    anchor=north west
  }
]
\addplot[
  fill=purple,
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (TreeFindMax, 5.81)
  (TreeToArray, 6.85)
  (TreeSameFringe, 12.54)
};
\addlegendentry{iterator}
\node[above] at ($(axis cs:TreeFindMax, 5.81)$) [xshift=-2.1*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:TreeToArray, 6.85)$) [xshift=-2.1*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:TreeSameFringe, 12.54)$) [xshift=-2.1*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[fill=black!10!white]
plot coordinates {
  (TreeFindMax, 12.24)
  (TreeToArray, 13.21)
  (TreeSameFringe, 23.91)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:TreeFindMax, 12.24)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {$2.11\times$};
\node[above] at ($(axis cs:TreeToArray, 13.21)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.93\times$};
\node[above] at ($(axis cs:TreeSameFringe, 23.91)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.91\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  postaction={
    pattern color=white,
    pattern=north east lines,
  },
]
plot coordinates {
  (TreeFindMax, 16.84)
  (TreeToArray, 17.01)
  (TreeSameFringe, 29.23)
};
\addlegendentry{continuations}
\node[above] at ($(axis cs:TreeFindMax, 16.84)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {$2.90\times$};
\node[above] at ($(axis cs:TreeToArray, 17.01)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {$2.48\times$};
\node[above] at ($(axis cs:TreeSameFringe, 29.23)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {$2.41\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,2},
  postaction={
    pattern color=white,
    pattern=crosshatch,
  },
]
plot coordinates {
  (TreeFindMax, 84.19)
  (TreeToArray, 86.47)
  (TreeSameFringe, 211.61)
};
\addlegendentry{streams}
\node[above] at ($(axis cs:TreeFindMax, 116.19)$) [xshift=2.0*\pgfkeysvalueof{/pgf/bar width},yshift=-245] {$14.49\times$};
\node[above] at ($(axis cs:TreeToArray, 119.47)$) [xshift=2.0*\pgfkeysvalueof{/pgf/bar width},yshift=-256] {$12.62\times$};
\node[above] at ($(axis cs:TreeSameFringe, 328.61)$) [xshift=2.0*\pgfkeysvalueof{/pgf/bar width},yshift=-890] {$16.82\times$};
\end{axis}
\end{tikzpicture}
\,
\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=2.1cm,
  ymin=0,
  axis on top,
  ymax=72,
  xtick=data,
  enlarge x limits=0.5,
  symbolic x coords={HashLongest, HashZip},
  restrict y to domain*=0:80,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=-1,
    at={(-0.20, 1.45)},
    anchor=north west
  }
]
\addplot[
  fill=purple,
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (HashLongest, 11.18)
  (HashZip, 63.42)
};
\addlegendentry{iterator}
\node[above] at ($(axis cs:HashLongest, 11.18)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:HashZip, 63.42)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[
  fill=black!10!white,
]
plot coordinates {
  (HashLongest, 14.09)
  (HashZip, 66.46)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:HashLongest, 14.09)$) [xshift=-0.1*\pgfkeysvalueof{/pgf/bar width}] {$1.26\times$};
\node[above] at ($(axis cs:HashZip, 66.46)$) [xshift=-0.1*\pgfkeysvalueof{/pgf/bar width}] {$1.05\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  postaction={
    pattern color=white,
    pattern=north east lines,
  },
]
plot coordinates {
  (HashLongest, 64.58)
  (HashZip, 154.28)
};
\addlegendentry{continuations}
\node[above] at ($(axis cs:HashLongest, 64.58)$) [xshift=1.4*\pgfkeysvalueof{/pgf/bar width},yshift=0] {$6.22\times$};
\node[above] at ($(axis cs:HashZip, 170.28)$) [xshift=1.4*\pgfkeysvalueof{/pgf/bar width},yshift=-123] {$2.11\times$};
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=2.1cm,
  ymin=0,
  axis on top,
  ymax=46,
  xtick=data,
  enlarge x limits=0.18,
  symbolic x coords={DFS, DenseDFS, BFS, DenseBFS},
  restrict y to domain*=0:55,
  visualization depends on=rawy\as\rawy,
  % after end axis/.code={
  %   \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  % },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=-1,
    at={(0.20, 1.45)},
    anchor=north west
  }
]
\addplot[
  fill=purple,
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (DFS, 15.21)
  (DenseDFS, 28.03)
  (BFS, 24.14)
  (DenseBFS, 42.12)
};
\addlegendentry{iterator}
\node[above] at ($(axis cs:DFS, 15.21)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:DenseDFS, 28.03)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:BFS, 24.14)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:DenseBFS, 42.12)$) [xshift=-1.8*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[fill=black!10!white]
plot coordinates {
  (DFS, 20.32)
  (DenseDFS, 30.72)
  (BFS, 28.29)
  (DenseBFS, 43.36)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:DFS, 20.32)$) [xshift=-0.2*\pgfkeysvalueof{/pgf/bar width}] {$1.34\times$};
\node[above] at ($(axis cs:DenseDFS, 30.72)$) [xshift=-0.2*\pgfkeysvalueof{/pgf/bar width}] {$1.09\times$};
\node[above] at ($(axis cs:BFS, 28.29)$) [xshift=-0.2*\pgfkeysvalueof{/pgf/bar width}] {$1.17\times$};
\node[above] at ($(axis cs:DenseBFS, 43.36)$) [xshift=0.1*\pgfkeysvalueof{/pgf/bar width}] {$1.03\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  postaction={
    pattern color=white,
    pattern=north east lines,
  },
]
plot coordinates {
  (DFS, 28.90)
  (DenseDFS, 31.50)
  (BFS, 30.96)
  (DenseBFS, 43.87)
};
\addlegendentry{continuations}
\node[above] at ($(axis cs:DFS, 28.90)$) [xshift=1.4*\pgfkeysvalueof{/pgf/bar width}] {$1.90\times$};
\node[above] at ($(axis cs:DenseDFS, 31.50)$) [xshift=1.8*\pgfkeysvalueof{/pgf/bar width}] {$1.12\times$};
\node[above] at ($(axis cs:BFS, 30.96)$) [xshift=1.8*\pgfkeysvalueof{/pgf/bar width}] {$1.28\times$};
\node[above] at ($(axis cs:DenseBFS, 44.87)$) [xshift=2.0*\pgfkeysvalueof{/pgf/bar width}] {$1.07\times$};
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=1.3cm,
  ymin=0,
  axis on top,
  ymax=13,
  xtick=data,
  enlarge x limits=0.6,
  symbolic x coords={Fibonacci, Taylor},
  restrict y to domain*=0:16,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=1,
    at={(0.00, 1.50)},
    anchor=north west
  }
]
\addplot[fill=black!10!white]
plot coordinates {
  (Fibonacci, 9.66)
  (Taylor, 1.46)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:Fibonacci, 9.66)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:Taylor, 1.46)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,2},
  postaction={
    pattern color=white,
    pattern=crosshatch,
  },
]
plot coordinates {
  (Fibonacci, 11.12)
  (Taylor, 11.53)
};
\addlegendentry{stream}
\node[above] at ($(axis cs:Fibonacci, 11.22)$) [xshift=0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.15\times$};
\node[above] at ($(axis cs:Taylor, 11.53)$) [xshift=0.8*\pgfkeysvalueof{/pgf/bar width}] {$8.37\times$};
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=1.4cm,
  ymin=0,
  axis on top,
  ymax=42,
  xtick=data,
  enlarge x limits=0.6,
  symbolic x coords={TestList, TestFract},
  restrict y to domain*=0:47,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=1,
    at={(0.00, 1.50)},
    anchor=north west
  }
]
\addplot[
  fill={rgb:red,10;green,2;blue,1},
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (TestList, 35.95)
  (TestFract, 9.83)
};
\addlegendentry{monad}
\node[above] at ($(axis cs:TestList, 35.95)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:TestFract, 9.83)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[fill=black!10!white]
plot coordinates {
  (TestList, 38.63)
  (TestFract, 13.86)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:TestList, 38.63)$) [xshift=0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.07\times$};
\node[above] at ($(axis cs:TestFract, 13.86)$) [xshift=0.8*\pgfkeysvalueof{/pgf/bar width}] {$1.41\times$};
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=2.0cm,
  ymin=0,
  axis on top,
  ymax=36,
  xtick=data,
  enlarge x limits=0.55,
  symbolic x coords={FastReq, NetReq},
  restrict y to domain*=0:40,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=-1,
    at={(0.00, 1.45)},
    anchor=north west
  }
]
\addplot[
  fill={rgb:red,10;green,2;blue,1},
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (FastReq, 11.31)
  (NetReq, 27.59)
};
\addlegendentry{async}
\node[above] at ($(axis cs:FastReq, 11.31)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:NetReq, 27.59)$) [xshift=-1.8*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[
  fill=black!10!white,
]
plot coordinates {
  (FastReq, 13.23)
  (NetReq, 27.62)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:FastReq, 13.23)$) [xshift=-0.1*\pgfkeysvalueof{/pgf/bar width}] {$1.17\times$};
\node[above] at ($(axis cs:NetReq, 27.62)$) [xshift=-0.1*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  postaction={
    pattern color=white,
    pattern=north east lines,
  },
]
plot coordinates {
  (FastReq, 427.812)
  (NetReq, 32.47)
};
\addlegendentry{threads}
\node[above] at ($(axis cs:FastReq, 427.812)$) [xshift=1.6*\pgfkeysvalueof{/pgf/bar width},yshift=-1045] {$245\times$};
\node[above] at ($(axis cs:NetReq, 32.47)$) [xshift=1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.25\times$};
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=2.0cm,
  ymin=0,
  axis on top,
  ymax=75,
  xtick=data,
  enlarge x limits=0.6,
  symbolic x coords={PC, BoundedPC},
  restrict y to domain*=0:84,
  visualization depends on=rawy\as\rawy,
  % after end axis/.code={
  %   \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  % },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=-1,
    at={(0.10, 1.45)},
    anchor=north west
  }
]
\addplot[
  fill={rgb:red,10;green,2;blue,1},
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (PC, 31.92)
  (BoundedPC, 52.03)
};
\addlegendentry{LTQ}
\node[above] at ($(axis cs:PC, 31.92)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.35\times$};
\node[above] at ($(axis cs:BoundedPC, 52.03)$) [xshift=-1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.09\times$};
\addplot[fill=black!10!white]
plot coordinates {
  (PC, 23.60)
  (BoundedPC, 47.81)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:PC, 23.60)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:BoundedPC, 47.81)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,2},
  postaction={
    pattern color=white,
    pattern=north east lines,
  },
]
plot coordinates {
  (PC, 35.83)
  (BoundedPC, 69.83)
};
\addlegendentry{future}
\node[above] at ($(axis cs:PC, 35.83)$) [xshift=1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.52\times$};
\node[above] at ($(axis cs:BoundedPC, 69.83)$) [xshift=1.6*\pgfkeysvalueof{/pgf/bar width}] {$1.46\times$};
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}[scale=0.56]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=2.7cm,
  ymin=0,
  axis on top,
  ymax=72,
  xtick=data,
  enlarge x limits=0.5,
  symbolic x coords={PingPong, ThreadRing},
  restrict y to domain*=0:80,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=2,
    at={( 0.10, 1.50)},
    anchor=north west
  },
  legend style={cells={align=left}}
]
\addplot[
  fill=purple,
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (PingPong, 40.43)
  (ThreadRing, 42.88)
};
\addlegendentry{reactor}
\node[above] at ($(axis cs:PingPong, 40.43)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\node[above] at ($(axis cs:ThreadRing, 42.88)$) [xshift=-2.4*\pgfkeysvalueof{/pgf/bar width}] {$1.21\times$};
\addplot[fill=black!10!white]
plot coordinates {
  (PingPong, 41.72)
  (ThreadRing, 48.30)
};
\addlegendentry{coroutine}
\node[above] at ($(axis cs:PingPong, 41.72)$) [xshift=-0.9*\pgfkeysvalueof{/pgf/bar width},yshift=6] {$1.03\times$};
\node[above] at ($(axis cs:ThreadRing, 48.30)$) [xshift=-0.6*\pgfkeysvalueof{/pgf/bar width}] {$1.36\times$};
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  postaction={
    pattern color=white,
    pattern=north east lines,
  },
]
plot coordinates {
  (PingPong, 58.37)
  (ThreadRing, 35.47)
};
\addlegendentry{Akka}
\node[above] at ($(axis cs:PingPong, 58.37)$) [xshift=0.5*\pgfkeysvalueof{/pgf/bar width}] {$1.44\times$};
\node[above] at ($(axis cs:ThreadRing, 35.47)$) [xshift=0.7*\pgfkeysvalueof{/pgf/bar width}] {$1.0\times$};
\addplot[
  fill=darkgray,
  postaction={
    pattern color=white,
    pattern=crosshatch,
  },
]
plot coordinates {
  (PingPong, 60.12)
  (ThreadRing, 37.48)
};
\addlegendentry{Akka coroutine}
\node[above] at ($(axis cs:PingPong, 60.12)$) [xshift=2.4*\pgfkeysvalueof{/pgf/bar width}] {$1.48\times$};
\node[above] at ($(axis cs:ThreadRing, 37.48)$) [xshift=2.4*\pgfkeysvalueof{/pgf/bar width}] {$1.06\times$};
\end{axis}
\end{tikzpicture}
\caption{Performance of coroutines and alternative frameworks (lower is better)}
\label{fig:benchmarks}
\end{figure*}

The goal of the evaluation is to assess coroutine performance
on a range of different use cases, most notably those from Section \ref{sec:use-cases}.
The source code of the benchmarks is available online \cite{coroutines}.
Evaluation was done in accordance with established JVM benchmarking methodologies
\cite{Georges:2007:SRJ:1297105.1297033}.
We used the ScalaMeter framework \cite{scalameter}
to repeat each benchmark $30$ times,
across $6$ different JVM process instances,
and we report the average values.
We used a quad-core $2.8$ GHz Intel i7-4900MQ processor
with $32$ GB of RAM,
and results are shown in Figure \ref{fig:benchmarks}.

\textbf{Iterators}.
We test tree iterators from Listing \ref{list:iterator}
against a manually implemented tree iterator.
The first benchmark, \textsl{TreeFindMax},
traverses a single tree and finds the largest integer,
while \textsl{TreeToArray} copies the integers to an array.
\textsl{TreeSameFringe} compares the corresponding integers
in two trees with a different layout \cite{Gabriel:1991:DPP:132218.132225}.
These benchmarks heavily modify the stack,
so a coroutine is $1.9-2.1\times$ slower than an iterator.
A CPS-based iterator,
built using Scala delimited continuations \cite{Rompf:2009:IFP:1631687.1596596},
is $2.4-2.9\times$ slower.
For comparison,
a lazy functional stream is $12-17\times$ slower.

The \textsl{HashLongest} benchmark traverses a hash table
to find the longest string (strings contain size information, so checks are cheap).
Since most of the time is spent in the loop and not in coroutine calls,
performance overhead compared to iterators is only $26\%$.
This benchmark reveals a downside of CPS-based continuations\footnote{In some cases,
the Scala compiler can eliminate tail-calls,
but typically not when invoking lambda objects
that encode the continuations produced by Scala's delimited continutations plugin.
}.
The relative overhead of allocating continuation closures
is considerable for hash table iterators,
so a continuation-based iterator is $6.22\times$ slower.
\textsl{HashZip} simultaneously traverses two hash tables,
picks an element from each pair, and inserts it into a third hash table,
effectively implementing a zip operation on the hash tables.
Since zipping does additional work of implementing the resulting hash table,
coroutines have only a $5\%$ overhead
compared to a manually implemented iterator,
while continuations are $2.1\times$ slower.

\textsl{DFS} and \textsl{BFS} benchmarks traverse a sparse graph (degree 3)
in depth-first and breadth-first order.
Coroutines have an overhead of $34\%$ and $17\%$
compared to manually implemented iterators,
and continuations $90\%$ and $28\%$, respectively.
Making the graphs denser (degree 16) amortizes the overhead of suspensions,
resulting in overheads of $9\%$ and $3\%$ for coroutines.

\textbf{Lazy streams}.
Functional lazy streams, or lazy lists,
are a neat abstraction for recursively defining number series.
Coroutines are also a good fit for this use-case, but are considerably faster,
since a stream needs to create a node object for each number in the series.

The \textsl{Fibonacci} benchmarks generates Fibonacci numbers,
and uses big integer arithmetic to do so.
The overhead of a lazy-stream-based solution
compared to a coroutine-based one is only $15\%$.
The \textsl{Taylor} benchmark generates a Taylor series,
using floating-point arithmetic.
The work involved in a floating-point computation
is much lower compared to big-integer arithmetic.
Since the relative overhead of lazy streams is much more pronounced in this case,
the stream-based solution is $8.4\times$ slower.

\textbf{ScalaCheck}.
The \textsl{TestList} and \textsl{TestFract} benchmarks compare
regular ScalaCheck generator-based testing \cite{scalacheck}
with backtracking from Section \ref{sec:use-cases}.
The \textsl{TestList} benchmark checks properties of list objects,
and is computation-heavy --
relative backtracking overhead due to creating snapshots is only $7\%$.
The \textsl{TestFract} benchmark checks properties of fractions
and does only simple arithmetic --
in this case, backtracking overhead is $41\%$.

\textbf{Async-Await}.
Here, network communication is the primary use-case.
\textsl{FastReq} creates an immediately completed request, and awaits it.
In this case,
coroutine-based implementation from Section \ref{sec:use-cases} has a $17\%$ overhead.
Just for comparison, starting a new thread for each request is $245\times$ slower.
In practice, the network introduces a delay between requests and responses.
\textsl{NetReq} uses a $1$ ms delay,
in which case coroutines have no observable overhead.

\textbf{Single-assignment variables}.
In this benchmark,
Oz-style single-assignment variables from Listing \ref{list:oz1}
are used to implement dataflow streams --
a variant of cons-lists with single-assignment tails.
This allows a straightforward encoding of the producer-consumer pattern
\cite{VanRoy:2004:CTM:983087}.
The \textsl{PC} benchmark compares dataflow streams based on Scala Futures \cite{SIP14}
with coroutine-based streams.
The direct-style coroutine API has an interesting performance impact.
Futures are $52\%$ slower because every tail-read
must allocate a closure and install a callback even if the value is already present,
whereas a coroutine can be directly resumed when a value is available.
The \texttt{LinkedTransferQueue} from the JDK
blocks the thread when waiting for a value,
and is $35\%$ slower.
\textsl{Bounded PC} adds an additional backpressure dataflow stream between
the producer and the consumer, and has similar performance ratios.

\textbf{Actors and event streams}.
We compare callback-style and direct-style
Akka actors \cite{akka}
and reactors
\cite{Prokopec:2015:ICE:2814228.2814245,reactors-website,Prokopec:2016:PSR:3001886.3001891,10.1007/978-3-319-64203-113}
on two benchmarks from the
Savina actor benchmark suite \cite{Imam:2014:SAB:2687357.2687368}.
Direct-style programs are encoded by hot-swapping the event loop,
as explained in Section \ref{sec:use-cases}.
The callback allocation in \texttt{receive} and \texttt{get} calls
causes a $3\%$ slowdown for reactors and $2.8\%$ for actors in \textsl{PingPong}.
In \textsl{ThreadRing}, slowdown is $12\%$ for reactors and $6\%$ for actors.

\begin{figure}
\begin{tikzpicture}[scale=0.58]
\begin{axis}[
  every axis plot post/.style={/pgf/number format/fixed},
  ybar=5pt,
  ylabel=$time/ms$,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=10,
    anchor=south
  },
  height=5cm,
  bar width=12pt,
  x=3.0cm,
  ymin=0,
  axis on top,
  ymax=60,
  xtick=data,
  enlarge x limits=0.06,
  symbolic x coords={TreeSameFringe, HashLongest, DFS, Fibonacci, TestFract, FastReq, PC, PingPong},
  restrict y to domain*=0:80,
  visualization depends on=rawy\as\rawy,
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=-1,
    at={(0.20, 1.14)},
    anchor=north west
  }
]
\addplot[fill=black!0!white]
plot coordinates {
  (TreeSameFringe, 23.91) 
  (HashLongest, 14.09)
  (DFS, 20.32)
  (Fibonacci, 9.66)
  (TestFract, 9.83)
  (PC, 31.92)
  (FastReq, 11.31)
  (PingPong, 40.43)
};
\addlegendentry{all-opts}
\node[above] at ($(axis cs:TreeSameFringe, 23.91)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\node[above] at ($(axis cs:HashLongest, 14.09)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\node[above] at ($(axis cs:DFS, 20.32)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\node[above] at ($(axis cs:Fibonacci, 9.66)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\node[above] at ($(axis cs:TestFract, 9.83)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\node[above] at ($(axis cs:PC, 31.92)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\node[above] at ($(axis cs:FastReq, 11.31)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\node[above] at ($(axis cs:PingPong, 40.43)$) [xshift=-2.2*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.0\times$}};
\addplot[
  fill={rgb:red,10;green,2;blue,1},
  postaction={
    pattern color=white,
    pattern=north west lines,
  },
]
plot coordinates {
  (TreeSameFringe, 34.41)
  (HashLongest, 17.10)
  (DFS, 22.79)
  (Fibonacci, 10.54)
  (TestFract, 10.18)
  (PC, 34.71)
  (FastReq, 12.61)
  (PingPong, 41.79)
};
\addlegendentry{no-is-needed}
\node[above] at ($(axis cs:TreeSameFringe, 34.41)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.43\times$}};
\node[above] at ($(axis cs:HashLongest, 17.10)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.21\times$}};
\node[above] at ($(axis cs:DFS, 22.79)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.12\times$}};
\node[above] at ($(axis cs:Fibonacci, 10.54)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.09\times$}};
\node[above] at ($(axis cs:TestFract, 10.18)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.04\times$}};
\node[above] at ($(axis cs:PC, 34.71)$) [xshift=-0.9*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.09\times$}};
\node[above] at ($(axis cs:FastReq, 12.61)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.12\times$}};
\node[above] at ($(axis cs:PingPong, 41.79)$) [xshift=-0.8*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.03\times$}};
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  postaction={
    pattern color=white,
    pattern=north east lines,
  },
]
plot coordinates {
  (TreeSameFringe, 40.39)
  (HashLongest, 18.28)
  (DFS, 26.56)
  (Fibonacci, 11.47)
  (TestFract, 10.69)
  (PC, 37.86)
  (FastReq, 13.44)
  (PingPong, 42.41)
};
\addlegendentry{no-must-load-no-is-needed}
\node[above] at ($(axis cs:TreeSameFringe, 40.39)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.68\times$}};
\node[above] at ($(axis cs:HashLongest, 18.28)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.30\times$}};
\node[above] at ($(axis cs:DFS, 26.56)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.31\times$}};
\node[above] at ($(axis cs:PC, 37.86)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.19\times$}};
\node[above] at ($(axis cs:Fibonacci, 11.47)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.18\times$}};
\node[above] at ($(axis cs:TestFract, 10.69)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.08\times$}};
\node[above] at ($(axis cs:FastReq, 13.44)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.18\times$}};
\node[above] at ($(axis cs:PingPong, 42.41)$) [xshift=0.6*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.05\times$}};
\addplot[
  fill={rgb:red,0;green,5;blue,2},
  postaction={
    pattern color=white,
    pattern=crosshatch,
  },
]
plot coordinates {
  (TreeSameFringe, 44.70)
  (HashLongest, 20.96)
  (DFS, 28.30)
  (Fibonacci, 11.71)
  (TestFract, 10.71)
  (PC, 41.02)
  (FastReq, 14.57)
  (PingPong, 42.48)
};
\addlegendentry{no-opts}
\node[above] at ($(axis cs:TreeSameFringe, 44.70)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.95\times$}};
\node[above] at ($(axis cs:HashLongest, 20.96)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.49\times$}};
\node[above] at ($(axis cs:DFS, 28.30)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.39\times$}};
\node[above] at ($(axis cs:PC, 41.02)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.29\times$}};
\node[above] at ($(axis cs:Fibonacci, 11.71)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.21\times$}};
\node[above] at ($(axis cs:TestFract, 10.71)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.08\times$}};
\node[above] at ($(axis cs:FastReq, 14.57)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.28\times$}};
\node[above] at ($(axis cs:PingPong, 42.48)$) [xshift=2.3*\pgfkeysvalueof{/pgf/bar width}] {\rotatebox{-90}{$1.05\times$}};
\end{axis}
\end{tikzpicture}
\caption{Impact of optimizations on performance (lower is better)}
\label{fig:optimizations}
\end{figure}

\textbf{Optimization Breakdown}.
We show a breakdown
of different optimizations from Section \ref{sec:optimizations}.
We pick eight benchmarks from Figure \ref{fig:benchmarks}
and run them after disabling different optimization combinations.
We observe the highest impact
on \textsl{TreeSameFringe}, \textsl{HashLongest}, \textsl{DFS} and \textsl{PC}.
In Figure \ref{fig:optimizations},
\textit{all-opts} shows performance with all optimizations enabled,
\textit{no-is-needed} disables the is-needed rule,
\textit{no-must-load-no-is-needed} additionally disables the must-load rule,
and \textit{no-opts} disables all optimizations.
Results show that optimizations have the highest impact on \textsl{TreeSameFringe},
where disabling them causes a total slowdown of almost $2\times$.
Here, $50\%$ of the performance comes from the is-needed rule.
In other benchmarks shown in Figure \ref{fig:optimizations},
total improvement from optimizations ranges from $5\%$ to $50\%$.


==> formal-semantics.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Formal Semantics}\label{sec:formal}

\begin{figure}[t]
% \hspace{-20mm}
\begin{minipage}[t]{7.5 cm}
$\ba[t]{l@{\hspace{-10mm}}r}
\texttt{t} ::= & \defmbox{terms:} \\
\biggap \texttt{(x:T) => t}
& \defmbox{abstraction}  \\
\biggap \texttt{t(t)}
& \defmbox{application}  \\
\biggap \texttt{x}
& \defmbox{variable}  \\
\biggap \texttt{()}
& \defmbox{unit value}  \\
\biggap \texttt{(x:T)} \overset{\texttt{T}}{\rightsquigarrow} \texttt{t}
& \defmbox{coroutine}  \\
\biggap \texttt{yield(t)}
& \defmbox{yielding}  \\
\biggap \texttt{start(t, t)}
& \defmbox{starting}  \\
\biggap \texttt{resume(t, t, t, t)}
& \defmbox{resuming}  \\
\biggap \texttt{snapshot(t)}
& \defmbox{snapshot}  \\
\biggap \texttt{fix(t)}
& \defmbox{recursion}  \\
\biggap i
& \defmbox{instance}  \\
\biggap \langle \texttt{t, v, v, v} \rangle_i
& \defmbox{resumption}  \\
\biggap \llbracket \texttt{t} \rrbracket_\texttt{v}
& \defmbox{suspension}  \\
\biggap \varnothing
& \defmbox{empty term}  \\
\ea$
\end{minipage}
\begin{minipage}[t]{6 cm}
\begin{minipage}[b]{6 cm}
$\ba[t]{l@{\hspace{6mm}}r}
\texttt{T} ::= & \defmbox{types:} \\
\biggap \texttt{T => T}
& \defmbox{function type}  \\
\biggap \texttt{T} \overset{\texttt{T}}{\rightsquigarrow} \texttt{T}
& \defmbox{coroutine type}  \\
\biggap \texttt{T} \leftrightsquigarrow \texttt{T}
& \defmbox{instance type}  \\
\biggap \texttt{Unit}
& \defmbox{unit type}  \\
\biggap \bot
& \defmbox{bottom type}  \\
\ea$
\end{minipage}
\\*

\begin{minipage}[b]{6 cm}
$\ba[t]{l@{\hspace{-6mm}}r}
\texttt{r} ::= & \defmbox{runtime terms:} \\
\biggap i
& \defmbox{instance}  \\
\biggap \langle \texttt{t, v, v, v} \rangle_i
& \defmbox{resumption}  \\
\biggap \llbracket \texttt{t} \rrbracket_\texttt{v}
& \defmbox{suspension}  \\
\biggap \varnothing
& \defmbox{empty term}  \\
\ea$
\end{minipage}
\\*

\begin{minipage}[b]{6 cm}
$\ba[t]{l@{\hspace{4mm}}r}
\texttt{v} ::= & \defmbox{values:} \\
\biggap \texttt{(x:T) => t}
& \defmbox{abstraction}  \\
\biggap \texttt{()}
& \defmbox{unit value}  \\
\biggap \texttt{(x:T)} \overset{\texttt{T}}{\rightsquigarrow} \texttt{t}
& \defmbox{coroutine}  \\
\biggap i
& \defmbox{instance}  \\
\biggap \varnothing
& \defmbox{empty term}  \\
\ea$
\end{minipage}
\end{minipage}

\caption{Syntax and types of the $\lambda_\leadsto$ calculus}
\label{fig:language}
\end{figure}

This section presents the $\lambda_\leadsto$
(pron. \emph{lambda-squiggly}) calculus that captures the core
of the programming model from Section \ref{sec:prog-model}.
This calculus is an extension of the
simply-typed lambda-calculus.
The complete formalization,
along with the proofs of the progress and preservation theorems,
is given in the corresponding tech report \cite{TODO-upload}.

\paratitle{Syntax}
Figure \ref{fig:language} shows the syntax.
The abstraction, application and variable terms are standard.
The \emph{coroutine} term represents coroutine declarations.
The \emph{yield} term corresponds to the \texttt{yieldval} statement shown earlier.
The \emph{start} term is as before, but uses prefix syntax.
The \emph{resume} term encodes
both the \texttt{resume} and the \texttt{value} from Section \ref{sec:prog-model}.
This is because resuming an instance
can complete that instance
(in our implementation, \texttt{resume} returns \texttt{false}),
it can result in a yield
(previously, \texttt{true}),
or fail because an instance had already completed earlier
(in our implementation, an exception is thrown).
In $\lambda_\leadsto$, the \texttt{resume} term therefore accepts four arguments:
the coroutine instance, the result handler,
the yield handler, and the handler for the already-completed case.
The \texttt{fix} term supports recursion \cite{pierce02}.

\begin{figure}[t]
\input{typing-rules.tex}
\input{typing-rules-runtime.tex}
\caption{Typing rules for the $\lambda_\leadsto$ calculus}
\label{fig:typing-relation-complete}
\end{figure}

The calculus differentiates between \emph{user terms},
which appear in user programs,
and \emph{runtime terms},
which only appear during the program evaluation.
A label $i$ is used to represent a coroutine instance.
Each coroutine instance has an evaluation state,
which changes over the lifetime of the instance.
A resumed instance $i$ is represented by the \emph{resumption term}
$\langle \texttt{t,v,v,v} \rangle_i$.
A term that yielded a value \texttt{v}, and is about to be suspended,
is represented by the \emph{suspension term}
$\llbracket \texttt{t} \rrbracket_\texttt{v}$.
Finally, the \emph{empty term} $\varnothing$
is used in the store $\mu$ (shown shortly) when encoding terminated coroutines.
The abstraction term $\texttt{(x:T)=>t}$,
the unit term $\texttt{()}$,
the coroutine definition
$\texttt{(x:T)} \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{t}$,
the instance label $i$ and the empty term $\varnothing$
are considered values.

Note that the calculus distinguishes between standard function types
$\texttt{T}_1\texttt{=>T}_2$
and coroutine types of the form
$\texttt{T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2$,
where $\texttt{T}_y$ is the type of values that the coroutine may yield.
Coroutine instances have the
$\texttt{T}_y \leftrightsquigarrow \texttt{T}_2$ type,
and a unit value has the type \texttt{Unit}.
The bottom type $\bot$ is used to represent
the fact that a term does not yield.
\\*

\paratitle{Example}
Recall the \texttt{rep} coroutine from Listing \ref{list:yield}.
We can encode it in $\lambda_\leadsto$ as follows:

{
\small
\centering
$
\texttt{(x:Int)}
\overset{\texttt{Int}}{\rightsquigarrow}
\texttt{((u:Unit)}
\overset{\texttt{Int}}{\rightsquigarrow}
\texttt{yield(x))(yield(x))}
$

}

The encoding uses a standard trick to sequence two statements \cite{pierce02},
but instead of a regular lambda,
relies on a coroutine to ignore the result of the first statement.
Starting this coroutine
creates a instance $i$, whose current term is saved in the store:

{
\small
\centering
$
\texttt{start(}
\texttt{(x:Int)}
\overset{\texttt{Int}}{\rightsquigarrow}
\texttt{((u:Unit)}
\overset{\texttt{Int}}{\rightsquigarrow}
\texttt{yield(x))(yield(x))}
\texttt{, 7)}
\rightarrow i
$

}

Assume that we now resume this instance once.
We provide three handlers to \texttt{resume}.
We show the complete yield handler (here, identity),
and name the other two $c_2$ and $c_4$:
{\small
  \setlength{\abovedisplayskip}{0pt}
  \setlength{\belowdisplayskip}{\abovedisplayskip}
  % \setlength{\abovedisplayshortskip}{0pt}
  % \setlength{\belowdisplayshortskip}{3pt}
\begin{align*}
\texttt{resume(}
i
\texttt{, }
c_2
\texttt{, }
\texttt{(x:Int)}
\overset{\bot}{\rightsquigarrow}
\texttt{x}
\texttt{, }
c_4
\texttt{)}
& \rightarrow \\
\langle
\texttt{((u:Unit)}
\overset{\texttt{Int}}{\rightsquigarrow}
\texttt{yield(7))(yield(7))}
\texttt{, }
c_2
\texttt{, }
\texttt{(x:Int)}
\overset{\bot}{\rightsquigarrow}
\texttt{x}
\texttt{, }
c_4
\rangle
& \rightarrow \\
\langle
\texttt{((u:Unit)}
\overset{\texttt{Int}}{\rightsquigarrow}
\texttt{yield(7))(} \llbracket \texttt{()} \rrbracket_\texttt{7} \texttt{)}
\texttt{, }
c_2
\texttt{, }
\texttt{(x:Int)}
\overset{\bot}{\rightsquigarrow}
\texttt{x}
\texttt{, }
c_4
\rangle
& \rightarrow \\
\langle
\llbracket
\texttt{((u:Unit)}
\overset{\texttt{Int}}{\rightsquigarrow}
\texttt{yield(7))(())}
\rrbracket_\texttt{7}
\texttt{, }
c_2
\texttt{, }
\texttt{(x:Int)}
\overset{\bot}{\rightsquigarrow}
\texttt{x}
\texttt{, }
c_4
\rangle
& \rightarrow
\texttt{((x:Int)}
\overset{\bot}{\rightsquigarrow}
\texttt{x)(7)}
\rightarrow
\texttt{7}
\end{align*}
}

\paratitle{Typing}
Before showing the typing rules,
we introduce the \emph{instance typing} $\Sigma$,
which tracks coroutine instance types,
and is used alongside the standard typing context $\Gamma$.

\begin{definition}[Instance typing]\label{def:main-instance-typing}
The \emph{instance typing} $\Sigma$
is a sequence of coroutine instance labels and their types
$i\texttt{:T}$,
where comma ($,$) extends a typing with a new binding.
\qed
\end{definition}

\begin{definition}[Typing relation]\label{def:main-typing-rules}
The \emph{typing relation}
$\Sigma | \Gamma \vdash \texttt{t:T} | \texttt{T}_y$
in Fig. \ref{fig:typing-relation-complete}
is a relation between the instance typing $\Sigma$,
the typing context $\Gamma$,
the term \m{t},
its type \m{T},
and the \emph{yield type} $\m{T}_y$,
where $\m{T}_y$ is the type of values that may be yielded when evaluating \m{t}.
\qed
\end{definition}

We inspect the most important rules here,
and refer the reader to
the tech report \cite{TODO-upload-and-cite}
for a complete discussion.
The \textsc{T-Abs} rule is the modification
of the standard abstraction typing rule.
Note that the yield type of the function body \textbf{must be $\bot$}.
This is because $\lambda_\leadsto$ models \emph{delimited coroutines} --
if a \texttt{yield} expression occurs,
it must instead be lexically enclosed within a coroutine term
(which corresponds to the \texttt{coroutine} statement).
We emphasize that $\lambda_\leadsto$ nevertheless models stackfulness --
a \texttt{yield} can still cross coroutine boundaries at runtime
if a coroutine calls another coroutine,
as illustrated in Section \ref{sec:use-cases}, and explained shortly.

Note further, that the \textsc{T-App} rule
permits a non-$\bot$ type on the subterms,
since the reduction of the function and its arguments
is itself allowed to yield.
A non-yielding term can be assumed to yield any type by the \textsc{T-Ctx} rule.
% but the assumption cannot be retracted once taken.
Given a term whose type is \texttt{T} and yield type is also \texttt{T},
the \textsc{T-Yield} rule types a \texttt{yield} expression as \texttt{Unit}
with the yield type \texttt{T}.
% The typing derivation will typically contain a \textsc{T-Ctx} step
% immediately before the \textsc{T-Yield} step.
%(unless typing a term such as \texttt{yield(yield(()))}).

The \textsc{T-Coroutine} rule
allows the body to yield a value of the type $\texttt{T}_y$,
which must correspond to the yield type of the coroutine.
The coroutine itself gets a $\bot$ yield type
(the coroutine definition effectively swallows the yield type).
Consider now the \textsc{T-AppCor} rule,
which is similar to the standard \textsc{T-App} rule for functions.
To directly call another coroutine $\texttt{t}_1$,
its yield type $\texttt{T}_y$ must correspond to the yield type
at the callsite.

Last, we examine the runtime term typing rules.
The \textsc{T-Suspension} rule requires that the
yielded value $\texttt{v}$ has the type $\texttt{T}_y$,
and that the suspension has the same type and yield type
as the underlying suspended term \texttt{t}.
The \textsc{T-Instance} rule
requires that the instance typing $\Sigma$
contains a corresponding type for $i$.
Finally, the \textsc{T-Resumption} term
has the type $\texttt{T}_R$
that corresponds to the return types of the handler coroutines
$\texttt{t}_2$, $\texttt{t}_3$ and $\texttt{t}_4$.
The corresponding yield type is $\texttt{T}_w$,
which is generally different from the yield type $\texttt{T}_y$
that the coroutine instance evaluation $\texttt{t}_1$ can yield.
The empty term can be assigned any type.

\begin{definition}[Well-typed program]\label{def:main-well-typed-term}
A term \texttt{t} is \emph{well-typed} if and only if
$\exists \texttt{T}, \texttt{T}_y, \Sigma$ such that
$\Sigma | \varnothing \vdash \texttt{t:T} | \texttt{T}_y$.
A term \texttt{t} is a \emph{well-typed user program}
if \texttt{t} is well-typed and $\texttt{T}_y = \bot$.
\qed
\end{definition}

\paratitle{Semantics}
Before showing the operational semantics,
we introduce the concept of a coroutine store $\mu$,
which is used to track the evaluation state
of the coroutine instances.

\begin{definition}[Coroutine store]\label{def:coroutine-store}
A \emph{coroutine store} $\mu$ is a sequence of
coroutine instance labels $i$ and their respective evaluation terms \texttt{t},
where the comma operator ($,$) extends the coroutine store
with a new binding $i \triangleright \texttt{t}$.
\qed
\end{definition}

\begin{figure}[t]

\hspace{0.4cm}
\begin{minipage}[t]{6.5cm}
\small
\infrule[\textsc{E-Start}]
{
i \not\in dom(\mu)
}
{
\texttt{start((x:T}_1\texttt{)}\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{t}
\texttt{,v)} | \mu
\rightarrow
i | \mu , i \triangleright [\texttt{x} \mapsto \texttt{v}]\texttt{t}
}
\noindent
\end{minipage}
\begin{minipage}[t]{6.5cm}
\small
\infrule[\textsc{E-Snapshot}]
{
i_2 \not\in dom(\mu)
\quad
i_1 \neq i_2
}
{
\texttt{snapshot(}i_1\texttt{)} | \mu , i_1 \triangleright \texttt{t}
\rightarrow
i_2 | \mu , i_1 \triangleright \texttt{t} , i_2 \triangleright \texttt{t}
}
\noindent
\end{minipage}
\\

\hspace{0.5cm}
\begin{minipage}[t]{5.0cm}
\small
$\quad \quad \texttt{yield(v)} | \mu \rightarrow
\llbracket \texttt{()} \rrbracket_\texttt{v} | \mu$

\hspace*{2cm}
\textsc{(E-Yield)}
\noindent
\end{minipage}
\begin{minipage}[t]{7.5cm}
\small
$\quad
\langle \llbracket \texttt{t}_1 \rrbracket_\texttt{v} \texttt{,v}_2\texttt{,v}_3\texttt{,v}_4 \rangle_i
| \mu , i \triangleright \llbracket \texttt{t}_0 \rrbracket_{v'}
\rightarrow
\texttt{v}_3\texttt{(v)} | \mu , i \triangleright \texttt{t}_1
$

\hspace*{2cm}
\textsc{(E-Capture)}
\noindent
\end{minipage}

\begin{minipage}[t]{12.0cm}
\small
\infrule[\textsc{E-Resume1}]
{
\texttt{t} \neq \llbracket \texttt{t}_0 \rrbracket_\varnothing
}
{
\texttt{resume(}i \texttt{,v}_2\texttt{,v}_3\texttt{,v}_4\texttt{)}
| \mu , i \triangleright \texttt{t}
\rightarrow
\langle \texttt{t,v}_2\texttt{,v}_3\texttt{,v}_4 \rangle_i
| \mu , i \triangleright \llbracket \texttt{t} \rrbracket_\varnothing
}
\noindent
\end{minipage}

\vspace{0.3cm}
\hspace*{1.7cm}
\begin{minipage}[t]{12.0cm}
\small
$
\texttt{resume(}i \texttt{,v}_2\texttt{,v}_3\texttt{,v}_4\texttt{)}
| \mu , i \triangleright \llbracket \texttt{t}_0 \rrbracket_\varnothing
\rightarrow
\texttt{v}_4 \texttt{(}\texttt{()}\texttt{)}
| \mu , i \triangleright \llbracket \texttt{t}_0 \rrbracket_\varnothing
$
\textsc{(E-Resume2)}
\noindent
\end{minipage}

\vspace{0.3cm}
\hspace*{0.7cm}
\begin{minipage}[t]{12.0cm}
\center
\small
$
\langle \texttt{v,v}_2\texttt{,v}_3\texttt{,v}_4 \rangle_i
| \mu , i \triangleright \llbracket \texttt{t}_0 \rrbracket_{\m{v}'}
\rightarrow
\texttt{v}_2 \texttt{(v)}
| \mu , i \triangleright \llbracket \texttt{v} \rrbracket_\varnothing
$
\textsc{(E-Terminate)}
\noindent
\end{minipage}


\caption{A subset of evaluation rules in the $\lambda_\leadsto$ calculus}
\label{fig:evaluation-rules-partial}
\end{figure}

We only show a subset with the
most important evaluation rules in Fig. \ref{fig:evaluation-rules-partial},
and present the complete set of rules in the tech report
\cite{TODO-upload-and-cite}.
The \textsc{E-Start} rule takes a coroutine value and an argument,
and uses them to create a new coroutine instance $i$,
where $i$ is a fresh label.
The coroutine store $\mu$ is modified to include
a binding from $i$ to the coroutine body \texttt{t} after substitution.
Such a coroutine instance $i$ can then be resumed by the \textsc{E-Resume1} rule,
which reduces a \texttt{resume} expression into an resumption term
$\langle \texttt{t,v}_2\texttt{,v}_3\texttt{,v}_4 \rangle_i$.
Note the convention that an executing or a terminated coroutine
has a suspension term $\llbracket \texttt{t}_0 \rrbracket_\varnothing$
in the coroutine store $\mu$.
The \textsc{E-Resume1} rule applies if and only if
$\texttt{t} \neq \llbracket \texttt{t}_0 \rrbracket_\varnothing$.
If the instance is terminated,
the \textsc{E-Resume2} rule applies instead,
which just invokes the `callback' $\texttt{v}_4$ to handle that case.

Consider now what happens when
a resumption term yields.
By \textsc{E-Yield},
the expression \texttt{yield(v)} reduces to a suspended unit value
that is yielding the value \texttt{v}.
A suspension term then spreads across the surrounding terms.
The following two example reductions
spread the suspension across an application.
There is one such rule for each non-value syntax form.


\infax{
\llbracket \texttt{t}_1 \rrbracket_\texttt{v} \texttt{(t}_2\texttt{)} | \mu
\rightarrow
\llbracket \texttt{t}_1\texttt{(t}_2\texttt{)} \rrbracket_\texttt{v} | \mu
}

\infax{
\texttt{v}_1 \texttt{(} \llbracket \texttt{t}_2 \rrbracket_\texttt{v} \texttt{)} | \mu
\rightarrow
\llbracket \texttt{v}_1\texttt{(t}_2\texttt{)} \rrbracket_\texttt{v} | \mu
}

Once the suspension reaches the coroutine resumption term,
the \textsc{E-Capture} reduces it to a call
to the yield handler $\texttt{v}_3$,
and puts the term in the suspension into the store $\mu$.

\paratitle{Safety}
We now state the safety properties of $\lambda_\leadsto$.
Complete proofs are in the tech report \cite{TODO-upload-and-cite}.

\begin{definition}[Well-typed coroutine store]\label{lem:well-typed-store}
A coroutine store $\mu$ is well-typed with respect to the instance typing $\Sigma$,
denoted $\Sigma \vdash \mu$,
if and only if it is true that $\forall i \in dom(\mu)$,
$\Sigma(i) = \texttt{T}_y \leftrightsquigarrow \texttt{T}_2
\Leftrightarrow
\Sigma | \varnothing \vdash \mu(i) \texttt{:T}_2 | \texttt{T}_y$,
and $dom(\Sigma) = dom(\mu)$.
\qed
\end{definition}

\begin{theorem}[Progress]\label{thm:main-progress}
Suppose that \texttt{t} is a closed, well-typed term
for some \texttt{T} and $\Sigma$.
Then, either \texttt{t} is a value,
or \texttt{t} is a suspension term
$\llbracket \texttt{t} \rrbracket_{\texttt{v}}$,
or, for any store $\mu$ such that $\Sigma \vdash \mu$,
there is some term $\texttt{t}'$ and store $\mu'$ such that
$\texttt{t} | \mu \rightarrow \texttt{t}' | \mu'$.
\end{theorem}

\begin{theorem}[Preservation]\label{thm:main-preservation}
If a term and the coroutine store are well-typed,
that is,
$\Sigma | \Gamma \vdash \texttt{t:T} | \texttt{T}_y$,
and
$\Sigma | \Gamma \vdash \mu$,
and if $\texttt{t} | \mu \rightarrow \texttt{t}' | \mu'$,
then there exists $\Sigma' \supseteq \Sigma$
such that
$\Sigma' | \Gamma \vdash \texttt{t}'\texttt{:T} | \texttt{T}_y$
and
$\Sigma' | \Gamma \vdash \mu'$.
\end{theorem}

\begin{cor}[Yield safety]\label{cor:main-yield-safety}
If a user program \texttt{t}$_u$ is well-typed,
then it does not evaluate to a suspension term
of the form $\llbracket \texttt{t} \rrbracket_{\texttt{v}}$.
\end{cor}



==> formal-subtyping.tex <==
% TODO: maybe remove the system with subtyping?


We next show that, in a language with subtyping,
the coroutine type
$\texttt{T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2$
and the instance type
$\texttt{T}_y \leftrightsquigarrow \texttt{T}_2$
are both covariant in their yield type $\texttt{T}_y$.
To achieve this,
we modify the $\lambda_\leadsto$ calculus
to include subtyping.
We define the subtyping relation $\texttt{<:}$ for coroutine types,
and add two new rules to the typing relation.
We name the new calculus $\lambda_{\leadsto\texttt{<:}}$.

\begin{definition}[Subtype relation]\label{def:subtyping-relation}
The \emph{subtype relation} on $\lambda_{\leadsto\texttt{<:}}$
is a two place relation between the types \texttt{S} and \texttt{T},
denoted as $\texttt{S<:T}$,
whose inductive definition is given in Fig. \ref{fig:main-text-subtyping-rules}.
We additionally require that the subtype relation forms a join-semilattice,
that is, for any two types \texttt{S}$_1$ and \texttt{S}$_2$,
there exists a unique type $\texttt{T} = \texttt{S}_1 \sqcup \texttt{S}_2$,
such that $\texttt{S}_1 \texttt{<:} \texttt{T}$,
$\texttt{S}_2 \texttt{<:} \texttt{T}$
and $\not\exists \texttt{T}' \neq \texttt{T}$
such that $\texttt{T}' \texttt{<:T}$, $\texttt{S}_1 \texttt{<:} \texttt{T}'$,
and $\texttt{S}_2 \texttt{<:} \texttt{T}'$.
We also define that
$\forall \texttt{S}, \texttt{S} \sqcup \bot = \texttt{S}$,
and we introduce the type $\top$,
such that $\forall \texttt{S}, \texttt{S} \sqcup \top = \top$.
\qed
\end{definition}

\begin{figure}[t]
\input{subtyping-rules.tex}
\caption{Subtyping rules for the $\lambda_{\leadsto\texttt{<:}}$ calculus}
\label{fig:main-text-subtyping-rules}
\end{figure}

\quad\quad\quad\quad\quad\quad
\input{new-typing-rules.tex}
\\

We then introduce a new typing rule \textsc{T-Sub},
defined with respect to the subtyping relation.
We also modify the earlier rule \textsc{T-Ctx} --
each time a new yield type $\texttt{T}_w$ is encountered,
the typechecker can take the least upper bound
of the previously assumed yield type $\texttt{T}_y$ and $\texttt{T}_w$.
In the appendix,
we show that the progress and preservation hold
in the $\lambda_{\leadsto\texttt{<:}}$ calculus.

% \begin{cor}[Yield covariance]\label{cor:main-yield-safety}
% Coroutines are covariant in their yield types --
% for any two types $\texttt{T}_{y1}$ and $\texttt{T}_{y2}$
% such that $\texttt{T}_{y1}\texttt{<:}\texttt{T}_{y2}$,
% the subtyping relations
% $
% \texttt{T}_1 \overset{\texttt{T}_{y1}}{\rightsquigarrow} \texttt{T}_2,
% \texttt{<:}
% \texttt{T}_1 \overset{\texttt{T}_{y2}}{\rightsquigarrow} \texttt{T}_2
% $,
% and
% $
% \texttt{T}_{y1} \leftrightsquigarrow \texttt{T}_2
% \texttt{<:}
% \texttt{T}_{y2} \leftrightsquigarrow \texttt{T}_2
% $
% hold.
% \end{cor}


\section{Simply Typed Lambda Calculus with Subtyping and Coroutines ($\lambda_{\leadsto\texttt{<:}}$)}
\label{sec:simply-typed-coroutines-subtyping}

The intuition that we want to prove in this section is that,
in a language with subtyping,
a coroutine type
$\texttt{T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2$
is covariant in its yield type.
Similarly, the coroutine instance type
$\texttt{T}_y \leftrightsquigarrow \texttt{T}_2$
is covariant in its yield type.
To prove this,
we extend the $\lambda_\leadsto$ model with subtyping,
and encode the desired covariance properties inside the subtyping relation.
We then prove the progress and preservation properties
for the extended model, $\lambda_{\leadsto\texttt{<:}}$.

% We start by extending the existing syntax.
% In addition to adding the subtyping rules,
% we augment $\lambda_{\leadsto\texttt{<:}}$ with simple records --
% this is a standard extension, since it allows ...

We start by introducing the subtype relation.

\begin{definition}[Subtype relation]\label{def:subtyping-relation}
The \emph{subtype relation} on $\lambda_{\leadsto\texttt{<:}}$
is a two place relation between the types \texttt{S} and \texttt{T},
denoted as $\texttt{S<:T}$,
which represents the cases in which it is
safe to provide instances of type \texttt{S}
when the type \texttt{T} is expected.
Its inductive definition is given in Fig. \ref{fig:subtyping-rules}.
We additionally require that the subtype relation forms a join-semilattice,
that is, for any two types \texttt{S}$_1$ and \texttt{S}$_2$,
there exists a unique type $\texttt{T} = \texttt{S}_1 \sqcup \texttt{S}_2$,
such that $\texttt{S}_1 \texttt{<:} \texttt{T}$,
$\texttt{S}_2 \texttt{<:} \texttt{T}$
and $\not\exists \texttt{T}' \neq \texttt{T}$
such that $\texttt{T}' \texttt{<:T}$, $\texttt{S}_1 \texttt{<:} \texttt{T}'$,
and $\texttt{S}_2 \texttt{<:} \texttt{T}'$.
We also define that
$\forall \texttt{S}, \texttt{S} \sqcup \bot = \texttt{S}$,
and we introduce the type $\top$,
such that $\forall \texttt{S}, \texttt{S} \sqcup \top = \top$.

The set of rules for the typing relation on $\lambda_{\leadsto\texttt{<:}}$
contains all the rules for $\lambda_\leadsto$ from \ref{def:typing-rules},
along with the following rule \textsc{T-Sub}
and an alternative version of the \textsc{T-Ctx} rule:
\\

\input{new-typing-rules.tex}
\qed
\end{definition}

Note that the new version of the \textsc{T-Ctx} rule
is a generalization of the rule from \ref{def:typing-rules}.
In $\lambda_{\leadsto\texttt{<:}}$,
the typechecker starts by assuming the $\bot$ type,
but can the change the decision more than once.
Each time a new yield is encountered,
the previous assumption is joined with the new one.
Since the join operation is commutative and associative,
the typechecker arrives at the same yield type regardless
of the order of traversing the type derivations.

\begin{figure}
\input{subtyping-rules.tex}
\caption{Subtype relation}
\label{fig:subtyping-rules}
\end{figure}


\begin{lemma}[Inversion of the subtyping relation]\label{lem:subtyping-inversion}
\begin{enumerate}
\item
If $\texttt{S<:T}_1\texttt{=>T}_2$,
then $\texttt{S} = \bot$ or $\texttt{S} = \texttt{S}_1\texttt{=>S}_2$,
such that $\texttt{T}_1\texttt{<:S}_1$ and $\texttt{S}_2\texttt{<:T}_2$.
\item
If $\texttt{S<:T}_y\leftrightsquigarrow\texttt{T}_2$,
then $\texttt{S} = \bot$ or
$\texttt{S} = \texttt{S}_y\leftrightsquigarrow\texttt{S}_2$,
such that $\texttt{S}_y\texttt{<:T}_y$ and $\texttt{S}_2\texttt{<:T}_2$.
\item
If $\texttt{S<:T}_1\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_2$,
then $\texttt{S} = \bot$ or
$\texttt{S} = \texttt{S}_1\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{S}_2$,
such that $\texttt{T}_1\texttt{<:S}_1$,
$\texttt{S}_y\texttt{<:T}_y$ and $\texttt{S}_2\texttt{<:T}_2$.
\end{enumerate}
\end{lemma}

\begin{proof}
We show the proof only for the third case, since the other cases are analogous.
If $\texttt{S} = \bot$, the result is immediate.
We only need to consider $\texttt{S} \neq \bot$.
By induction on the subtyping relation,
the relation
$\texttt{S<:T}_1\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_2$
must be derived through \textsc{S-Refl}, \textsc{S-Trans} or \textsc{S-Coroutine}.
The \textsc{S-Refl} case is immediate.

If the last rule used to derive
$\texttt{S<:T}_1\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_2$
is \textsc{S-Trans},
then we know that there exists some type \texttt{U} such that
$\texttt{S<:U}$ and
$\texttt{U<:T}_1\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_2$.
Inductively, \texttt{U} has the form
$\texttt{U}_1\overset{\texttt{U}_y}{\rightsquigarrow}\texttt{U}_2$,
such that $\texttt{T}_1\texttt{<:U}_1$,
$\texttt{U}_y\texttt{<:T}_y$ and $\texttt{U}_2\texttt{<:T}_2$.
But since \texttt{U} is a coroutine type,
we can apply the induction hypothesis to \texttt{S<:U},
so we conclude that \texttt{S} has the form
$\texttt{S}_1\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{S}_2$,
such that $\texttt{U}_1\texttt{<:S}_1$,
$\texttt{S}_y\texttt{<:U}_y$ and $\texttt{S}_2\texttt{<:U}_2$.
If we know apply the \textsc{S-Trans} rule to the facts
$\texttt{S}_j\texttt{<:U}_j$ and $\texttt{U}_j\texttt{<:T}_j$,
where $j \in \lbrace 1, 2, y \rbrace$,
we prove the desired result.

Finally, if the last rule is \textsc{S-Coroutine},
then \texttt{S} has the correct form
$\texttt{S}_1\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{S}_2$,
with the relations $\texttt{T}_1\texttt{<:S}_1$,
$\texttt{S}_y\texttt{<:T}_y$ and $\texttt{S}_2\texttt{<:T}_2$
correspond to the premise of the \textsc{S-Coroutine} rule.
\end{proof}

We next show the main parts of the inversion lemma
that are different with respect to \ref{lem:inversion}
for the $\lambda_\leadsto$ model,
and needed to prove preservation.

\begin{lemma}[Inversion of the coroutine typing]\label{lem:subtyping-typing-inversion}
\begin{enumerate}
\item
If $\Sigma | \Gamma \vdash
\texttt{(x:S}_1\texttt{)}\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{s}_2
\texttt{:T}_1\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_2 | \texttt{T}_w$,
then $\texttt{T}_1\texttt{<:S}_1$,
and
$\Sigma | \Gamma , \texttt{x:S}_1 \vdash
\texttt{s}_2 \texttt{:T}_2 | \texttt{T}_y$.
\item
If $\Sigma | \Gamma \vdash
i\texttt{:T}_y\leftrightsquigarrow\texttt{T}_2 | \texttt{T}_w$,
then $\exists \texttt{S}_y, \texttt{S}_2$ such that
$i \texttt{:S}_y \leftrightsquigarrow \texttt{S}_2 \in \Sigma$,
$\texttt{S}_y\texttt{<:T}_y$, $\texttt{S}_2\texttt{<:T}_2$.
\end{enumerate}
\end{lemma}

\begin{proof}
\begin{enumerate}
\item
Consider the rule \textsc{T-Coroutine}.
If this rule was used to derive the type of
$\texttt{(x:S}_1\texttt{)}\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{s}_2$,
then $\texttt{T}_1 = \texttt{S}_1$,
$\texttt{T}_y = \texttt{S}_y$.

Otherwise, the type of the term was derived by the \textsc{T-Sub} rule.
Then, there is some type
$\texttt{S<:T}_1\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_2$
such that
$\Sigma | \Gamma \vdash
\texttt{(x:S}_1\texttt{)}\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{s}_2
\texttt{:S} | \texttt{T}_w$.
But, from \ref{lem:subtyping-inversion},
we know that
$\texttt{S} = \texttt{S}_1\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{S}_2$,
and that $\texttt{T}_1\texttt{<:S}_1$,
$\texttt{S}_y\texttt{<:T}_y$ and $\texttt{S}_2\texttt{<:T}_2$.
By applying \textsc{T-Coroutine} inductively,
we determine that the typing relation for the coroutine body $\texttt{s}_2$ is
$\Sigma | \Gamma , \texttt{x:S}_1 \vdash \texttt{s}_2 \texttt{:S}_2 | \texttt{S}_y$,
and the claim follows from
$\texttt{S}_y\texttt{<:T}_y$ and $\texttt{S}_2\texttt{<:T}_2$.
\item
Similar.
\end{enumerate}
\end{proof}

\begin{lemma}[Substitution]\label{lem:subtyping-substitution}
If $\Sigma | \Gamma , \texttt{x:S} \vdash \texttt{t:T} | \texttt{T}_y$,
and $\Sigma | \Gamma \vdash \texttt{s:S} | \texttt{T}_y$,
it follows that
$\Sigma | \Gamma \vdash [\texttt{x} \mapsto \texttt{s}] \texttt{t:T} | \texttt{T}_y$.
\end{lemma}

\begin{proof}
The proof is a standard induction on the typing derivations,
with an additional case for \textsc{T-Sub} and \textsc{T-Ctx}.
\end{proof}

\begin{theorem}[Preservation]\label{thm:subtyping-preservation}
If a term and the coroutine store are well-typed,
that is,
$\Sigma | \Gamma \vdash \texttt{t:T} | \texttt{T}_y$,
and
$\Sigma | \Gamma \vdash \mu$,
and if $\texttt{t} | \mu \rightarrow \texttt{t}' | \mu'$,
then there exists $\Sigma' \supseteq \Sigma$
such that
$\Sigma' | \Gamma \vdash \texttt{t}'\texttt{:T} | \texttt{T}_y$
and
$\Sigma' | \Gamma \vdash \mu'$.
\end{theorem}

\begin{proof}
Casewise on the typing derivations,
similar to the proof for \ref{thm:preservation}.

Consider the \textsc{T-AppCor} case,
where $\texttt{t} = \texttt{t}_1\texttt{(t}_2\texttt{)}$,
$\Sigma | \varnothing \vdash
\texttt{t}_1\texttt{:T}_2\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_1
| \texttt{T}_y$,
and
$\Sigma | \varnothing \vdash
\texttt{t}_2\texttt{:T}_2 | \texttt{T}_y$
We skip over the subcases \textsc{E-App1} and \textsc{E-App2}
(in which either $\texttt{t}_1$ or $\texttt{t}_2$ is not a value),
since they are the same as before.
For \textsc{E-AppCor},
$\texttt{t}_1 =
\texttt{(x:S}_2\texttt{)}\overset{\texttt{S}_y}{\rightsquigarrow}\texttt{t}_{11}$,
$\texttt{t}_2 = \texttt{v}_2$,
and $\texttt{t}' = [\texttt{x} \mapsto \texttt{v}_2] \texttt{t}_{11}$.
By \ref{lem:subtyping-typing-inversion},
we know that
$\texttt{T}_2\texttt{<:S}_2$
and
$\Sigma | \Gamma , \texttt{x:S}_2 \vdash
\texttt{t}_{11} \texttt{:T}_1 | \texttt{T}_y$.
By \textsc{T-Sub} and \textsc{T-Ctx},
$\Sigma | \Gamma \vdash \texttt{t}_2\texttt{:S}_2 | \texttt{S}_y$.
By \ref{lem:subtyping-substitution},
we then have
$\Sigma | \Gamma \vdash \texttt{t}'\texttt{:T}_1 | \texttt{T}_y$.
Note also that $\mu' = \mu$. This proves the claim for this case.

The other cases are proven in a similar way,
by relying on the \ref{lem:subtyping-typing-inversion},
along with the \textsc{T-Sub} and \textsc{T-Ctx} rules.
In particular, terms whose evaluation potentially modifies the coroutine store $\mu$,
such as the \texttt{resume} term in the conclusion of \textsc{T-Resume},
rely on the second case of \ref{lem:subtyping-typing-inversion}.
\end{proof}

Before showing the progress property, we need to establish the canonical forms
for specific types.
We show a revised version of \ref{lem:canonical}.

\begin{lemma}[Canonical forms]\label{lem:subtyping-canonical}
\begin{enumerate}
\item
If \texttt{v} is a value of type \texttt{Unit}, then \texttt{v} is \texttt{()}.
\item
If \texttt{v} is a value of type $\texttt{T}_1 \texttt{=>} \texttt{T}_2$,
then $\texttt{v} = \texttt{(x:S}_1\texttt{)=>t}_2$.
\item
If \texttt{v} is a value of type
$\texttt{T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2$,
then $\texttt{v} =
\texttt{(x:S}_1\texttt{)} \overset{\texttt{S}_y}{\rightsquigarrow} \texttt{t}_2$.
\item
If \texttt{v} is a value of type
$\texttt{T}_y \leftrightsquigarrow \texttt{T}_2$,
then $\texttt{v} = i$, where $i$ is an instance label.
\end{enumerate}
\end{lemma}

\begin{proof}
We consider only the third statement.
The typing rules that could have lead to the value of this type
are \textsc{T-Coroutine} and \textsc{T-Sub}.
In the case of \textsc{T-Coroutine},
the result follows immediately from the premise.
In the case of of \textsc{T-Sub},
we have
$\texttt{S<:} \texttt{T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2$
and
$\Sigma | \Gamma \vdash \texttt{v:S} | \texttt{T}_y$.
By \ref{lem:subtyping-typing-inversion},
$\texttt{S} = \texttt{S}_1 \overset{\texttt{S}_y}{\rightsquigarrow} \texttt{S}_2$.
The result then follows from the induction hypothesis.
\end{proof}

\begin{theorem}[Progress]\label{thm:subtyping-progress}
Suppose that \texttt{t} is a closed, well-typed term
for some \texttt{T} and $\Sigma$,
as defined in \ref{def:well-typed-term}.
Then, either \texttt{t} is a value,
or \texttt{t} is a suspension term
$\llbracket \texttt{t} \rrbracket_{\texttt{v}}$,
or, for any store store $\mu$ such that $\Sigma \vdash \mu$,
there is some term $\texttt{t}'$ and store $\mu'$ such that
$\texttt{t} | \mu \rightarrow \texttt{t}' | \mu'$.
\end{theorem}

\begin{proof}
Analogous to the proof of \ref{thm:progress}.
\end{proof}

==> implementation-discussion.tex <==

\section{Description of the Scala implementation}
\label{sec:implementation-details}

In this section,
we describe an implementation
of a Scala AST that contains coroutine control constructs,
to a Scala AST that does not contain coroutines,
but has equivalent semantics, as described in Section \ref{sec:prog-model}.
The section is less formal than the previous sections,
and its goal is to describe some of the concrete implementation details.

The transformation consists of several phases.
First, the AST is converted to a canonical form
that simplifies subsequent transformations.
Second, the canonical AST is converted into a control flow graph.
Third, the control flow graph is cut into segments at the points
where the coroutine yields or directly calls other coroutines.
Fourth, control flow graph segments
are converted back to ASTs, which generate the coroutine's entry points.

\input{phases.tex}

We describe these phases in the following sections.
We maintain a running example program that undergoes the transformation,
and show its form at the end of each phase.
We start with the data model underlying coroutines.


\subsection{Data Model}\label{sec:data-model-appendix}

Each coroutine frame, similar to a method invocation frame,
must store the following:
pointer to the coroutine descriptor,
program counter,
local variables and return values.
As explained in Section \ref{sec:prog-model}, coroutines allow direct calls.
Consequently, a coroutine instance must encode a call stack of coroutine frames.
Some alternative approaches, such as continuations based on CPS transform,
encode calls as a chain of function objects.
We deliberately avoid the object chaining approach, since it is less efficient,
as we show in Section \ref{sec:eval}.

A coroutine call stack can generally be implemented as a single contiguous memory area.
Scala is historically constrained by the JVM platform,
which allows arrays that contain either references or primitive values, but not both.
For this reason,
our implementation separates coroutine descriptors, program counters,
local references and local primitive values into separate stacks.
Creating large call stacks when a coroutine instance starts is costly.
To prevent wasting processing time when
the instance only needs a single or several frames,
the initial size of the stacks is set to $4$ entries.
If a stack push detects an overflow,
a new stack is allocated, its size doubled and old entries copied.
The total work done in push and pop operations is in the worst case
$2\times$ larger compared to an optimally sized stack.
This worst-case is rarely seen in practice,
since most programs have call trees with the average branching factor
greater than $1$ -- the allocated stack space is usually used more than once.
Besides one or more call stacks,
a coroutine instance contains
the last yield value, the result value (if terminated),
and an optionally thrown exception.


\subsection{AST Canonicalization}

The calculus from Section \ref{sec:formal}
models the core coroutine functionality.
Most language implementations
have a more elaborate intermediate format,
which usually includes some combination of
variable declaration, assignment, expressions,
field selection and method calls,
blocks, \texttt{if}-statements, \texttt{while}-loops,
or pattern matching.

In the canonicalization phase,
the AST consisting of typical language node types
gets converted into a restricted form:
single operator expressions,
assignments, declarations, method calls,
\texttt{if}-statements and \texttt{while}-loops.
The advantage of this simplification is that
subsequent phases have fewer cases to consider,
conversion back to ASTs is easier,
and optimizations that analyze data dependencies are less complex
(Section \ref{sec:optimizations}).
As a design decision, we use restricted forms of control constructs
(e.g. \texttt{if}-statements and \texttt{while}-loops)
in the canonicalized form instead of transforming them
into the minimal representation from Section \ref{sec:formal} --
a Scala representation consisting solely of function applications
would degrade performance, or otherwise require intricate optimizations.

\begin{figure}[t]
\small
\centering
\begin{minipage}[t]{5.5cm}
\infrule[\textsc{C-Declaration}]
{ \Phi, \texttt{x} \succ \texttt{t} \rightarrow
  \texttt{C}_{t} \ |\ \texttt{x}_{t} \succ \Delta
}
{ \Phi \vdash
  \texttt{var x=t} \rightarrow
  \texttt{C}_{t} \texttt{;} \texttt{var x=x}_{t} \ |\ \texttt{()}
  \succ \Delta , \texttt{x}
}
\noindent
\end{minipage}
\quad
\begin{minipage}[t]{3.9cm}
\infrule[\textsc{C-Assignment}]
{ \Phi \succ \texttt{t} \rightarrow
  \texttt{C}_{t} \ |\ \texttt{x}_{t} \succ \Delta
}
{
  \Phi \succ \texttt{x=t} \rightarrow
  \texttt{C}_{t} \texttt{;} \texttt{x=x}_{t} \ |\ \texttt{()}
  \succ \Delta
}
\noindent
\end{minipage}
\quad
\begin{minipage}[t]{4.5cm}
\infrule[\textsc{C-Selection}]
{ \texttt{x} \not\in \Phi \cup \Delta
  \quad
  \Phi \succ
  \texttt{t} \rightarrow
  \texttt{C}_t \ |\ \texttt{x}_t
  \succ \Delta
}
{ \Phi \succ
  \texttt{t.m} \rightarrow
  \texttt{C}_t \texttt{;} \texttt{val x=x}_t{.m} \ |\ \texttt{x}
  \succ \Delta , \texttt{x}
}
\noindent
\end{minipage}
\\*

\begin{minipage}[t]{5.8cm}
\infrule[\textsc{C-MethodCall}]
{ \texttt{x} \not\in \Phi \cup \bigcup_{j=0}^{n} \quad
  \Phi \succ \texttt{t}_0 \rightarrow \texttt{C}_0 \ |\ \texttt{x}_0 \succ \Delta_0 \\*
  \forall i \in \{ 1 , \ldots , n \} \enskip
  \Phi \cup \bigcup_{j=0}^{i-1} \Delta_j \succ \texttt{t}_i \rightarrow
  \texttt{C}_i \ |\ \texttt{x}_i \succ \Delta_i \\*
  \texttt{C}_m =
  \texttt{C}_0 \texttt{;} \texttt{C}_1 \texttt{;} \mydots \texttt{;} \texttt{C}_n
  \texttt{;}
  \texttt{val x=x}_0\texttt{.m(x}_1\texttt{,}\mydots\texttt{,x}_n\texttt{)}
}
{ \Phi \succ
  \texttt{t}_0\texttt{.m(t}_1\texttt{,}\mydots\texttt{,t}_n\texttt{)}
  \rightarrow
  \texttt{C}_m \ |\ \texttt{x}
  \succ
  \bigcup_{j=0}^{n} \Delta_j , \texttt{x}
}
\noindent
\end{minipage}
\quad\quad\quad\quad
%\\*
\begin{minipage}[t]{7.6cm}
\infrule[\textsc{C-Block}]
{ \texttt{x} \not\in \Phi \cup \bigcup_{j=1}^{n} \Delta_j
  \\*
  \forall i \in \{ 1 , \ldots , n \} \enskip
  \Phi \cup \bigcup_{j=1}^{i-1} \Delta_j
  \succ \texttt{t}_i \rightarrow \texttt{C}_i \ |\ \texttt{x}_i
  \succ \Delta_i
}
{ \Phi \succ
  \texttt{\{} \texttt{t}_1 \texttt{;} \mydots \texttt{;} \texttt{t}_n \texttt{\}}
  \rightarrow
  \texttt{var x;\{}
  \texttt{C}_1 \texttt{;} \mydots \texttt{;} \texttt{C}_n
  \texttt{;x=x}_n\texttt{\}}
  \ |\ \texttt{x}
  \succ \{ \texttt{x} \}
}
\noindent
\end{minipage}

\vspace{2mm}
\begin{minipage}[t]{0.0cm}
\infrule[\textsc{C-ShortCircuitOr}]
{ \texttt{x} \not\in \Phi \cup \Delta_1 \cup \Delta_2 \quad
  \Phi \succ \texttt{t}_1 \rightarrow \texttt{C}_1 \ |\ \texttt{x}_1 \succ \Delta_1 \\*
  \Phi \cup \Delta_1 , \texttt{x} \succ
  \texttt{t}_2 \rightarrow \texttt{C}_2 \ |\ \texttt{x}_2 \succ \Delta_2 \\*
  \texttt{C}_s =
  \texttt{C}_1 \texttt{;var x;if (x}_1\texttt{) x=true else \{} \texttt{C}_2 \texttt{;x=x}_2\texttt{\}}
}
{ \Phi \succ
  \texttt{t}_1\texttt{||t}_2 \rightarrow
  \texttt{C}_s
  \ |\ \texttt{x}
  \succ
  \Delta_1 , \texttt{x}
}
\noindent
\end{minipage}
\hspace{7cm}
%\\*
\begin{minipage}[t]{8.0cm}
\infrule[\textsc{C-IfThenElse}]
{ \texttt{x} \not\in \Phi \cup \Delta_t \cup \Delta_f
  \quad
  \Phi \succ \texttt{t}_b \rightarrow \texttt{C}_b \ |\ \texttt{x}_b \succ \Delta_b \\*
  \Phi \cup \Delta_b , \texttt{x} \succ
  \texttt{t}_t \rightarrow \texttt{C}_t \ |\ \texttt{x}_t
  \succ \Delta_t \quad
  \Phi \cup \Delta_b , \texttt{x} \succ
  \texttt{f}_f \rightarrow \texttt{C}_f \ |\ \texttt{x}_f
  \succ \Delta_f \\*
  \texttt{C}_{if} =
  \texttt{if (x}_b\texttt{) \{} \texttt{C}_t \texttt{;x=x}_t\texttt{\}}
  \texttt{ else \{} \texttt{C}_f \texttt{;x=x}_f\texttt{\}}
}
{ \Phi \succ \texttt{if (t}_b\texttt{) t}_t\texttt{ else t}_f \rightarrow
  \texttt{C}_b \texttt{;var x;} \texttt{C}_{if} \ |\ \texttt{x}
  \succ \Delta_b , \texttt{x}
}
\noindent
\end{minipage}

\begin{minipage}[t]{7.1cm}
%\\*
\infrule[\textsc{C-While}]
{ \Phi , \texttt{x} \succ
  \texttt{t}_w \rightarrow \texttt{C}_w \ |\ \texttt{x}_w \succ \Delta_w \quad
  \Phi \cup \Delta_w , \texttt{x} \succ
  \texttt{t}_b \rightarrow \texttt{C}_b \ |\ \texttt{x}_b \succ \Delta_b \\*
  \texttt{x} \not\in \Phi \cup \Delta_b \cup \Delta_w \quad
  \texttt{C}_{loop} = \texttt{while (x}\texttt{) \{}
  \texttt{C}_b \texttt{;} \texttt{C}_w \texttt{;x=x}_w\texttt{\}}
}
{ \Phi \succ
  \texttt{while (x) b} \rightarrow
  \texttt{C}_w \texttt{;} \texttt{var x=x}_w \texttt{;} \texttt{C}_{loop} \ |\
  \texttt{()}
  \succ \Delta_w , \texttt{x}
}
\noindent
\end{minipage}
\quad\quad\quad\quad
\begin{minipage}[t]{3.0cm}
%\\*
\infrule[\textsc{C-Constant}]
{ \texttt{k} \in \text{constants}
}
{ \Phi \succ \texttt{k} \rightarrow
  \varnothing \ |\ \texttt{k} \succ \varnothing
}
\noindent
\end{minipage}
\begin{minipage}[t]{3.0cm}
%\\*
\infrule[\textsc{C-Identifier}]
{ \texttt{x} \in \Phi
}
{ \Phi \succ \texttt{x} \rightarrow
  \varnothing \ |\ \texttt{x} \succ \varnothing
}
\noindent
\end{minipage}

% \vspace{2mm}
% \begin{minipage}[t]{12.4cm}
% %\\*
% \infrule[\textsc{C-PatternMatch}]
% { t = \texttt{x match \{ case p}_1 \texttt{=>b}_1 \texttt{; } \mydots \texttt{; }
%   \texttt{case p}_n \texttt{=>b}_n \texttt{ \}} \\*
%   \texttt{v} \in fresh \quad
%   canonical(\texttt{x}) = \mathbb{D}_x \ |\ \texttt{x'} \quad
%   \forall i \in \{ 1, \mydots, n \} \quad
%   canonical(\texttt{b}_i) = \mathbb{D}_{b_i} \ |\ \texttt{b}'_i \\*
%   \mathbb{D}_{p_i} = \texttt{val p}_i \texttt{ = x'} \quad
%   \texttt{p}'_i = \texttt{x' match \{ case p}_i \texttt{=>true; }
%   \texttt{case \_=>false \}}
% }
% { canonical(t) =
%   \substack{
%     \texttt{var v; } \mathbb{D}_x \texttt{; }
%     \texttt{if (p}'_1 \texttt{) \{ } \mathbb{D}_{p_1} \texttt{; } \mathbb{D}_{b_1}
%     \texttt{; v = b}'_1 \texttt{ \} }
%     \\*
%     \texttt{else if } \mydots \texttt{ else if (p}'_n \texttt{) \{ }
%     \mathbb{D}_{p_n} \texttt{; } \mathbb{D}_{b_n} \texttt{; v = b}'_n \texttt{ \} }
%   }
%   \ \bigr|\
%   \texttt{v}
% }
% \noindent
% \end{minipage}

\caption{Informal rewrite rules for canonicalization in Scala}
\label{fig:canonicalization}
\end{figure}

\begin{definition}[Canonicalization transformation]\label{def:canonicalization}
The \emph{canonicalization transformation} is a five place relation
$\Phi \succ \texttt{t} \rightarrow \texttt{C} | \texttt{x} \succ \Delta$,
where $\Phi$ is the set of free variables for the term \texttt{t},
the term $\texttt{C}$ is the transformation of the term \texttt{t},
\texttt{x} is the identifier or the constant that has the same value
as the result of evaluating \texttt{t},
and $\Delta$ is the set of variables declared by the term $\texttt{C}$.
We also define $\Delta , \texttt{x} \triangleq \Delta \cup \{ \texttt{x} \}$.
\qed
\end{definition}

Fig. \ref{fig:canonicalization} shows
the core subset of rewrite rules used in our Scala implementation.
For example, the \textsc{C-Identifier} rule
says that a free variable \texttt{x} translates to an empty tree $\varnothing$,
does not introduce any new identifiers,
and can be referenced with \texttt{x}.
The \textsc{C-Declaration} applies
to local variable declarations --
given that the right hand side \texttt{t}
translates into a term $\texttt{C}_t$,
whose value corresponds to the identifier $\texttt{x}_t$,
the variable declaration translates
to the term $\texttt{C}_t$ followed
by the simple declaration $\texttt{var x=x}_t$.
The other rules work analogously,
and sometimes introduce intermediate variables $\texttt{x}$,
which must not appear inside $\Phi$ and the relevant $\Delta$ sets of the subterms.
%Most other languages require similar rewrite rules.

Consider now the \texttt{bucket} coroutine from Section \ref{sec:prog-model},
which yields the elements of a list.
After canonicalization, this coroutine is transformed
into a new coroutine shown in Listing \ref{list:hash-bucket-canonical}.

\begin{lstlisting}[caption={Canonicalized list coroutine},language=scala,label=list:hash-bucket-canonical,captionpos=t,abovecaptionskip=-\medskipamount]
val bucket = coroutine { (b: List[Int]) =>
  var x_0 = b != Nil
  var x_1 = x_0
  while (x_1) {
    var x_2 = b.head
    var x_3 = yieldval(x_2)
    var x_4 = b.tail
    b = x_4
    var x_0 = b != Nil
    x_1 = x_0 }
  () }
\end{lstlisting}


\subsection{Control Flow Graph Conversion}

\tikzstyle{cfg}=[draw,circle,fill=white,inner sep=0,minimum size=11pt]
\tikzstyle{ptr}=[densely dotted]
\tikzstyle{edg}=[]

\begin{figure*}
\centering
\small
\hspace*{-1.2cm}
\begin{minipage}[t]{2.7cm}
\small
\infrule[\textsc{G-Declaration}]
{ \not\exists \texttt{x}_t \enskip
  \texttt{t} = \texttt{yieldval(x}_t\texttt{)} \\*
  \not\exists \texttt{x}_1 , \texttt{x}_2 \enskip
  \texttt{t} = \texttt{x}_1\texttt{(x}_2\texttt{)} \wedge
  \Sigma | \Gamma \not\vdash \texttt{x}_1 \texttt{:}
  \texttt{T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2 | \bot
}
{ \begin{tikzpicture}
  \node()    at (-2.10, -0.25) []    {$\texttt{var x=t} \rightarrow$};
  \node(yn)  at ( 0.00,  0.00) [cfg] {};
  \node      at ( 0.00, -0.45) []    {$\texttt{var x=t}$};
  \node(ynl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(ynr) at ( 0.90, -0.15) []    {\scriptsize{$last$}};
  %
  \draw[-stealth,ptr] (ynl) -- (yn);
  \draw[-stealth,ptr] (ynr) -- (yn);
  \end{tikzpicture}
}
\end{minipage}
\quad\quad\quad\quad\quad\quad\quad\quad\quad\enskip
\begin{minipage}[t]{3.9cm}
\small
\begin{tikzpicture}
  \node()    at (-1.80, -0.25) []    {$\texttt{x=x}_t \rightarrow$};
  \node(yn)  at ( 0.00,  0.00) [cfg] {};
  \node      at ( 0.05, -0.45) []    {$\texttt{x=x}_t$};
  \node(ynl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(ynr) at ( 0.90, -0.15) []    {\scriptsize{$last$}};
  %
  \draw[-stealth,ptr] (ynl) -- (yn);
  \draw[-stealth,ptr] (ynr) -- (yn);
\end{tikzpicture}

\hspace*{1.4cm}
\textsc{(G-Assignment)}
\noindent
\end{minipage}
\begin{minipage}[t]{5.0cm}
\small
\begin{tikzpicture}
  \node()    at (-2.90, -0.25) []    {$\texttt{var x=yieldval(x}_t\texttt{)} \rightarrow$};
  \node(yn)  at ( 0.00,  0.00) [cfg] {\scriptsize{Y}};
  \node      at ( 0.00, -0.45) []    {$\texttt{var x=yieldval(x}_t\texttt{)}$};
  \node(ynl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(ynr) at ( 0.90, -0.15) []    {\scriptsize{$last$}};
  %
  \draw[-stealth,ptr] (ynl) -- (yn);
  \draw[-stealth,ptr] (ynr) -- (yn);
\end{tikzpicture}

\hspace*{2.0cm}
\textsc{(G-YieldVal)}
\noindent
\end{minipage}

\hspace*{-0.5cm}
\begin{minipage}[t]{6.9cm}
\infrule[\textsc{G-AppCor}]
{ \Sigma | \Gamma \vdash
  \texttt{t}_c\texttt{:T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2 | \bot \\*
  \texttt{t} = \texttt{var x = t}_c\texttt{(x}_1 \texttt{, } \ldots \texttt{, x}_n \texttt{)}
}
{ \begin{tikzpicture}
  \node()    at (-1.60, -0.25) []    {$\texttt{t} \rightarrow$};
  \node(yn)  at ( 0.00,  0.00) [cfg] {\scriptsize{C}};
  \node      at ( 0.00, -0.45) []    {$\texttt{t}$};
  \node(ynl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(ynr) at ( 0.90, -0.15) []    {\scriptsize{$last$}};
  %
  \draw[-stealth,ptr] (ynl) -- (yn);
  \draw[-stealth,ptr] (ynr) -- (yn);
  \end{tikzpicture}
}
\noindent
\end{minipage}
% \vspace{2mm}
% \begin{minipage}[t]{4.4cm}
% \infrule[\textsc{Yield-To}]
% { \Gamma \vdash \texttt{var v = yieldto(c)}
% }
% { \begin{tikzpicture}
%   \node(yn)  at ( 0.00,  0.00) [cfg] {\scriptsize{Yt}};
%   \node      at ( 0.00, -0.45) []    {$\substack{\Gamma \odot v \\* \texttt{c}}$};
%   \node(ynl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
%   \node(ynr) at ( 0.90, -0.15) []    {\scriptsize{$last$}};
%   %
%   \draw[-stealth,ptr] (ynl) -- (yn);
%   \draw[-stealth,ptr] (ynr) -- (yn);
%   \end{tikzpicture}
% }
% \noindent
% \end{minipage}
\quad\quad
\begin{minipage}[t]{8cm}
\infrule[\textsc{G-IfThenElse}]
{ \texttt{t} = \texttt{if (t}_c\texttt{) t}_1\texttt{ else t}_2
  \\*
  \begin{tikzpicture}
  \node()    at (-0.70,  0.00) []    {$\texttt{t}_1 \rightarrow$};
  \node(tn1) at ( 0.00,  0.00) [cfg] {\scriptsize{1}};
  \node(tn2) at ( 1.00,  0.00) [cfg] {\scriptsize{2}};
  \path[-,dashed] (tn1.north east) edge[bend left=+30] (tn2.north west);
  \path[-,dashed] (tn1.south east) edge[bend left=-30] (tn2.south west);
  \end{tikzpicture}
  \quad
  \begin{tikzpicture}
  \node()    at (-0.70,  0.00) []    {$\texttt{t}_2 \rightarrow$};
  \node(fn1) at ( 0.00,  0.00) [cfg] {\scriptsize{3}};
  \node(fn2) at ( 1.00,  0.00) [cfg] {\scriptsize{4}};
  \path[-,dashed] (fn1.north east) edge[bend left=+30] (fn2.north west);
  \path[-,dashed] (fn1.south east) edge[bend left=-30] (fn2.south west);
  \end{tikzpicture}
}
{ %\qquad
  %\qquad
  %\qquad
  %\qquad
  \begin{tikzpicture}
  \node()    at (-1.60, -0.25) []    {$\texttt{t} \rightarrow$};
  \node(in1) at ( 0.00,  0.00) [cfg] {\scriptsize{Is}};
  \node      at ( 0.00, -0.45) []    {$\texttt{t}_c$};
  \node(inl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(in2) at ( 2.50,  0.00) [cfg] {\scriptsize{Ie}};
  \node      at ( 2.50, -0.45) []    {$\varnothing$};
  \node(inr) at ( 3.40, -0.15) []    {\scriptsize{$last$}};
  %
  \node(tn1) at ( 0.75,  0.30) [cfg] {\scriptsize{1}};
  \node(tn2) at ( 1.75,  0.30) [cfg] {\scriptsize{2}};
  \path[-,dashed] (tn1.north east) edge[bend left=+30] (tn2.north west);
  \path[-,dashed] (tn1.south east) edge[bend left=-30] (tn2.south west);
  %
  \node(fn1) at ( 0.75, -0.30) [cfg] {\scriptsize{3}};
  \node(fn2) at ( 1.75, -0.30) [cfg] {\scriptsize{4}};
  \path[-,dashed] (fn1.north east) edge[bend left=+30] (fn2.north west);
  \path[-,dashed] (fn1.south east) edge[bend left=-30] (fn2.south west);
  %
  \draw[-stealth,edg] (in1) -- (tn1);
  \draw[-stealth,edg] (in1) -- (fn1);
  \draw[-stealth,edg] (tn2) -- (in2);
  \draw[-stealth,edg] (fn2) -- (in2);
  %
  \draw[-stealth,ptr] (inl) -- (in1);
  \draw[-stealth,ptr] (inr) -- (in2);
  %
  \path[-stealth,dashed] (in1.south east) edge[bend left=-60] (in2.south west);
  \end{tikzpicture}
  %\qquad
  %\qquad
  %\raisebox{15pt}{\textsc{(If-Then-Else)}}
}
\noindent
\end{minipage}

\vspace{2mm}
\hspace{-0.4cm}
\begin{minipage}[t]{5.6cm}
\infrule[\textsc{G-While}]
{ \raisebox{-5pt}{
  \begin{tikzpicture}
  \node()    at (-2.80,  0.00) []    {$\texttt{t} = \texttt{while (t}_c\texttt{) t}_b$};
  \node()    at (-0.60,  0.00) []    {$\texttt{t}_b \rightarrow$};
  \node(tn1) at ( 0.00,  0.00) [cfg] {\scriptsize{1}};
  \node(tn2) at ( 1.00,  0.00) [cfg] {\scriptsize{2}};
  \path[-,dashed] (tn1.north east) edge[bend left=+30] (tn2.north west);
  \path[-,dashed] (tn1.south east) edge[bend left=-30] (tn2.south west);
  \end{tikzpicture}
  }
}
{ \begin{tikzpicture}
  \node()    at (-1.60, -0.25) []    {$\texttt{t} \rightarrow$};
  \node(wn1) at ( 0.00,  0.00) [cfg] {\scriptsize{Ws}};
  \node      at ( 0.00, -0.45) []    {$\texttt{t}_c$};
  \node(wnl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(wn2) at ( 2.50,  0.00) [cfg] {\scriptsize{We}};
  \node      at ( 2.50, -0.45) []    {$\varnothing$};
  \node(wnr) at ( 3.40, -0.15) []    {\scriptsize{$last$}};
  %
  \node(bn1) at ( 0.75,  0.00) [cfg] {\scriptsize{1}};
  \node(bn2) at ( 1.75,  0.00) [cfg] {\scriptsize{2}};
  \path[-,dashed] (bn1.north east) edge[bend left=+30] (bn2.north west);
  \path[-,dashed] (bn1.south east) edge[bend left=-30] (bn2.south west);
  %
  \draw[-stealth,edg] (wn1) -- (bn1);
  \draw[-stealth,edg] (bn2) -- (wn2);
  \path[-stealth,edg] (wn1.north east) edge[bend left=+30] (wn2.north west);
  \path[-stealth,edg] (wn2.south west) edge[bend left=+30] (wn1.south east);
  %
  \draw[-stealth,ptr] (wnl) -- (wn1);
  \draw[-stealth,ptr] (wnr) -- (wn2);
  \end{tikzpicture}
}
\noindent
\end{minipage}
\quad\quad
\begin{minipage}[t]{7.1cm}
\infrule[\textsc{G-Block}]
{ \begin{aligned}
  \texttt{t} = \texttt{\{ t}_1 &\texttt{; } \ldots \texttt{; } \texttt{t}_n \texttt{ \}}
  \end{aligned}
  \quad
  \raisebox{-5pt}{
  \begin{tikzpicture}
  \node()    at (-1.60,  0.00) []    {$\forall i \in \{ 1, \ldots, n \} \,\, \texttt{t}_i \rightarrow$};
  \node(tn1) at ( 0.00,  0.00) [cfg] {\scriptsize{i}};
  %\node      at ( 0.00, -0.40) []    {$\substack{\Gamma'_i}$};
  \node(tn2) at ( 1.00,  0.00) [cfg] {\scriptsize{i'}};
  %\node      at ( 1.00, -0.40) []    {$\substack{\ \ \ \Gamma_{i + 1}}$};
  \path[-,dashed] (tn1.north east) edge[bend left=+30] (tn2.north west);
  \path[-,dashed] (tn1.south east) edge[bend left=-30] (tn2.south west);
  \end{tikzpicture}
  }
}
{ \begin{tikzpicture}
  \node()    at (-1.60, -0.25) []    {$\texttt{t} \rightarrow$};
  \node(wn1) at ( 0.00,  0.00) [cfg] {\scriptsize{Bs}};
  \node      at ( 0.00, -0.45) []    {$\substack{\Gamma \\* \varnothing}$};
  \node(wnl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(wn2) at ( 5.00,  0.00) [cfg] {\scriptsize{Be}};
  \node      at ( 5.00, -0.45) []    {$\substack{\Gamma \\* \varnothing}$};
  \node(wnr) at ( 5.90, -0.15) []    {\scriptsize{$last$}};
  %
  \node(1n1) at ( 0.75,  0.00) [cfg] {\scriptsize{1}};
  \node      at ( 0.75, -0.40) []    {$\substack{\Gamma'_1}$};
  \node(1n2) at ( 1.75,  0.00) [cfg] {\scriptsize{1'}};
  \node      at ( 1.75, -0.40) []    {$\substack{\Gamma_2}$};
  \path[-,dashed] (1n1.north east) edge[bend left=+30] (1n2.north west);
  \path[-,dashed] (1n1.south east) edge[bend left=-30] (1n2.south west);
  %
  \node(nn1) at ( 3.25,  0.00) [cfg] {\scriptsize{n}};
  \node      at ( 3.25, -0.40) []    {$\substack{\Gamma'_n}$};
  \node(nn2) at ( 4.25,  0.00) [cfg] {\scriptsize{n'}};
  \node      at ( 4.25, -0.40) []    {$\substack{\ \ \ \Gamma_{n + 1}}$};
  \path[-,dashed] (nn1.north east) edge[bend left=+30] (nn2.north west);
  \path[-,dashed] (nn1.south east) edge[bend left=-30] (nn2.south west);
  %
  \node(dot) at ( 2.50,  0.00) []    {$\ldots$};
  \draw[-stealth,edg] (1n2) -- (dot);
  \draw[-stealth,edg] (dot) -- (nn1);
  %
  \draw[-stealth,edg] (wn1) -- (1n1);
  \draw[-stealth,edg] (nn2) -- (wn2);
  %
  \draw[-stealth,ptr] (wnl) -- (wn1);
  \draw[-stealth,ptr] (wnr) -- (wn2);
  \end{tikzpicture}
}
\noindent
\end{minipage}
\caption{Informal illustration of the core control flow graph construction rules}
\label{fig:cfg-construction}
\end{figure*}

In this phase, a canonicalized AST is converted to a control-flow graph.
The transformation is explained as a set of mappings
between the input AST and the output CFG nodes.
Figure \ref{fig:cfg-construction} shows
the informal rewrite relations for different types of ASTs.
Pointers \texttt{head} and \texttt{last} always
point to the first and the last node in the control flow of the resulting CFG.
Rule \textsc{G-Declaration} states that
declaration of a variable \texttt{x},
whose right-hand size is not a \texttt{yieldval}
and is not a direct coroutine call,
produces a single node, with the declaration stored inside the node.
Rules \textsc{G-YieldVal} and \textsc{G-AppCor} are similar,
but they tag the output nodes as yields or direct calls,
respectively.
The \textsc{G-IfThenElse} rule constructs the CFG
from the transformation results of the two branches.
Branching node \textsl{Is} stores the branch condition \lstinline$c$,
and a non-successor link to the merge node \textsl{Ie},
shown with a dashed line.
The \textsc{G-While} rule similarly encloses the loop body
between \textsl{Ws} and \textsl{We} nodes,
which are connected with successor links (solid lines).
The rule \textsc{G-Block} transforms a block with a list of statements
into a chain of CFG nodes.

Recall once more the \texttt{bucket} coroutine from Section \ref{sec:prog-model}.
The respective control flow graph that is the output CFG conversion
is shown below.
Nodes that do not represent structured control flow or yielding
are annotated with the corresponding line number
in Listing \ref{list:hash-bucket-canonical}.
\\*

\hspace{2cm}
\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{2}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{3}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{Ws}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{5}};
\draw[-stealth,edg] (n2) -- (n3);
\node(n4)    at ( 3.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (n3) -- (n4);
\node(n5)    at ( 3.75,  0.00) [cfg] {\scriptsize{7}};
\draw[-stealth,edg] (n4) -- (n5);
\node(n6)    at ( 4.50,  0.00) [cfg] {\scriptsize{8}};
\draw[-stealth,edg] (n5) -- (n6);
\node(n7)    at ( 5.25,  0.00) [cfg] {\scriptsize{9}};
\draw[-stealth,edg] (n6) -- (n7);
\node(n8)    at ( 6.00,  0.00) [cfg] {\scriptsize{10}};
\draw[-stealth,edg] (n7) -- (n8);
\node(n9)    at ( 6.75,  0.00) [cfg] {\scriptsize{We}};
\draw[-stealth,edg] (n8) -- (n9);
\node(n10)   at ( 7.50,  0.00) [cfg] {\scriptsize{11}};
\draw[-stealth,edg] (n9) -- (n10);
\node(ret)   at ( 8.40, -0.00) []    {\scriptsize{$return$}};
\draw[-stealth,edg] (n10) -- (ret);
\path[-stealth,edg] (n2.north east) edge[bend left=+20] (n9.north west);
\path[-stealth,edg] (n9.south west) edge[bend left=+20] (n2.south east);
%
\end{tikzpicture}


\subsection{Control Flow Graph Splitting}\label{sec:cfg-split-appendix}

Resuming a coroutine effectively jumps to the middle of its body.
Such a jump is not possible in the source language
that supports only structured programming constructs.
The transformation therefore
outputs multiple \emph{entry point} subroutines,
each containing only structured control flow.
Each such entry point corresponds either to the beginning of the coroutine,
or to the continuation after a yield point or after a direct coroutine call.
Therefore, the control flow graph created in the previous phase
must be split into multiple segments, each corresponding to an entry point.

The splitting algorithm starts at the node that corresponds
to the coroutine method entry,
and traverses the nodes of the graph until reaching a previously unseen yield-site.
The yield-site is then added to the work-list,
and the process is repeated until the work-list becomes empty.
If the graph traversal encounters an \textsl{Ie} node
whose corresponding \textsl{Is} node was not seen as part of the same segment
(which could happen if there was a yield inside an \texttt{if}-branch),
such a node is converted into a \textsl{Be} (block exit) node.
Similarly, a \textsl{We} node without a corresponding \textsl{Ws} node
is replaced with a \textsl{Be} node,
followed by the start of the loop.

The control flow graph of the
\texttt{bucket} coroutine from Section \ref{sec:prog-model},
produced in the previous phase,
is split into the following segments:

\hspace{2cm}
\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{2}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{3}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{Ws}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{5}};
\draw[-stealth,edg] (n2) -- (n3);
\node(n4)    at ( 3.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (n3) -- (n4);
\node(n9)    at ( 4.75,  0.00) [cfg] {\scriptsize{We}};
\node(n10)   at ( 5.50,  0.00) [cfg] {\scriptsize{11}};
\draw[-stealth,edg] (n9) -- (n10);
\node(ret)   at ( 6.40, -0.00) []    {\scriptsize{$return$}};
\draw[-stealth,edg] (n10) -- (ret);
\path[-stealth,edg] (n2.north east) edge[bend left=+20] (n9.north west);
\path[-stealth,edg] (n9.south west) edge[bend left=+20] (n2.south east);
%
\end{tikzpicture}

\hspace{2cm}
\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{7}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{8}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{9}};
\draw[-stealth,edg] (n2) -- (n3);
\node(n4)    at ( 3.00,  0.00) [cfg] {\scriptsize{10}};
\draw[-stealth,edg] (n3) -- (n4);
\node(n5)    at ( 3.75,  0.00) [cfg] {\scriptsize{Be}};
\draw[-stealth,edg] (n4) -- (n5);
\node(n6)    at ( 4.50,  0.00) [cfg] {\scriptsize{Ws}};
\draw[-stealth,edg] (n5) -- (n6);
\node(n7)    at ( 5.25,  0.00) [cfg] {\scriptsize{5}};
\draw[-stealth,edg] (n6) -- (n7);
\node(n8)    at ( 6.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (n7) -- (n8);
\node(n9)    at ( 6.75,  0.00) [cfg] {\scriptsize{We}};
\node(n10)   at ( 7.50,  0.00) [cfg] {\scriptsize{11}};
\draw[-stealth,edg] (n9) -- (n10);
\node(ret)   at ( 8.40, -0.00) []    {\scriptsize{$return$}};
\draw[-stealth,edg] (n10) -- (ret);
\path[-stealth,edg] (n6.north east) edge[bend left=+20] (n9.north west);
\path[-stealth,edg] (n9.south west) edge[bend left=+20] (n6.south east);
%
\end{tikzpicture}


\subsection{AST Generation}\label{sec:ast-gen-appendix}

In this phase,
segments of the original CFG are used to produce ASTs for the entry point methods.
Each entry point first restores the local variables from the stack,
and ends by storing them back to the stack.
The end of each entry point must either store the yield value into the coroutine,
or store the result value.
These entry point methods are placed into a common Scala class.
A separate \texttt{entry} method is then added,
which switches on the current program counter of the coroutine instance,
and dispatches to the proper entry point.

\begin{multicols}{2}
\begin{lstlisting}[caption={Entry point 0 for the list traversal coroutine},language=scala,label=list:hash-bucket-ep0,captionpos=t,abovecaptionskip=-\medskipamount]
def ep0(i: Instance[Int, Unit]): Unit = {
  var b = i.refstack[i.refstacktop + 0]
  var x_0 = b != Nil
  var x_1 = x_0
  while (x_1) {
    var x_2 = b.head
    i.value = x_2
    i.valstack[i.valstacktop + 0] = x_1
    i.pcstack[i.pcstacktop + 0] = 1
    return
  }
  i.result = ()
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Entry point 1 for the list traversal coroutine},language=scala,label=list:hash-bucket-ep1,captionpos=t]
def ep1(i: Instance[Int, Unit]): Unit = {
  var b = i.refstack[i.refstacktop + 0]
  var x_1 = i.valstack[i.valstacktop + 0]
  {
    var x_3 = ()
    var x_4 = b.tail
    b = x_4
    var x_4 = b != Nil
    x_1 = x_4
  }
  while (x_1) {
    var x_2 = b.head
    i.value = x_2
    i.valstack[i.valstacktop + 0] = x_1
    i.pcstack[i.pcstacktop + 0] = 1
    return
  }
  i.result = ()
}
\end{lstlisting}
\end{multicols}

Listings \ref{list:hash-bucket-ep0} and \ref{list:hash-bucket-ep1}
show the implementation of the entry points of the \texttt{bucket} coroutine.
Note that each method starts by restoring the local variable \texttt{b}
from the reference stack of the coroutine instance \texttt{i}.
Each entry point ends by either storing the yield value
into the \texttt{value} field of the coroutine instance,
or the result value into the \texttt{result} field.
Local variables are then stored onto the stack
(there are two stacks -- \texttt{valstack} for primitive values
and \texttt{refstack} for references),
and the program counter is stored to the \texttt{pcstack}.


\subsection{Exception Handling and Non-Local Control Flow}
\label{sec:non-local-appendix}

Exception handling is a special case of non-local control flow,
in which the non-local jump, an exception throw,
targets the nearest enclosing \texttt{try} block.
We introduce \textsl{E}-nodes that are similar to basic block nodes,
but model \texttt{try} statements.
We also introduce the throw node \textsl{T},
which behaves like a yield point,
but sets the \texttt{exception} field of the instance.
An entry point throws at the beginning of its body if this field is non-empty.
This effectively unwinds the stack until the exception is caught.

The \texttt{return} statement is similarly enabled
by adding a new node type \textsl{R},
which behaves like a last regular node in the control flow graph.
Arbitrary \texttt{goto} statements can be encoded as additional exit points.
This approach also allows encoding other kinds of non-local control constructs.


\subsection{Optimizations}
\label{sec:optimizations-appendix}

The translation back to ASTs
benefits from reusing the host language optimizations.
However, most compilers do not optimize code across different entry point methods.
One large overhead is that
entry points must load the local variables in the initial block,
and yield points must store the variables in scope.
These loads and stores have high overheads.
For this reason,
we define a $mustLoad$ relation
that states that a variable must be loaded in a CFG segment
only if it is read in that block before being assigned.
We similarly define a $wasChanged$ relation
to store only those variables that the CFG segment mutated.
Finally,
the variable is not stored at an exit point
if the subsequent CFG segments never read the variable before writing it,
which is defined by the $isNeeded$ relation.
All three relations are implemented as straightforward CFG traversals.

Consider the entry points of the \texttt{bucket} coroutine from
Listings \ref{list:hash-bucket-ep0} and \ref{list:hash-bucket-ep1}.
The store of the variable \texttt{x\_1} (i.e. the loop condition)
to the value stack is unnecessary,
since all the reachable entry points write to \texttt{x\_1}
before reading \texttt{x\_1}.
Therefore, the $isNeeded$ relation does not hold for \texttt{x\_1} at this exit point,
and the corresponding stack store can be removed from the code.
Similarly, the $mustLoad$ relation does not hold for \texttt{x\_1},
so the corresponding stack load can be removed from \texttt{ep1}.


==> implementation.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Implementation}
\label{sec:implementation}

This section describes our metaprogramming-based coroutine implementation in Scala,
which consists of a runtime library and an AST-level transformation.

% The transformation follows the general approach of the formal transformation model
% from Section \ref{sec:formal-transformation}:
% \newline
% \hphantom{,}
% \hspace{-3.4mm}
% \begin{enumerate*}[label=(\arabic{*}),itemsep=0mm]
% \item
% The transformation is restricted to sections delimited
% with the \texttt{coroutine} keyword.
% \newline
% \hphantom{,}
% \hspace{-3.4mm}
% \item
% The coroutine body is spliced into a sequence of segments
% at the yield points.
% Local state is stored at the end of each segment,
% and either a yield or a result value is produced.
% \newline
% \hphantom{,}
% \hspace{-3.4mm}
% \item
% Yielding stores the call stack,
% and resuming retrieves the call stack.
% However, the stack is built eagerly --
% a new stack frame is added whenever a coroutine calls into another coroutine
% (instead of lazily, as in Section \ref{sec:formal-transformation}).
% Consequently, yielding does not traverse the stack,
% and is $O(1)$ with respect to the stack size.
% As a tradeoff, a snapshot must duplicate the call stack.
% \end{enumerate*}


\subsection{Preliminaries}\label{sec:preliminaries}

Our implementation relies on Scala Macros
\cite{Burmako:2013:SML:2489837.2489840},
the metaprogramming API in Scala\footnote{We have an ongoing second implementation
that relies on a newer Scala Macros API,
but we are using the original Scala Macros for the evaluation purposes in this paper.
}.
The following are the key metaprogramming features of Scala Macros
that our transformation scheme relies on.
First, it must be possible to declare \textit{macro definitions}
that take ASTs as input arguments and return transformed ASTs.
Second, it must be possible to invoke such macro definitions from user programs,
which makes the compiler execute the macro with its argument expressions
and replace the macro invocation with the resulting ASTs.
Third, it must be possible to decompose and compose ASTs
inside the macro definition.
Finally, it must be possible to inspect the types of the expressions
passed to the macro, and reason about symbol identity.
The following is an example of a macro definition:

\begin{lstlisting}[language=scala,label=list:log,captionpos=t]
def log(msg: String): Unit = macro log_impl
def log_impl(c: Context)(msg: c.Tree): c.Tree =
  q"""if (loggingEnabled) info(currentTime() + ": " + $msg)"""
\end{lstlisting}

In the above, we declared a \texttt{log} macro
with the macro implementation \texttt{log\_impl},
which takes the corresponding \texttt{Tree} of \texttt{msg} as argument.
The \texttt{log\_impl} method uses the quasiquote notation \texttt{q""}
to build an AST \cite{EPFL-REPORT-185242},
which in turn checks if logging is enabled
before constructing the command line output from the \texttt{msg} string.
Values are interpolated into the AST using the \texttt{\$} notation,
as is the case with the expression \texttt{\$msg} above.

Scala macro definitions can be packaged into libraries.
Our coroutine implementation is therefore a macro library,
which the user program can depend on.
User coroutines implemented with our coroutine library
can be similarly packaged into third party libraries.


\subsection{Runtime Model}\label{sec:data-model}

When yielding, the coroutine instance must store the state of the local variables.
When resuming, that state must be retrieved into the local variables.
Since coroutines are stackful, i.e. they support nested coroutine calls,
it is necessary to store the entire coroutine call stack.

\paratitle{Call stacks}
Our implementation uses arrays to represent coroutine call stacks.
A call stack is divided into a sequence of coroutine frames,
which are similar to method invocation frames.
Each frame stores the following:
\begin{enumerate*}[label=(\arabic{*}),itemsep=0mm]
\item
pointer to the coroutine object (i.e. €coroutine€ block),
\item
the position in the coroutine where the last yield occurred,
\item
the local variables and the return values.
\end{enumerate*}
A coroutine call stack can be implemented as a single contiguous memory area.
Scala is constrained by the JVM platform,
on which arrays contain either object references or primitive values, but not both.
For this reason, our implementation separates
coroutine descriptors, program counters and local variables
into reference and value stacks.

It would be costly to create a large call stack whenever a coroutine instance starts.
Many coroutines only need a single or several frames,
so we set the initial stack size to $4$ entries.
When pushing, a stack overflow check
potentially reallocates the stack, doubling its size.
In the worst case, the reallocation overhead is
$2\times$ compared to an optimally sized stack.

{
\setlength{\intextsep}{-5pt}
\begin{wrapfigure}[9]{R}[0pt]{0.4\textwidth}
\begin{minipage}{0.4\textwidth}
\begin{lstlisting}[caption={Coroutine instance class},language=scala,label=list:instance-class,captionpos=t]
class Instance[Y, R] {
  var _live = true
  var _call = false
  var _value: Y = null
  var _result: R = null
  var _exception:
    Exception = null
  /* Call stack arrays */
}
\end{lstlisting}
\end{minipage}
\end{wrapfigure}
\paratitle{Coroutine instance class}
A coroutine instance is represented by the \texttt{Instance} class
shown in Listing \ref{list:instance-class}.
A new instance is created by the \texttt{start} method.
In addition to the call stack,
a coroutine instance tracks
if the instance is live (i.e. non-terminated),
if a nested call is in progress,
what the last yield value was,
the result value (if the instance terminated),
and the exception that was thrown (if any).
The coroutine instance exposes the \texttt{value},
\texttt{result} and \texttt{exception} user-facing methods,
which either return the value of the respective field,
or throw an error if the field is not set.
The instance also exposes the \texttt{resume} method,
which is described shortly.

}

\paratitle{Coroutine class}
For each \texttt{coroutine} declaration in the program,
the transformation macro generates a new anonymous subclass
of the \texttt{Coroutine} class shown in Listing \ref{list:coroutine-class}.

{
\setlength{\intextsep}{-5pt}
\begin{wrapfigure}[9]{L}[0pt]{0.55\textwidth}
\begin{minipage}{0.55\textwidth}
\begin{lstlisting}[caption={Coroutine definition base classes},language=scala,label=list:coroutine-class,captionpos=t]
class Coroutine[Y, R] {
  def _enter(i: Instance[Y, R]): Unit
}
class Coroutine1[T0, Y, R]
extends Coroutine[Y, R] {
  def _call(
    i: Instance[Y, R], a0: T0): Unit
}
/* One class for each arity */
\end{lstlisting}
\end{minipage}
\end{wrapfigure}
\noindent
Each concrete \texttt{Coroutine} subclass
defines several entry point methods,
and implements the \texttt{\_enter} method of the \texttt{Coroutine} base class.
An \emph{entry point method} is a replica of the \texttt{coroutine} block
such that it starts from either:
\begin{enumerate*}[label=(\arabic{*}),itemsep=0mm]
\item
the beginning of the method, or
\item
a \texttt{yieldval} statement, or
\item
a call to another coroutine.
\end{enumerate*}
The \texttt{\_enter} method is called when a coroutine instance resumes.
It reads the current position from the coroutine instance,
and dispatches to the proper entry point method
with a \texttt{switch} statement.
A \texttt{goto} primitive is unavailable in Scala,
so the \texttt{\_enter} method emulates the \texttt{goto} semantics.

\setlength{\intextsep}{-16pt}
\begin{wrapfigure}[11]{R}[0pt]{0.4\textwidth}
\begin{minipage}{1\textwidth}
\begin{lstlisting}[caption={The \texttt{resume} trampoline},language=scala,label=list:resume-implementation,captionpos=t]
def resume[Y, R](i: Instance[Y, R]) = {
  if (!i._live) throw sys.error()
  i._hasValue = false
  i._value = null

  do { i._cstack(i._ctop)`\label{code:trampoline-start}`._enter(i) }
  while (i._call)`\label{code:trampoline-end}`

  i._live
}
\end{lstlisting}
\end{minipage}
\end{wrapfigure}
Listing \ref{list:coroutine-class} also shows
the abstract \texttt{Coroutine1} subclass.
The \texttt{Coroutine1} subclass declares the \texttt{\_call} method
which stores the resume-site or callsite arguments
into the proper locations in the call stack.
This method is invoked by \texttt{start} and by coroutine calls.
Neither JVM nor Scala support variadic templates,
so we include $4$ different arity classes
(the same approach is used for \texttt{Function} classes in Scala,
and functional interface classes in Java).

}

{
\paratitle{Trampolining}
An entry point method ends at a position
at which the original \texttt{coroutine} block has
a \texttt{yieldval},
a coroutine call,
or a return.
Therefore, each entry point method
in the \texttt{Coroutine} class is tail-recursive.
Consequently, nested coroutine calls
can be invoked from a trampoline-style loop.

The \texttt{resume} method in Listing \ref{list:resume-implementation}
implements a trampoline
in lines \ref{code:trampoline-start}-\ref{code:trampoline-end}.
After resetting the yield-related fields,
\texttt{resume} repetitively reads the topmost coroutine
from the coroutine stack \texttt{\_cstack},
and invokes \texttt{\_enter}.
If an entry point calls another coroutine, or returns from a coroutine call,
the \texttt{\_call} field is set to \texttt{true}.
Otherwise, if an entry point yields or stops the instance,
the \texttt{\_call} field is set to \texttt{false},
and the loop terminates.

}


\subsection{Transformation}\label{sec:transformation-implementation}

The transformation is performed by
the following \texttt{coroutine} macro,
which takes a Scala AST, typed \texttt{c.Tree}.
The \texttt{coroutine} macro checks that the AST is statically a function type,
and reports a compiler error otherwise.
The macro returns an AST that holds a definition
of an anonymous \texttt{CoroutineN} subclass (for a specific arity \texttt{N}),
and a new instance of that class.

\begin{lstlisting}[
  language=scala,
  label=list:hash-bucket-canonical,
  captionpos=t,
  abovecaptionskip=-\medskipamount
]
def coroutine[T, R](f: Any): Any = macro coroutine_impl[T, R]
def coroutine_impl[T, R](c: Context)(f: c.Tree): c.Tree =
  /* Implementation of the macro */
\end{lstlisting}

The transformation consists of four compilation phases.
First, the input AST is converted into a normal form.
Second, the normalized AST is converted into a control flow graph.
Third, the control flow graph is cut into segments at the points
where the coroutine yields or calls other coroutines.
Finally, control flow graph segments are converted back to ASTs,
which represent the coroutine's entry points
and are used to generate the anonymous class.

{
\setlength{\intextsep}{0pt}
\begin{wrapfigure}[11]{R}[0pt]{0.45\textwidth}
\begin{minipage}{0.45\textwidth}
\begin{lstlisting}[
  caption={Canonicalized list coroutine},
  language=scala,
  label=list:hash-bucket-canonical,
  captionpos=t,
  abovecaptionskip=-\medskipamount
]
val bucket = coroutine {
  (b: List[Int]) =>
  var x_0 = b != Nil
  var x_1 = x_0
  while (x_1) {
    var x_2 = b.head
    var x_3 = yieldval(x_2)
    var x_4 = b.tail
    b = x_4
    var x_0 = b != Nil
    x_1 = x_0 }
  () }
\end{lstlisting}
\end{minipage}
\end{wrapfigure}
\paratitle{AST normalization}
This phase converts the input AST with arbitrary phrases
into a normalized AST.
The phrases in the normalized AST are restricted to:
\begin{enumerate*}[label=(\arabic{*}),itemsep=0mm]
\item
single operator expressions on constants and identifiers,
\item
assignments and declarations whose right-hand side
is a constant or an identifier\footnote{
We sometimes slightly deviate from this in the examples,
for better readability.
},
\item
method calls on constants and identifiers,
\item
\texttt{if}-statements and \texttt{while}-loops
whose condition is a constant or an identifier
and whose body is normalized,
\item
basic blocks whose statements are normalized.
\end{enumerate*}
The benefit of normalization
is that the subsequent phases have fewer cases to consider.

\paratitle{Example}
Recall the \texttt{bucket} coroutine from Listing \ref{list:hash-bucket},
which yields the elements of a list.
After normalization, this coroutine is transformed
into the coroutine in Listing \ref{list:hash-bucket-canonical}.

}

\tikzstyle{cfg}=[draw,circle,fill=white,inner sep=0,minimum size=11pt]
\tikzstyle{ptr}=[densely dotted]
\tikzstyle{edg}=[]

{
\setlength{\intextsep}{2pt}
\begin{wrapfigure}{L}[0pt]{0.30\textwidth}
\begin{minipage}{0.30\textwidth}
\small
\begin{tikzpicture}
  \node()    at (-2.10, -0.25) []    {$\texttt{var x=t} \rightarrow$};
  \node(yn)  at ( 0.00,  0.00) [cfg] {};
  \node      at ( 0.00, -0.45) []    {$\texttt{var x=t}$};
  \node(ynl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(ynr) at ( 0.90, -0.15) []    {\scriptsize{$last$}};
  %
  \draw[-stealth,ptr] (ynl) -- (yn);
  \draw[-stealth,ptr] (ynr) -- (yn);
\end{tikzpicture}
\end{minipage}
\end{wrapfigure}
\noindent
\paratitle{Control flow graph conversion}
A normalized AST is converted to a control flow graph.
The transformation is implemented as a set of mappings
between the input AST and the output CFG nodes.
An example rule
for a variable declaration is informally shown above on the left,
where a declaration is replaced by a single node that records the AST.

\setlength{\intextsep}{0pt}
\begin{wrapfigure}{R}[0pt]{0.40\textwidth}
\begin{minipage}{0.40\textwidth}
\small
\infrule[]
{ \raisebox{-5pt}{
  \begin{tikzpicture}
  \node()    at (-2.80,  0.00) []    {$\texttt{t} = \texttt{while (t}_c\texttt{) t}_b$};
  \node()    at (-0.60,  0.00) []    {$\texttt{t}_b \rightarrow$};
  \node(tn1) at ( 0.00,  0.00) [cfg] {\scriptsize{1}};
  \node(tn2) at ( 1.00,  0.00) [cfg] {\scriptsize{2}};
  \path[-,dashed] (tn1.north east) edge[bend left=+30] (tn2.north west);
  \path[-,dashed] (tn1.south east) edge[bend left=-30] (tn2.south west);
  \end{tikzpicture}
  }
}
{ \begin{tikzpicture}
  \node()    at (-1.60, -0.25) []    {$\texttt{t} \rightarrow$};
  \node(wn1) at ( 0.00,  0.00) [cfg] {\scriptsize{Ws}};
  \node      at ( 0.00, -0.45) []    {$\texttt{t}_c$};
  \node(wnl) at (-0.90, -0.15) []    {\scriptsize{$head$}};
  \node(wn2) at ( 2.50,  0.00) [cfg] {\scriptsize{We}};
  \node      at ( 2.50, -0.45) []    {$\varnothing$};
  \node(wnr) at ( 3.40, -0.15) []    {\scriptsize{$last$}};
  %
  \node(bn1) at ( 0.75,  0.00) [cfg] {\scriptsize{1}};
  \node(bn2) at ( 1.75,  0.00) [cfg] {\scriptsize{2}};
  \path[-,dashed] (bn1.north east) edge[bend left=+30] (bn2.north west);
  \path[-,dashed] (bn1.south east) edge[bend left=-30] (bn2.south west);
  %
  \draw[-stealth,edg] (wn1) -- (bn1);
  \draw[-stealth,edg] (bn2) -- (wn2);
  \path[-stealth,edg] (wn1.north east) edge[bend left=+30] (wn2.north west);
  \path[-stealth,edg] (wn2.south west) edge[bend left=+30] (wn1.south east);
  %
  \draw[-stealth,ptr] (wnl) -- (wn1);
  \draw[-stealth,ptr] (wnr) -- (wn2);
  \end{tikzpicture}
}
\end{minipage}
\end{wrapfigure}
The rule for \texttt{while}-loops, informally shown on the right,
relies on the recursive transformation of the body $\texttt{t}_b$ of the loop.
Given that $\texttt{t}_b$ transforms to a CFG
that starts with a node $1$ and ends with a node $2$,
a \texttt{while}-loop transforms to a pair of
\textsl{Ws} and \textsl{We} nodes,
which are connected with successor links (solid lines)
as shown in the figure.

}

\paratitle{Example}
Recall once more the \texttt{bucket} coroutine from Listing \ref{list:hash-bucket}.
The resulting control flow graph is shown below.
Nodes that do not represent structured control flow or yielding
are annotated with the line number from Listing \ref{list:hash-bucket-canonical},
and the $Y$ node represents the yield-site.
\\*

{
\centering
\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{3}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{4}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{Ws}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{6}};
\draw[-stealth,edg] (n2) -- (n3);
\node(n4)    at ( 3.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (n3) -- (n4);
\node(n5)    at ( 3.75,  0.00) [cfg] {\scriptsize{8}};
\draw[-stealth,edg] (n4) -- (n5);
\node(n6)    at ( 4.50,  0.00) [cfg] {\scriptsize{9}};
\draw[-stealth,edg] (n5) -- (n6);
\node(n7)    at ( 5.25,  0.00) [cfg] {\scriptsize{10}};
\draw[-stealth,edg] (n6) -- (n7);
\node(n8)    at ( 6.00,  0.00) [cfg] {\scriptsize{11}};
\draw[-stealth,edg] (n7) -- (n8);
\node(n9)    at ( 6.75,  0.00) [cfg] {\scriptsize{We}};
\draw[-stealth,edg] (n8) -- (n9);
\node(n10)   at ( 7.50,  0.00) [cfg] {\scriptsize{12}};
\draw[-stealth,edg] (n9) -- (n10);
\node(ret)   at ( 8.40, -0.00) []    {\scriptsize{$return$}};
\draw[-stealth,edg] (n10) -- (ret);
\path[-stealth,edg] (n2.north east) edge[bend left=+15] (n9.north west);
\path[-stealth,edg] (n9.south west) edge[bend left=+15] (n2.south east);
%
\end{tikzpicture}

}

\paratitle{Control flow graph splitting}
Resuming a coroutine effectively jumps to the middle of its body.
Such a jump is not possible if the target language
that supports only structured programming constructs.
As explained in Section \ref{sec:data-model},
the transformation outputs multiple entry point subroutines,
each containing only structured control flow.
Therefore, the CFG from the previous phase
is split into multiple segments, each corresponding to an entry point.

The splitting starts at the node that corresponds to the coroutine method entry,
and traverses the nodes of the graph until reaching a previously unseen
yield-site or coroutine call.
The search is repeated from each split, taking care not to repeat the search twice.
If the graph traversal encounters a control flow node (such as \textsl{We})
whose corresponding \textsl{Ws} node was not seen as part of the same segment
(which can happen if there is a yield inside a \texttt{while}-loop),
such a node is converted into a \textsl{Be} (block exit) node,
followed by a loop again.

{
\centering
\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{3}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{4}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{Ws}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{6}};
\draw[-stealth,edg] (n2) -- (n3);
\node(n4)    at ( 3.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (n3) -- (n4);
\node(n9)    at ( 4.75,  0.00) [cfg] {\scriptsize{We}};
\node(n10)   at ( 5.50,  0.00) [cfg] {\scriptsize{12}};
\draw[-stealth,edg] (n9) -- (n10);
\node(ret)   at ( 6.40, -0.00) []    {\scriptsize{$return$}};
\draw[-stealth,edg] (n10) -- (ret);
\path[-stealth,edg] (n2.north east) edge[bend left=+20] (n9.north west);
\path[-stealth,edg] (n9.south west) edge[bend left=+20] (n2.south east);
%
\end{tikzpicture}

\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{Bs}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{8}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{9}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{10}};
\draw[-stealth,edg] (n2) -- (n3);
\node(n4)    at ( 3.00,  0.00) [cfg] {\scriptsize{11}};
\draw[-stealth,edg] (n3) -- (n4);
\node(n5)    at ( 3.75,  0.00) [cfg] {\scriptsize{Be}};
\draw[-stealth,edg] (n4) -- (n5);
\node(n6)    at ( 4.50,  0.00) [cfg] {\scriptsize{Ws}};
\draw[-stealth,edg] (n5) -- (n6);
\node(n7)    at ( 5.25,  0.00) [cfg] {\scriptsize{6}};
\draw[-stealth,edg] (n6) -- (n7);
\node(n8)    at ( 6.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (n7) -- (n8);
\node(n9)    at ( 6.75,  0.00) [cfg] {\scriptsize{We}};
\node(n10)   at ( 7.50,  0.00) [cfg] {\scriptsize{12}};
\draw[-stealth,edg] (n9) -- (n10);
\node(ret)   at ( 8.40, -0.00) []    {\scriptsize{$return$}};
\draw[-stealth,edg] (n10) -- (ret);
\path[-stealth,edg] (n6.north east) edge[bend left=+20] (n9.north west);
\path[-stealth,edg] (n9.south west) edge[bend left=+20] (n6.south east);
%
\end{tikzpicture}

}

\paratitle{Example}
The control flow graph of the
\texttt{bucket} coroutine from Listing \ref{list:hash-bucket},
produced in the previous phase,
is split into the following pair of segments.
Note that the second segment starts from the yield-site inside the loop,
and that one loop iteration is effectively unrolled.

\begin{multicols}{2}
\begin{lstlisting}[caption={Entry points of \texttt{bucket}},language=scala,label=list:hash-bucket-ep0,captionpos=t,abovecaptionskip=-\medskipamount]
def _enter(
  i: Instance[Int, Unit]
): Unit =
  i._pstack(i._ptop) match {
    case 0 => _ep0(i)
    case 1 => _ep1(i)
  }

def _ep0(
  i: Instance[Int, Unit]
): Unit = {
  var b = i._rstack(i._rtop + 0)
  var x_0 = b != Nil
  var x_1 = x_0
  while (x_1) {
    var x_2 = b.head
    i.value = x_2
    i._pstack(i._ptop + 0) = 1
    return
  }
  i._result = ()
  i._cstack(i._ctop) = null
  i._ctop -= 1
  i._ptop -= 1 }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Entry points of \texttt{bucket}, cont.},language=scala,label=list:hash-bucket-ep1,captionpos=t,showlines=true]
def _ep1(
  i: Instance[Int, Unit]
): Unit = {
  var b = i._rstack(i._rtop + 0)
  var x_1 = false
  {
    var x_3 = ()
    var x_4 = b.tail
    b = x_4
    var x_0 = b != Nil
    x_1 = x_0
  }

  while (x_1) {
    var x_2 = b.head
    i.value = x_2
    i._rstack(i._rtop + 0) = b
    i._pstack(i._ptop + 0) = 1
    return
  }
  i._result = ()
  i._cstack(i._ctop) = null
  i._ctop -= 1
  i._ptop -= 1 }
\end{lstlisting}
\end{multicols}

\paratitle{AST generation}
This phase transforms the CFG segments
back into the ASTs for the entry point methods.
Each entry point starts by restoring the local variables from the call stack.
At each yield-site and each coroutine call (commonly, the exit),
the entry point method stores the local variables back to the stack.
It then either stores the yield value into the coroutine,
or stores the result value.
The entry point methods are placed into a \texttt{Coroutine} subclass,
and the \texttt{\_enter} method dispatches to the proper entry points.

\paratitle{Example}
Listings \ref{list:hash-bucket-ep0} and \ref{list:hash-bucket-ep1}
show the implementation of the entry points of the \texttt{bucket} coroutine.
Note that each method starts by restoring the local variable \texttt{b}
from the reference stack of the coroutine instance \texttt{i}.
Each entry point ends by either storing the yield value
into the \texttt{value} field of the coroutine instance,
or the result value into the \texttt{result} field.
Local variables are then stored onto the stack
(there are two stacks -- \texttt{\_vstack} for primitive values
and \texttt{\_rstack} for references),
and the program counter is stored to the \texttt{\_pstack}.

\begin{figure}
\begin{multicols}{2}
\begin{lstlisting}[
  caption={Error-handling coroutines},
  language=scala,
  label=list:exception-handling-coroutines,
  captionpos=t,
  abovecaptionskip=-\medskipamount
]
val fail =
  coroutine { (e: Error) =>
    throw e
  }
val forward =
  coroutine { () =>
    fail(new Error)
  }
val main =
  coroutine { () =>
    try forward()
    catch {
      case e: Error =>
        println("Failed.")
    }
  }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[
  caption={Normalized \texttt{main} coroutine},
  language=scala,
  label=list:exception-normalized-main,
  captionpos=t,
  showlines=true
]
/* main */
var x_0: Exception = null
try forward()
catch {
  case e => x_0 = e
}
var x_1 = x_0 != null
if (x_1) {
  var x_2 =
    x_0.isInstanceOf[Error]
  if (x_2) {
    println("Failed.")
  } else {
    throw x_0
  }
}
\end{lstlisting}
\end{multicols}
\end{figure}


\subsection{Exception handling}

Code inside the \texttt{coroutine} block can throw an exception.
In this case, standard exception handling semantics apply --
the control flow must continue from
the nearest dynamically enclosing \texttt{catch} block
that handles the respective exception type.
To ensure this, the transformation does three things:
\begin{enumerate*}[label=(\arabic{*}),itemsep=0mm]
\item
it normalizes the \texttt{try}-\texttt{catch} and \texttt{throw} ASTs,
\item
it treats each \texttt{throw} statement as a suspension point
that writes to the instance's \texttt{\_exception} field,
\item
it places an exception handler at the beginning of each entry point.
\end{enumerate*}

To explain these steps,
we use the example in Listing \ref{list:exception-handling-coroutines}.
The \texttt{fail} coroutine takes an \texttt{Error} argument and throws it.
The \texttt{forward} coroutine creates an \texttt{Error} object,
and calls the \texttt{fail} coroutine
without handling its exceptions.
The \texttt{main} coroutine calls the \texttt{forward} coroutine
inside a \texttt{try} block,
and catches the subset of exceptions with the \texttt{Error} type.

\paratitle{Normalization}
The normalized coroutine \texttt{main}
is shown in Listing \ref{list:exception-normalized-main}.
The \texttt{catch} handler is transformed so that, once caught,
the exception is immediately stored into \texttt{x\_0}.
The variable \texttt{x\_0}
is matched against the \texttt{Error} type
in the subsequent \texttt{if}-statements.

\paratitle{Exception throws}
The transformation of the \texttt{throw} statement
from the \texttt{fail} coroutine
is in Listing \ref{list:exception-entry-point-fail}.
The parameter is loaded into the variable \texttt{e},
and immediately stored into the \texttt{exception} field.
The coroutine stack \texttt{\_cstack} is then popped,
and the coroutine returns.

\paratitle{Stack unwinding}
The final rule is to wrap every entry point
that starts at a return from a coroutine call
into an \emph{unwinding exception handler}.
In addition, if the previous entry point ended
inside a \emph{user exception handler},
then a replica of that handler is added.

The \texttt{forward} coroutine does not have an exception handler,
so its second entry point \texttt{\_ep1}
contains only the \emph{unwinding} handler,
as shown in Listing \ref{list:exception-entry-point-forward}.
On the other hand,
\texttt{main}'s first entry point \texttt{\_ep0}
ends with a coroutine call.
Listing \ref{list:exception-entry-point-main} shows that
the second entry point \texttt{\_ep1}
therefore has both the \emph{unwinding} handler
and the \emph{user} handler.
If the user handler cannot handle the exception,
then the exception is rethrown.

\begin{multicols}{2}
\begin{lstlisting}[
  caption={1st entry point of \texttt{fail}},
  language=scala,
  label=list:exception-entry-point-fail,
  captionpos=t,
  showlines=true
]
/* fail, _ep0 */
var e = i._rstack(i._rtop)
i._exception = e
i._rstack(i._rtop) = null
i._rtop -= 1
return
\end{lstlisting}
\vspace{-3mm}
\begin{lstlisting}[
  caption={2nd entry point of \texttt{main}},
  language=scala,
  label=list:exception-entry-point-main,
  captionpos=t,
  showlines=true
]
/* main, _ep1 */
try {
  try {
    var x_0 = i._exception
    if (x_0 != null) throw x_0
  } catch { case e => x_0 = e }
  var x_1 = x_0 != null
  if (x_1) {
    var x_2 =
      x_0.isInstanceOf[Error]
    if (x_2) println("Failed.")
    else throw x_0
  }
  /* Normal exit */
} catch { case x_1 =>
  /* Exceptional exit */
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[
  caption={Entry points of \texttt{forward}},
  language=scala,
  label=list:exception-entry-point-forward,
  captionpos=t,
  showlines=true
]
/* forward, _ep0 */
var x_0 = new Error
fail._call(i, x_0)
i._ctop += 1
i._cstack(i._ctop) = null
i._ptop += 1
i._pstack(i._ptop) = 0
i._call = true
return

/* forward, _ep1 */
try {
  var x_0 = i._exception
  if (x_0 != null) throw x_0
  i._cstack(i._ctop) = null
  i._ctop -= 1
  i._ptop -= 1
  return
} catch { case x_1 =>
  i._exception = x_1
  i._cstack(i._ctop) = null
  i._ctop -= 1
  i._ptop -= 1
  return
}

\end{lstlisting}
\end{multicols}


\subsection{Optimizations}\label{sec:optimizations}

An entry point method does not need to
load all the local variables at the beginning,
nor store all of them to the stack.
For example, the entry points of the \texttt{bucket} coroutine
in Listings \ref{list:hash-bucket-ep0} and \ref{list:hash-bucket-ep1}
only store a subset of all the variables in the scope.
In particular, \texttt{\_ep0} does not store the variables
\texttt{b}, \texttt{x\_0}, \texttt{x\_1} and \texttt{x\_2},
while \texttt{\_ep1} only stores \texttt{b}.
In this section, we explain the optimization rules
used to avoid the unnecessary loads and stores.

\paratitle{Scope rule}
A variable does not need to be loaded or stored
if it is not in scope after the exit point.
This rule applies to, for example,
the variables \texttt{x\_3} and \texttt{x\_4} from Listing \ref{list:hash-bucket-ep1}.

\begin{definition}
A control flow graph node $d$ dominates a node $n$
if every control flow path from the begin node to $n$ must go through $d$.
\qed
\end{definition}

\paratitle{Must-load rule}
A local variable \texttt{v} must be loaded from the stack
if the respective entry point contains at least one read of \texttt{v}
that is not dominated by a write of \texttt{v}.

{
\setlength{\intextsep}{0pt}
\begin{wrapfigure}{R}[0pt]{0.36\textwidth}
\begin{minipage}{0.36\textwidth}
\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{Bs}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{8}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{9}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{10}};
\draw[-stealth,edg] (n2) -- (n3);
\node(ret)   at ( 3.30, -0.00) []    {\scriptsize{$\ldots$}};
\draw[-stealth,edg] (n3) -- (ret);
%
\end{tikzpicture}
\end{minipage}
\end{wrapfigure}
\paratitle{Example}
Consider the variable \texttt{b} of the entry point \texttt{\_ep1}
of the \texttt{bucket} coroutine in Listing \ref{list:hash-bucket-ep1}.
In the corresponding control flow graph,
the read in the node $8$ precedes the write in the node $9$.
Consequently, there exists a read that is not dominated by any write,
and \texttt{b} must be loaded.

}

\begin{definition}
A control flow path is a connected sequence of CFG nodes.
A control flow path is \emph{\m{v}-live}
if the variable \m{v} is in scope in all the nodes of that control flow path.
\end{definition}

\paratitle{Was-changed rule}
A local variable \texttt{v} must not be stored to the stack
if there is no \texttt{v}-live control flow path that starts with a write to \texttt{v}
and ends at the respective exit node.

{
\setlength{\intextsep}{0pt}
\begin{wrapfigure}{L}[0pt]{0.38\textwidth}
\begin{minipage}{0.38\textwidth}
\begin{tikzpicture}
\node(entry) at (-0.90, -0.00) []    {\scriptsize{$entry$}};
\node(n0)    at ( 0.00,  0.00) [cfg] {\scriptsize{3}};
\draw[-stealth,edg] (entry) -- (n0);
\node(n1)    at ( 0.75,  0.00) [cfg] {\scriptsize{4}};
\draw[-stealth,edg] (n0) -- (n1);
\node(n2)    at ( 1.50,  0.00) [cfg] {\scriptsize{Ws}};
\draw[-stealth,edg] (n1) -- (n2);
\node(n3)    at ( 2.25,  0.00) [cfg] {\scriptsize{6}};
\draw[-stealth,edg] (n2) -- (n3);
\node(n4)    at ( 3.00,  0.00) [cfg] {\scriptsize{Y}};
\draw[-stealth,edg] (n3) -- (n4);
\node(n9)    at ( 3.75,  0.00) [minimum height=7mm] {};
\path[-...,edg] (n2.north east) edge[bend left=+20] (n9.north west);
\path[...-stealth,edg] (n9.south west) edge[bend left=+20] (n2.south east);
%
\end{tikzpicture}
\end{minipage}
\end{wrapfigure}
\paratitle{Example}
Consider the variable \texttt{b} of the entry point \texttt{\_ep0}
of the \texttt{bucket} coroutine in Listing \ref{list:hash-bucket-ep0}.
In the corresponding CFG,
the variable \texttt{b} is read in nodes $3$ and $6$.
However, there is no write to \texttt{v}
that connects to the exit node $Y$.
Therefore, at $Y$,
\texttt{b} did not change its value since the begin node,
so it does not have to be stored.

}

\begin{definition}
We say that an exit node $x$ \emph{resumes} at an entry point $e$,
if the exit node corresponds to the begin node of $e$
in the original control flow graph.
\qed
\end{definition}

\begin{definition}
Relation $needed(x, \texttt{v}, e)$
between an exit node $x$, the variable \texttt{v} and an entry point method $e$
holds if and only if either:
\begin{enumerate*}[label=(\arabic{*}),itemsep=0mm]
\item
$x$ resumes at $e$, and the must-load rule applies to \texttt{v} and $e$,
or
\item
$x$ resumes at $e'$,
and there is a \texttt{v}-live control flow path between the begin node of $e'$
and some exit node $x'$ of $e'$,
such that $needed(x', \texttt{v}, e)$.
\end{enumerate*}
\qed
\end{definition}

\paratitle{Is-needed rule}
A local variable \texttt{v}
must not be stored to the stack at an exit node $x$
if there is no entry point method $e$
such that $needed(x, \texttt{v}, e)$.

\paratitle{Example}
Intuitively, this rule applies when it becomes impossible
to reach (without \texttt{v} going out of scope)
an entry point that would need to load \texttt{v}.
This rule applies to the variable \texttt{x\_2}
in the entry point \texttt{\_ep1} in Listing \ref{list:hash-bucket-ep1}.
Variable \texttt{x\_2} is in scope at the exit point,
however, it does not need to be loaded when \texttt{\_ep1} is reentered,
and it goes out of scope before it is needed again.


==> introduction.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Introduction}

Asynchronous programming is becoming increasingly important,
with applications ranging from
actor systems \cite{akka,Haller:2009:SAU:1496391.1496422},
futures and network programming
\cite{Cantelon:2013:NA:2601501,SIP14},
user interfaces \cite{EPFL-REPORT-176887},
to functional stream processing
\cite{Meijer:2012:YMD:2160718.2160735}.
Traditionally, these programming models
were realized either by blocking execution threads
(which can be detrimental to performance \cite{1327913}),
or callback-style APIs
\cite{Cantelon:2013:NA:2601501,SIP14,johnson1988designing},
or with monads
\cite{Wadler:1995:MFP:647698.734146}.
However, these approaches often feel unnatural,
and the resulting programs can be hard to understand and maintain.
\textit{Coroutines} \cite{Conway:1963:DST:366663.366704}
overcome the need for blocking threads, callbacks and monads
by allowing parts of the execution to pause at arbitrary points,
and resuming that execution later.

There are generally two approaches to implement control flow constructs like coroutines:
\emph{call stack manipulation} and \emph{program transformation}.
In the first approach, the runtime is augmented with call stack introspection
or the ability to swap call stacks during the execution of the program.
We are aware of several such attempts in the context of the JVM runtime
\cite{LAMP-CONF-2007-002,Stadler:2009:LCJ:1596655.1596679},
which did not become official due to the considerable changes required by the language runtime.
In the second approach,
the compiler transforms the program that uses coroutines
into an equivalent program without coroutines.
In Scheme, a similar control flow construct \texttt{call/cc} was supported
by transforming the program into the continuation-passing style (CPS)
\cite{Sussman:1998:SIE:609145.609186}.
The CPS transform can also be selectively applied to delimited parts of the program
\cite{Asai:2017:SCT:3175493.3162069,Felleisen:1988:TPF:73560.73576,Fischer:2007:TLS:1244381.1244403,NIELSEN2001311,Rompf:2009:IFP:1631687.1596596}.
Mainstream languages like Python, C\#, JavaScript, Dart and Scala
offer suspension primitives such as generators, enumerators and async-await,
which often target specific domains.

\paratitle{Coroutines based on metaprogramming}
We explore a new transformation approach for coroutines
that relies on the static metaprogramming support of the host language
(in our case Scala),
and assumes no call stack introspection
or call stack manipulation support in the runtime
(in our case JVM).
The metaprogramming-based solution has several benefits:

\noindent
(1) The language runtime and the compiler do not need to be modified.
This puts less pressure on the language and the runtime maintainers.

\noindent
(2) Since the metaprogramming API is typically standardized,
the coroutine implementation is unaffected
by the changes in the runtime or in the compiler.

\noindent
(3) The implementation does not need to be replicated for each supported backend.
Our own implementation works with both the JVM runtime,
and the Scala.JS browser backend.

\noindent
(4) Coroutines can be encapsulated as a standalone library.
Our implementation in Scala is distributed
independently from the standard Scala distribution.

We note that our approach is not strictly limited to metaprogramming --
it can also be implemented inside the compiler.
However, to the best of our knowledge,
we are the first ones to implement and evaluate coroutines using a metaprogramming API.

\paratitle{Summary}
Our coroutine model is statically typed, stackful, and delimited.
Static typing improves program safety,
stackfulness allows better composition,
and delimitedness allows applying coroutines to selected parts of the program
(this is explained further in Section \ref{sec:prog-model}).
Regions of the program can be selectively marked as suspendable,
without modifying or recompiling existing libraries.
These regions represent first-class coroutines
that behave similar to first-class function values.
We show that the model generalizes
many existing suspendable and asynchronous programming models.
We extend this model with snapshots,
and show that the extension allows expressing backtracking and continuations.
Finally, we show that the metaprogramming approach has a reasonable performance
(at most $2.11\times$ overheads compared to equivalent manually optimized code)
by comparing it against alternative frameworks.
We also formalize coroutines with snapshots and prove standard safety properties.

\paratitle{Contributions}
The main novelties in this work are as follows:
\begin{itemize}[topsep=0pt]
\item
We show that \emph{AST-level static metaprogramming support of the host language}
is sufficient to implement first-class, typed, stackful, delimited coroutines
that are reasonably efficient.
\item
We propose a new form of coroutines, namely \emph{coroutine with snapshots},
which increases the power of coroutines.
For example, it allows emulating backtracking and continuations.
\item
We formalize stackful coroutines with snapshots in $\lambda_\leadsto$ by
extending the simply typed lambda calculus,
and we prove soundness of the calculus.
\end{itemize}
Some of the features of the proposed model,
such as the typed coroutines and first-class composability,
have been explored before in various forms
\cite{yield-mainstream,Moura:2009:RC:1462166.1462167,Fischer:2007:TLS:1244381.1244403,Felleisen:1988:TPF:73560.73576}.
We build on earlier work, and we do not claim novelty for those features.
However, to the best of our knowledge,
the precise model that we describe is new,
as we argue in Section \ref{sec:related} on related work.

\paratitle{Structure and organization}
This paper is organized as follows:
\begin{itemize}[topsep=0pt]
\item
Section \ref{sec:prog-model}
describes the core primitives of the proposed programming model --
coroutine definitions, coroutine instances,
yielding, resuming, coroutine calls, and snapshots.
\item
Section \ref{sec:use-cases}
presents use-cases such as Erlang-style actors \cite{programming-erlang96},
async-await \cite{scala-async},
Oz-style variables \cite{VanRoy:2004:CTM:983087},
event streams \cite{EPFL-CONF-188383,Meijer:2012:YMD:2160718.2160735},
backtracking \cite{scalacheck},
and delimited continuations \cite{Rompf:2009:IFP:1631687.1596596}.
\item
In Section \ref{sec:formal},
we formalize coroutines with snapshots in $\lambda_\leadsto$ and prove its soundness.
\item
In Section \ref{sec:implementation},
we describe the AST-level coroutine transformation
implemented in Scala.
\item
In Section \ref{sec:eval},
we experimentally compare the performance of our implementation
against Scala Delimited Continuations, Scala Async,
iterators, and lazy streams.
\end{itemize}

\vspace{2mm}
\paratitle{Syntax}
Our examples throughout this paper
are in the Scala programming language \cite{200464/IC}.
We took care to make the paper accessible to a wide audience
by using a minimal set of Scala features.
The \texttt{def} keyword declares a method,
while \texttt{var} and \texttt{val}
declare mutable and final variables, respectively.
Lambdas are declared with the right-arrow symbol \texttt{=>}.
Type annotations go after the variable name, colon-delimited (\texttt{:}).
Type parameters are put into square brackets \texttt{[]}.
Parenthesis can be omitted from nullary and unary method calls.
% The \texttt{Unit} type is the equivalent of \texttt{void}.


==> new-typing-rules.tex <==
\begin{minipage}[t]{5cm}
\small
\infrule[\textsc{T-Sub}]
{ \Sigma | \Gamma \vdash \texttt{t:S} | \texttt{T}_y \quad \texttt{S<:T}
}
{ \Sigma | \Gamma \vdash \texttt{t:T} | \texttt{T}_y
}
\noindent
\end{minipage}
\begin{minipage}[t]{5cm}
\small
\infrule[\textsc{T-Ctx}]
{ \Sigma | \Gamma \vdash \texttt{t:T} | \texttt{T}_y
}
{ \Sigma | \Gamma \vdash \texttt{t:T} | \texttt{T}_y \sqcup \texttt{T}_w
}
\noindent
\end{minipage}


==> old-implementation.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Implementation}
\label{sec:implementation}

Our implementation is done in Scala,
whose intermediate format has a richer set of ASTs compared to $\lambda_\leadsto$.
While the calculus is interesting
for the purpose of studying the transformation formally,
we have found it inconvenient to map Scala ASTs to $\lambda_\leadsto$,
and then map the transformed code back to Scala.
We describe the concrete implementation briefly in this section,
and in more detail in Section \ref{sec:implementation-details} of the appendix.

The implementation consists of several phases.
First, the AST is converted to a canonical form
that simplifies subsequent transformations.
Second, the canonical AST is converted into a control flow graph.
Third, the control flow graph is cut into segments at the points
where the coroutine yields or directly calls other coroutines.
Fourth, control flow graph segments
are converted back to ASTs, which generate the coroutine's entry points.

\input{phases.tex}


\subsection{Data Model}\label{sec:main-data-model}

Each coroutine frame, similar to a method invocation frame,
must store the following:
pointer to the coroutine descriptor,
the program counter,
and the local variables.
As explained in Section \ref{sec:prog-model}, coroutines allow direct calls.
Consequently, a coroutine instance has a call stack of coroutine frames.
Some alternative approaches, such as continuations based on the CPS transform,
encode calls as a chain of function objects.
We deliberately avoid the object chaining approach, since it is less efficient,
as we show in Section \ref{sec:eval}.

A coroutine call stack can generally be implemented as a single contiguous memory area.
%Our implementation targets Scala, historically constrained by the JVM platform,
%which allows arrays that contain either references or primitive values, but not both.
%For this reason,
%our implementation separates coroutine descriptors, program counters,
%local references and local primitive values into separate stacks.
Creating large call stacks when a coroutine instance starts is costly.
To prevent wasting processing time when
the instance only needs a single or several frames,
the initial size of the stacks is set to $4$ entries.
If a stack push detects an overflow,
a new stack is allocated, its size doubled and old entries copied.
%The total work done in push and pop operations is in the worst case
%$2\times$ larger compared to an optimally sized stack.
%This worst-case is rarely seen in practice,
%since most programs have call trees with the average branching factor
%greater than $1$ -- allocated stack space is usually used more than once.
Besides one or more call stacks,
a coroutine instance contains
the last yield value, the result value (if terminated),
and an optionally thrown exception.


\subsection{AST Canonicalization}

In this phase,
the AST consisting of typical language node types
gets converted into a restricted form:
single operator expressions,
assignments, declarations, method calls,
\texttt{if}-statements and \texttt{while}-loops.
The advantage is that
subsequent phases have fewer cases to consider,
conversion back to ASTs is easier,
and optimizations that analyze data dependencies are less complex.
% As a design decision, we use restricted forms of control constructs
% (e.g. \texttt{if}-statements and \texttt{while}-loops)
% in the canonicalized form instead of transforming them
% into the minimal representation from Section \ref{sec:formal} --
% a representation consisting solely of coroutine applications
% would degrade performance, or otherwise require intricate optimizations.


\subsection{Control Flow Graph Conversion}

In this phase, the AST is converted to a control-flow graph.
A single recursive pass over the AST converts each canonicalized form
into a subgraph, and recursively binds those subgraphs together.
A \emph{scope},
which contains the current list of basic blocks and variables in those blocks,
is assigned to each CFG node.
The scope is used to restore the local variables when reconstructing the AST.


\subsection{Control Flow Graph Splitting}\label{sec:cfg-split}

The CFG produced in the previous phase
is split at the nodes that correspond to yield-sites
into a set of \emph{segments}.
The splitting algorithm starts at the node that corresponds
to the coroutine method entry,
and traverses the nodes of the graph until reaching a previously unseen yield-site.
The yield-site is then added to the work-list,
and the process is repeated until the work-list becomes empty.


\subsection{AST Generation}\label{sec:ast-gen}

Segments of the original CFG are used to produce multiple coroutine entry points.
The first entry point starts at the entry of the original method,
and the remaining entry points start at the yield points.
Each entry point first restores the local variables the stack,
and ends by storing them back to the stack.
These entry point methods are placed into a common Scala class.
A separate \texttt{entry} method is added,
which switches on the current program counter of the coroutine instance,
and dispatches to the proper entry point method.


\subsection{Optimizations}\label{sec:optimizations}

Our approach,
as opposed to the formal transformation from Section \ref{sec:formal-transformation},
avoids the need for optimizing away the CPS function applications.
Furthermore,
the translation back to ASTs
benefits from reusing the host language optimizations.
Still, most compilers do not optimize code across different entry point methods.
One large overhead is that
entry points must load the local variables in the initial block,
and yield points must store the variables in scope.
These loads and stores have high overheads.
For this reason,
we define a $mustLoad$ relation
that states that a variable must be loaded in a CFG segment
only if it is read in that block before being assigned.
We similarly define a $wasChanged$ relation
to store only those variables that the CFG segment mutated.
Finally,
the variable is not stored at an exit point
if the subsequent CFG segments never read it,
which is defined by the $isNeeded$ relation.
All three relations are implemented as straightforward CFG traversals.


==> old-introduction.tex <==

\section{Introduction}

As concurrent and distributed computing grow in popularity,
so does the need for more expressive control structures.
The asynchronous nature of these computations
necessitates frequent use of callbacks and inversion of control
\cite{akka} \cite{Cantelon:2013:NA:2601501}
\cite{SIP14} \cite{EPFL-REPORT-176887} \cite{Meijer:2012:YMD:2160718.2160735}.
In addition to reacting to asynchronous inputs from their environment,
computations must suspend and migrate between mobile devices and data centers,
be persisted and rerun later,
or be replicated across multiple locations.

% Being able to suspend a computation and have it resumed later
% has multiple benefits in this context.
% Suspended computations can be reactivated after
% their inputs arrive or specific conditions are met;
% or they can be sent across the wire,
% persisted and stored into the database,
% and reinstantiated many times to improve robustness or throughput.
Traditionally, these requirements were met
either by blocking execution threads
(which can be detrimental to performance \cite{1327913}),
or with inversion of control and callback-style APIs
\cite{Cantelon:2013:NA:2601501} \cite{SIP14} \cite{johnson1988designing}
in object-oriented programming,
or with monads in functional programming \cite{Wadler:1995:MFP:647698.734146}.
However, these approaches feel unnatural for many programmers,
and result in programs that are hard to understand and follow.
\textit{Coroutines} \cite{Conway:1963:DST:366663.366704}
overcome the need for
blocking, inversion of control, callbacks and monads
by allowing the execution to pause at the desired points.

Despite the increasing demand,
most mainstream programming languages do not offer
general support for suspending computations.
When support does exist, it is often tailored for specific use-cases,
and cannot be applied to new ones when they arise.
As an example,
a planning model based on \emph{behavior trees}
\cite{6907656}
became popular in applied artificial intelligence research in the recent years.
An agent is encoded as a specific behavior tree,
which is then traversed to generate a behavior,
occasionally suspending the traversal to decide on an action.
Behavior tree planning is essentially domain-specific AST interpretation,
plus the ability to suspend and yield decisions.
There is no conceptual reason not to encode behavior trees
as normal programs with \textit{yield} statements.
And yet, faced with the lack of coroutine support in major languages,
AI researchers were effectively forced to implement their own AST interpreters.

This phenomenon is not isolated to AI.
Absence of coroutines is why many elegant abstractions, such as
Erlang-style actors \cite{programming-erlang96},
Oz-style dataflow variables \cite{VanRoy:2004:CTM:983087},
or Esterel-style pause statements \cite{Berry:1992:ESP:147276.147279},
made it to major runtimes such as JVM in a rather truncated form.

Given the advantages,
why is suspending a computation poorly supported?
On one hand, attempts to augment major runtimes such as JVM with continuations
\cite{LAMP-CONF-2007-002} \cite{Stadler:2009:LCJ:1596655.1596679}
were not successful in the past,
in part due to a gap between PL and VM communities,
and partly due to high integration costs.
On the other hand,
languages with support for suspending computations often provide primitives
that are too tied to particular use-cases:
for example, Python generators and C\# enumerators generate one-off datasets,
while Async-Await in C\#, Dart and Scala incorporates concurrency.
As we argue in Section \ref{sec:related},
these are not sufficiently general to encode other forms of suspendable programs.
Furthermore, extensibility of these primitives is limited --
for example, they are not applicable to behavior trees mentioned earlier.

This paper proposes delimited first-class type-safe coroutines.
In our model,
the programmer denotes the sections of the program that can potentially suspend
at arbitrary points.
Importantly, these suspending sections can call into other suspending sections --
our coroutines are not lexically limited to the scope of one function,
and this enables composing suspendable computations.
The translation is done statically at compile time,
as a source-to-source transformation on the AST-level.
This transformation depends on the static
metaprogramming support of the host language,
described more closely in Section \ref{sec:preliminaries}.
We note that our transformation
can be applied selectively on delimited sections of the program --
it does not require recompiling the entire program.

Our implementation is done in Scala,
a statically compiled, type-safe language that primary targets the JVM.
Past attempts to bring coroutines to JVM
relied either on bytecode instrumentation,
which showed incomplete, and hard to evolve \cite{coroutines-java};
or on JVM modifications,
which did not become standard \cite{Stadler:2009:LCJ:1596655.1596679};
or on threads, which proved heavyweight.
The language metaprogramming API is usually more stable,
and less susceptible to breaking changes.
Another advantage is that
the implementation is not bound to the backend platform --
Scala has an alternative backend
that compiles to JavaScript \cite{EPFL-REPORT-190834},
and our implementation works on NodeJS and in the browsers as well.

The design is driven by the following principles:

\begin{itemize}
\item
\textbf{Generality.}
The model should subsume other models by easily encoding them.
Domain-specific alternatives such as generators, async-await or backtracking
should be easy to express.
This obviates the need for multiple competing models.
For example, C\# exposes both enumerators and async-await, for historical reasons,
but this should be avoided.

\item
\textbf{Composability.}
It should be possible to mix user-defined coroutines
with coroutines defined in different modules.
Coroutines encoded by independent clients
must be able to \emph{mutually call themselves and suspend in nested calls}
(as explained in Section \ref{sec:prog-model}).
Also, to allow abstracting over the coroutine implementation,
coroutines should be \emph{first-class program values}.
When we say \emph{composable}, we require these two properties.

\item
\textbf{Type-safety.}
Coroutines should be type-safe.
In particular, the type of the coroutine
should determine the type of values that it yields or returns to the caller.

\item
\textbf{Ease of use.}
The coroutine model must be easily understood by its end-users, programmers,
which is a prerequisite for its adoption.
This was an issue with some previous models --
for example, we noticed that users find shift-reset continuations hard to grasp.

\item
\textbf{Efficiency.}
Even without runtime support,
the coroutine model should have reasonable performance,
and acceptable overheads.
For example, allocating a heap object for each invocation frame
or chaining lambdas to call into another coroutine is not acceptable.

\item
\textbf{Selectivity.}
It must be possible to apply the transformation selectively,
i.e. on specific sections of the user code that need to suspend.
This precludes the need for whole program transformation,
since users cannot always modify existing program sources.

\item
\textbf{Feasibility.}
It must be possible to translate,
without recompiling legacy code or third-party libraries,
a program using coroutines to standard language constructs.
This ensures portability between multiple backends.
Later,
when and if the runtime decides to cooperate,
it can improve performance
with facilities such as \texttt{longjmp},
stack introspection or with targeted JIT optimizations.
\end{itemize}


\subsection{Contributions}\label{sec:contributions}

This paper makes the following contributions:

\begin{itemize}
\item
A programming model for typed, first-class, stackful coroutines,
that compose through direct calls
(even when coroutines are defined in different libraries),
that can act as both symmetric and asymmetric,
and support snapshotting to clone the execution state on demand,
which makes coroutines as expressive as continuations;
accompanied with case studies
that show its applicability to other areas
(Section \ref{sec:prog-model}).

\item
A formal description of the programming model
and its operational semantics,
along with the progress and preservation proofs,
and the proof for the yield type covariance (Section \ref{sec:formal}).

\item
A source-to-source transformation
(a) that works on explicitly delimited sections of the code,
(b) that uses static metaprogramming,
(c) requires no special runtime support, and
(d) applies coroutine-specific optimizations.
The transformation is formalized, and a concrete implementation is discussed
(Section \ref{sec:transformation}).

\item
A complete implementation of the proposed approach in Scala,
which relies on Scala Macros \cite{Burmako:2013:SML:2489837.2489840}
and Scala Quasiquotes \cite{EPFL-REPORT-185242}
(the two Scala's metaprogramming APIs).
Our implementation is distributed as a Scala library.

\item
An experimental evaluation comparing
the performance of our implementation
against Scala Delimited Continuations, Scala Async,
iterators, and lazy streams
on benchmarks ranging from collection traversal
to backtracking and concurrent execution
(Section \ref{sec:eval}).
\end{itemize}

Coroutines were extensively investigated in the past
\cite{Anton2010}
\cite{LAMP-CONF-2007-002}
\cite{Felleisen:1988:TPF:73560.73576}
\cite{Liskov:1977:AMC:359763.359789}
\cite{Moura:2009:RC:1462166.1462167}
\cite{yield-mainstream}
\cite{Sabry:1992:RPC:141478.141563}
\cite{Stadler:2009:LCJ:1596655.1596679},
and domain-specific variants
were proposed on numerous occasions
\cite{pep-delegation}
\cite{EPFL-CONF-188383}
\cite{scala-async}
\cite{Liskov:1977:AMC:359763.359789}
\cite{pep-generators}.
However, as discussed in Section \ref{sec:related},
we are unaware of any coroutine implementation
with the combination of features that we propose --
to the best of our knowledge,
this is the first type-safe stackful
coroutine implementation that incorporates snapshots,
provides first-class coroutine values,
which relies only on the metaprogramming API of the language,
and has similar performance to hand-optimized code,
as reported in Section \ref{sec:eval}.
%Here, snapshots and reliance on metaprogramming
%are the two most important contributions.

\subsection{Preliminaries}\label{sec:preliminaries}

Our examples throughout this paper
are in the Scala programming language \cite{200464/IC}.
We took care to make the paper accessible to a wide audience
by using a minimal set of Scala features.
The \texttt{def} keyword declares a method,
while \texttt{var} and \texttt{val}
declare mutable and final variables, respectively.
Lambdas are declared with the right-arrow symbol \texttt{=>}.
Type annotations go after the variable name, colon-delimited (\texttt{:}).
Type parameters are put into square brackets \texttt{[]}.
Parenthesis can be omitted from nullary and unary method calls.

Our implementation is written in Scala,
and it relies on Scala Macros
\cite{Burmako:2013:SML:2489837.2489840},
its metaprogramming API.
The following are the key metaprogramming features of Scala Macros
that our transformation scheme relies on.
First, it must be possible to declare \textit{macro definitions}
that take ASTs as input arguments and return transformed ASTs.
Second, it must be possible to invoke such macro definitions from user programs,
which makes the compiler execute the macro with its argument expressions
and replace the macro invocation with the resulting AST.
Third, it must be possible to decompose and compose those ASTs
inside the macro definition.
Finally, it must be possible to inspect the types of the expressions
passed to the macro, and reason about symbol identity.
The following is an example of a macro definition:

\begin{lstlisting}[language=scala,label=list:pull,captionpos=t]
def log(msg: String): Unit = macro log_impl
def log_impl(c: Context)(msg: c.Tree): c.Tree =
  q"""if (loggingEnabled) info(currentTime() + ": " + $msg)"""
\end{lstlisting}

Above, we declared a \texttt{log} macro
with the macro implementation \texttt{log\_impl},
which takes the corresponding \texttt{Tree} arguments.
The \texttt{log\_impl} method uses the quasiquote notation \texttt{q""}
to build an AST \cite{EPFL-REPORT-185242},
which in turn checks if logging is enabled
before constructing the command line output from the \texttt{msg} string.
Values are interpolated into the AST using the \texttt{\$} notation,
as is the case with the expression \texttt{\$msg} above.

As an added benefit, Scala macro definitions can be packaged into libraries,
and then separately shipped.
Our own coroutine implementation is therefore a macro library,
which the users can import into their programs.
Furthermore, user coroutines implemented using our coroutine library
can be packaged into third party libraries in a similar way.


==> old-programming-model.tex <==

\section{Programming Model}\label{sec:prog-model}

A subroutine is a sequence of program statements that carry out a specific task.
The same subroutine may execute multiple times during the program execution.
When a program section calls a subroutine,
execution is suspended at that callsite and transferred to the subroutine.
Execution at the callsite resumes only after the subroutine completes execution.
For example, the program in Listing \ref{list:subroutine}
declares a subroutine that
adds an integer to itself,
and then invokes it with the argument \texttt{7}.

\begin{multicols}{2}
\begin{lstlisting}[
caption={Subroutine example},language=scala,label=list:subroutine,captionpos=t,
abovecaptionskip=-\medskipamount,
belowskip=-\medskipamount
]
val dup = (x: Int) => { x + x }
dup(7)
\end{lstlisting}
\columnbreak
\begin{lstlisting}[
caption={Coroutine example},language=scala,label=list:coroutine,captionpos=t,
abovecaptionskip=-\medskipamount,
belowskip=-\medskipamount
]
val dup =
  coroutine { (x: Int) => x + x }
\end{lstlisting}
\end{multicols}

Upon calling \texttt{dup} with the input \texttt{7},
the subroutine does an addition, returns the result and terminates.
When the execution resumes from the callsite, subroutine invocation no longer exists.

\emph{Coroutines} generalize subroutines by being able to
suspend during their execution, so that their execution can be resumed later.
In our implementation, a coroutine is declared
inside the \texttt{coroutine} block.
We show the coroutine equivalent of \texttt{dup}
in Listing \ref{list:coroutine}.

Similarly to how invoking a subroutine creates a running instance of that subroutine
on the program stack, starting a coroutine creates a new \emph{coroutine instance}.
Unlike a subroutine, whose execution cannot be observed by the program,
execution of a coroutine has to be resumed by the its caller.
The caller must be able to refer to the coroutine instance.
Therefore, the coroutine instance must be a first class value,
and we create it with the \texttt{call} keyword,
as shown in Listing \ref{list:call}.
The coroutine instance \texttt{i} is suspended immediately after creation,
and is just about to start executing the expression,
as shown in Listing \ref{list:exec-dup}.

\begin{multicols}{2}
\begin{lstlisting}[
caption={Starting a coroutine},numbers=none,language=scala,label=list:call,
captionpos=t,
abovecaptionskip=-\medskipamount,
belowskip=-\medskipamount
]
val i = call(dup(7))
\end{lstlisting}
\columnbreak
\begin{lstlisting}[
caption={Execution of \texttt{dup}},numbers=none,language=scala,mathescape,
label=list:exec-dup,captionpos=t,
abovecaptionskip=-\medskipamount,
belowskip=-\medskipamount
]
$_\uparrow$7 + 7 $\Rightarrow$ 7 + 7$_\uparrow$
\end{lstlisting}
\end{multicols}

To resume the coroutine instance \texttt{i},
the main program can use the expression \texttt{i.resume},
which runs the instance to its completion and returns \texttt{false},
indicating that the coroutine completed
and \texttt{resume} can no longer be called.
As shown so far, coroutines are not more expressive than subroutines,
and introduce additional boilerplate.
To understand their advantages, we next see how a coroutine suspends itself.

Statements that suspend the coroutine must be enclosed within the
coroutine's lexical scope,
which we call the \emph{coroutine context}.
In the previous example,
the coroutine context consists of statements inside the
\texttt{coroutine} block, i.e. \texttt{x + x}.
When the coroutine suspends,
it must yield a value to the caller that previously resumed it.
This is done with the \texttt{yieldval} statement in our implementation,
and it allows moving control decisions to the enclosing program.
For example,
the \texttt{dup} coroutine hardcodes the decision
to add its argument together.
Listing \ref{list:yield}
shows how to rewrite it to instead yield the argument twice,
deferring the decision of how to combine the values to its caller.

\begin{multicols}{2}
\begin{lstlisting}[caption={Yielding values},language=scala,label=list:yield,captionpos=t,abovecaptionskip=-\medskipamount]
val dup = coroutine { (x:Int) =>
  yieldval(x)
  yieldval(x) }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Resuming a coroutine},language=scala,mathescape,label=list:resume-value,captionpos=t]
val i = call(dup(7))
var sum = 0
while (i.resume) sum += i.value
\end{lstlisting}
\end{multicols}

The caller then decides how to use the values.
By returning \texttt{true},
\texttt{resume} indicates that the coroutine did not complete.
In this case,
method \texttt{value} returns the last yielded value.
The main program can iterate the values in a \texttt{while} loop,
as shown in Listing \ref{list:resume-value}.
While the caller is invoking \texttt{resume},
the coroutine goes through the following execution states:
%in Listing \ref{list:exec-states}.

%\begin{multicols}{2}
\begin{lstlisting}[language=scala,mathescape,numbers=none,label=list:exec-states,captionpos=t]
{ $_\uparrow$yieldval(7); yieldval(7) } $\Rightarrow$ { yieldval(7); $_\uparrow$yieldval(7) } $\Rightarrow$
$\Rightarrow$ { yieldval(7); yieldval(7)$_\uparrow$ } $\Rightarrow$ { yieldval(7); yieldval(7)$_{\;\,}$}
\end{lstlisting}
%\columnbreak
%\begin{lstlisting}[caption={Execution states of \texttt{dup}},language=scala,mathescape,label=list:exec-states,captionpos=t]
%$_\uparrow$yieldval(7); yieldval(7)
%yieldval(7); $_\uparrow$yieldval(7)
%yieldval(7); yieldval(7)$_\uparrow$
%yieldval(7); yieldval(7)$_{\;\,}$
%\end{lstlisting}
%\end{multicols}

The last \texttt{resume} returns \texttt{false},
indicating that the coroutine completed, and it is illegal to call \texttt{value}.
To retrieve the return value of the coroutine,
the program must call \texttt{result}.
Note that the type of the yielded values \texttt{Y} does not need to correspond
to the return type \texttt{R} of the coroutine --
in the previous example, the \emph{yield type} is \texttt{Int},
while the return type is \texttt{Unit}.


\textbf{Coroutine typing.}
In the previous sections,
we saw that coroutine definitions are first-class values.
As such, both coroutines and coroutine instances are typed.
Previous examples relied on type inference to avoid explicit type annotations,
which we show next.

Similar to a function type,
a coroutine type must encode the types $\texttt{P}_i$ of its parameters
and the return type \texttt{R}.
Additionally, a coroutine type must encode the type of the values it yields,
called the yield type \texttt{Y}.
Generally, a coroutine has the type
\texttt{(P1, ..., PN) \textasciitilde> (Y, R)}.
We annotate the first version of the \texttt{dup} coroutine as follows:

\begin{lstlisting}[language=scala,mathescape,label=list:type-coroutine-dup,captionpos=t,numbers=none]
val dup: Int ~> (Nothing, Int) = coroutine { (x: Int) => x + x }
\end{lstlisting}

Since this coroutine does not yield any values,
its yield type is \texttt{Nothing}, the bottom type in Scala.
A coroutine \texttt{once}, which yields its argument once,
has the yield type \texttt{Int}:

\begin{lstlisting}[language=scala,mathescape,label=list:type-coroutine-once,captionpos=t,numbers=none]
val once: Int ~> (Int, Unit) = coroutine { (x: Int) => yieldval(x) }
\end{lstlisting}

Instances need not encode input parameters.
For a yield type \texttt{Y} and a return type \texttt{R},
a coroutine instance has the type
\texttt{Y <\textasciitilde> R}.
For example, \texttt{once} gives the type
\texttt{Int <\textasciitilde> Unit}:

\begin{lstlisting}[language=scala,mathescape,label=list:type-coroutine-instance,captionpos=t,numbers=none]
val i: Int <~> Unit = call(once(7))
\end{lstlisting}

Distinguishing between yield types and return types
allows a coroutine to have different responsibilities
towards the site that created the coroutine instance
and towards its direct caller.
This is an essential prerequisite for composability,
which we explore next.

\begin{figure}

\begin{center}
\begin{tikzpicture}
  [
    frame/.style={rectangle,draw,line width=0.2mm},
    empty/.style={rectangle,draw,dashed,line width=0.2mm},
  ]
  \node(sl)  at (-1.00, 0.00)  [] {};
  \node(s0)  at (-1.00, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s1)  at (-1.00, 0.30)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s2)  at (-1.00, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(c0)  at ( 1.50, 0.00)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small A};
  \node(c1)  at ( 1.50, 0.30)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(c2)  at ( 1.50, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node()    at (-1.20, 1.00)  [] {\small caller};
  \node()    at ( 1.60, 1.30)  [align=center] {\small coroutine\\ \small instance};
  \node(p1)  at (-0.40, 0.90)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $1$};
  \node(p2)  at (-0.30,-0.55)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $2$};
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s1) edge[bend left=+30] node[above=3.5pt,xshift=-0.5mm] {\small\lstinline$resume$} (c0);
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (c0) edge[bend left=+30] node[below=2.5pt,xshift=3mm] {\small\lstinline$yieldval$} (s1);
\end{tikzpicture}
\quad\quad
\begin{tikzpicture}
  [
    frame/.style={rectangle,draw,line width=0.2mm},
    empty/.style={rectangle,draw,dashed,line width=0.2mm},
  ]
  \node(s0)  at (-1.00, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s1)  at (-1.00, 0.30)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s2)  at (-1.00, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(c0)  at ( 0.90, 0.45)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small A};
  \node(c1)  at ( 0.90, 0.75)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(c2)  at ( 0.90, 1.05)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(d0)  at ( 2.80, 0.00)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small B};
  \node(d1)  at ( 2.80, 0.30)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(d2)  at ( 2.80, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node()    at (-1.20, 1.00)  [] {\small caller};
  \node(p1)  at (-0.50, 0.85)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $1$};
  \node()    at ( 0.90, 1.40)  [] {\small instance A};
  \node(p2)  at ( 1.55, 1.05)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $2$};
  \node(p3)  at ( 1.35, 0.70)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $3$};
  \node()    at ( 1.95, 0.70)  [] {\small \lstinline$resume$};
  \node()    at ( 3.30, 1.00)  [] {\small instance B};
  \node(p4)  at ( 1.00,-0.42)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $4$};
  \draw[-stealth,thick,shorten <=1.5pt,shorten >=1.5pt] (s1) edge[bend left=+20] node[above=1.5pt,xshift=1.5mm] {\small\lstinline$resume$} (c0);
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (c0) edge[bend left=+20] node[above=11pt,xshift=1.3mm] {\small\lstinline$call$} (d0);
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (d0) edge[bend left=+30] node[below=2.5pt] {\small\lstinline$yieldval$} (c0);
\end{tikzpicture}
\quad\quad
\begin{tikzpicture}
  [
    frame/.style={rectangle,draw,line width=0.2mm},
    empty/.style={rectangle,draw,dashed,line width=0.2mm},
  ]
  \node(s0)  at (-1.10, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s1)  at (-1.10, 0.30)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s2)  at (-1.10, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(c0)  at ( 1.20, 0.00)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small A};
  \node(c1)  at ( 1.20, 0.30)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small B};
  \node(c2)  at ( 1.20, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node()    at (-1.20, 1.00)  [] {\small caller};
  \node(p1)  at (-0.50,-0.50)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $1$};
  \node(p2)  at ( 1.60, 0.60)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $2$};
  \node(p3)  at (-0.50, 0.80)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $3$};
  \node()    at ( 1.60, 1.30)  [align=center] {\small coroutine\\ \small instance};
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s1) edge[bend left=-30] node[below=2.5pt,xshift=1.0mm] {\small\lstinline$resume$} (c0);
  \draw[-stealth,thick,shorten <=0.5pt,shorten >=0.5pt] (c0) ++(330:2.3mm) arc (-120:75:2.3mm) --++(180:2mm) node[above=-10.5pt,xshift=9.0mm,text width=1cm] {\small \textit{direct}\\\textit{call}};
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (c1) edge[bend left=-20] node[above=-0.5pt,xshift=2.0mm] {\small\lstinline$yieldval$} (s1);
\end{tikzpicture}

\begin{tikzpicture}
\node()  at (-4.20, 0.00)  [] {\small \; RESUME AND YIELD VALUE};
\node()  at ( 0.60, 0.00)  [] {\small \; \; COROUTINE CALL};
\node()  at ( 6.70, 0.00)  [] {\small DIRECT CALL};
\node()  at ( 8.90, 0.00)  [] {};
\end{tikzpicture}
\end{center}

\caption{Control constructs: \lstinline$yieldval$, \lstinline$call$ and direct calls}
\label{fig:control}
\end{figure}


\textbf{Coroutine composability.}
%Composability allows reusing existing coroutines.
Being able to invoke a coroutine as if it were a normal subroutine
allows composing suspendable subcomponents.
A \emph{direct coroutine call} is akin to a normal function call
(i.e. a beta-reduction on coroutines),
and is different from starting a new coroutine with \texttt{call}.
When a coroutine $A$ calls a coroutine $B$ directly,
$A$'s execution suspends until $B$ completes.
If $B$ yields a value,
control is not transferred to $A$,
but to the site that invoked \texttt{resume} on $A$
(Fig. \ref{fig:control}, right).
This way, $A$ and $B$ work together to yield a common set of values.
Since a coroutine execution can yield,
these direct coroutine calls are only allowed inside coroutine definitions.

Consider the task of yielding elements of a closed addressing hash table.
The coroutine \texttt{bucket}
in Listing \ref{list:hash-bucket}
yields individual elements of each bucket,
while the coroutine in Listing \ref{list:hash-table}
traverses the table
and delegates the task of actual yielding to \texttt{bucket}.

\begin{multicols}{2}
\begin{lstlisting}[caption={List coroutine},language=scala,label=list:hash-bucket,captionpos=t,abovecaptionskip=-\medskipamount]
val bucket = coroutine { (b: List[Int]) =>
  while (b != Nil) {
    yieldval(b.head)
    b = b.tail
  } }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Array coroutine},language=scala,mathescape,label=list:hash-table,captionpos=t]
coroutine { (t: Array[List[Int]]) =>
  var i = 0
  while (i < t.length) {
    bucket(t(i))`\label{code:bucket}`
    i += 1 } }
\end{lstlisting}
\end{multicols}

Different control constructs are illustrated in Figure \ref{fig:control}.
The leftmost figure represents a normal \texttt{resume}-\texttt{yield} control transfer
between the caller (e.g. main program) and the coroutine instance.
In the middle,
the main program resumes an existing coroutine instance $A$,
which then runs \texttt{call} to create a second coroutine instance $B$,
and resumes $B$.
When the instance $B$ yields,
control is returned to the instance $A$, and not to the caller (e.g. main program).
A direct call (e.g. to the \texttt{bucket} coroutine in line \ref{code:bucket})
is shown on the right.
Unlike \texttt{call},
a direct call does not create a new coroutine instance,
but instead reuses the stack of the current instance.
The two coroutines share a common callsite,
and this allows separating the yielding logic between them.

\textbf{Snapshots.}
Some coroutine use-cases require more than just suspending the coroutine --
starting from an arbitrary state, the rest of the coroutine may have to be executed
more than once.
When called on a coroutine instance,
the \texttt{snapshot} operation duplicates it and returns a new instance
with exactly the same execution state.
Coroutine operations can then be called independently on the two coroutine instances.

\begin{lstlisting}[language=scala,mathescape,label=list:snapshot,captionpos=t,numbers=none]
val i1: Int <~> Unit = call(once(7))
val i2: Int <~> Unit = i1.snapshot
\end{lstlisting}

%Augmenting coroutines with snapshots makes them
%equivalent to shift-reset style delimited continuations,
%as shown in Section \ref{sec:use-cases}.


==> old-use-cases.tex <==
%!TEX root = coroutines-ecoop.tex

\subsection{Use Cases}\label{sec:use-cases}

We now show a series of use-cases for coroutines.
A comparison between original APIs and coroutine-based APIs from the user's perspective
is given in the appendix, Section \ref{sec:use-case-comparison}.

\textbf{Iterators.}
Data structure iterators are one of the earliest coroutine applications
\cite{Liskov:1977:AMC:359763.359789}.
We showed a hash table iterator implementation
in Listings \ref{list:hash-bucket} and \ref{list:hash-table}.
Since direct calls allow recursion,
we can implement an iterator for binary trees in a similar way:

\begin{lstlisting}[caption={Tree iterator implementation},language=scala,mathescape,label=list:iterator,captionpos=t]
val iterate = coroutine { (t: Tree) =>
  if (t.left != null) iterate(t.left)
  yieldval(t.element)
  if (t.right != null) iterate(t.right) }
\end{lstlisting}

We implement iterators for graphs, with both BFS or DFS traversal, analogously.
We test the performance of different iterator implementations in Section \ref{sec:eval}.

\textbf{AI agents.}
AI agents such as behavior trees \cite{6907656}
are essentially suspendable computations.
The following agent searches for a nearby friend,
and yields either \texttt{Move} or \texttt{Chat} commands.

\begin{multicols}{2}
\begin{lstlisting}[label=list:decide,language=scala,captionpos=t,abovecaptionskip=-\medskipamount]
val decide = coroutine { () =>
  while (true) {
    val e = findNearestFriend()
    if (self.near(e)) chat(e)
    else {
      val dest = findUnexplored()
      move(dest)
    } } }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[label=list:commands,language=scala,captionpos=t]
val chat = coroutine { (c:NPC) =>
  do yieldval(Chat(c))
  while (self.near(c)) }
val move = coroutine { (dest:XY) =>
  var path = aStar(here, dest)
  while (path.nonEmpty) {
    yieldval(Move(path.head))
    path = path.tail } }
\end{lstlisting}
\end{multicols}

\textbf{Async-await.}
The \texttt{async} statement, which starts asynchronous computations,
and \texttt{await}, which blocks until a value is available,
are used to rewrite direct-style code into an asynchronous callback chain on futures.
In Scala, type \texttt{Future} exposes the \texttt{onSuccess} method,
which takes a callback to run once its value is available,
and \texttt{value}, used to pull the value if already available.
\texttt{Promise} is the future's writing end,
and exposes \texttt{success},
which sets the value of the corresponding future at most once \cite{SIP14}.

In the following,
we use coroutines to replicate Scala's Async-Await framework \cite{scala-async}.
Method \texttt{await} returns a coroutine that yields a future
and then returns its value.
The \texttt{async} method takes a computation \texttt{b},
starts a coroutine instance, executes it asynchronously in a \texttt{Future},
and recursively installs a new callback whenever the coroutine resumes.

\begin{lstlisting}[caption={Async-await implementation},language=scala,mathescape,label=list:async-await,captionpos=t]
def await[R]: Future[R] ~> (Future[R], R) =
  coroutine { (f: Future[R]) => yieldval(f); f.value }
def async[Y, R](b: () ~> (Future[Y], R)): Future[R] = {
  val i = call(b())
  val p = new Promise[R]
  @tailrec def loop(): Unit =
    if (i.resume) i.value.onSuccess(x => loop()) else p.success(i.result)
  Future { loop() }
  p.future
}
\end{lstlisting}

It is worth noting that the encoding
of Async-Await in Listing \ref{list:async-await}
additionally allows terms inside \texttt{async} contexts
to directly call other coroutines,
and these nested calls can then call \texttt{await}.
This is not possible in the
current Async-Await implementation in Scala \cite{scala-async}.

\textbf{Erlang-style actors.}
Since JVM does not have continuations,
actor frameworks are unable to implement exact Erlang-style semantics,
in which the \texttt{receive} statement can be called anywhere in the actor.
Instead, frameworks like Akka expose a top-level \texttt{receive} method \cite{akka},
which returns a partial function used to handle messages.
This function can be swapped during the actor lifetime
with the \texttt{become} statement.
In this example,
we define a function \texttt{recv}
that suspends in the middle of the actor and awaits a message.

We first define an auxiliary type \texttt{Rec[T]},
which describes partial functions that take \texttt{Any} objects.
Method \texttt{act} declares an Erlang-style actor --
it takes coroutines that may yield
partial functions of the \texttt{Rec[T]} type,
which describe how to process the next message.
These partial functions are extended with the \texttt{andThen} combinator
to recursively resume the coroutine instance,
and passed to the \texttt{become} method.
The user-defined actor
can invoke the method \texttt{recv}
to block until a message arrives.
The \texttt{recv} method returns a coroutine that takes
a message-handling function,
extends it using \texttt{andThen} to update a local variable \texttt{res},
and then yields the function back to \texttt{act}.
After \texttt{act} resumes the actor,
the \texttt{recv} returns the result stored in \texttt{res}
back to the user-defined actor.

\begin{lstlisting}[label=list:erlang,caption={Erlang-style actor implementation},language=scala,mathescape,captionpos=t]
type Rec[T] = PartialFunction[Any, T]
def act(c: () ~> (Rec[Unit], Unit)) = Actor { self =>
  val i = call(c())
  def loop() = if (i.resume) self.become(i.value.andThen(_ => loop()))
  loop() }
def recv[T]: Rec[T] ~> (Rec[Unit], T) = coroutine { (f: Rec[T]) =>
  var res: T = _
  yieldval(f.andThen(x => res = x))
  res }
\end{lstlisting}

\textbf{Event streams}.
The \emph{reactor model} generalizes the actor model by replacing
the \texttt{receive} statement with
a first-class entity called an \emph{event stream}
\cite{Prokopec:2015:ICE:2814228.2814245}.
Event streams expose the \texttt{onEvent} method,
similar to \texttt{onSuccess} on futures.
Instead of installing a callback,
the goal is to extract an event in the direct-style,
by calling a special method \texttt{get} on the event stream.
The \texttt{react} method below defines a suspendable reactor,
and \texttt{get} extracts the next event out of a reactor's event stream.
The same technique can be applied to other event streams implementations,
for example Rx-style streams \cite{EPFL-CONF-188383}
\cite{Meijer:2012:YMD:2160718.2160735}.

\begin{lstlisting}[label=list:reactors,caption={Direct-style event streams in reactors},language=scala,mathescape,captionpos=t]
type Obs = (() => Unit) => Sub
def react(c: () ~> (Obs, Unit)) = Reactor[T] { self =>
  val i = call(c())
  def loop() = if (i.resume) i.value(() => loop())
  loop() }
def get[T](e: Events[T]): () ~> (Obs, T) = coroutine { () =>
  var res: T = _
  val subscribe = (f: () => Unit) => { e.onEvent(x => { res = x; f() }) }
  yieldval(subscribe)
  res }
\end{lstlisting}

\textbf{Symmetric coroutines.}
When a coroutine can yield and transfer control to other instances,
and not just to its resume-site,
the coroutine implementation is called \emph{symmetric}.
Our coroutine implementation is \emph{asymmetric},
and does not allow this by default.
However, consider a recursive type defined as
\texttt{type Target=Target<\textasciitilde>Unit}.
Using \texttt{Target} as the yield type allows a coroutine to yield
a coroutine instance that should be resumed next.
This, together with a \texttt{run} function defined as follows,
allows simulating symmetric coroutines:

\begin{lstlisting}[label=list:symmetric-run,numbers=none,language=scala,captionpos=t,abovecaptionskip=-\medskipamount]
@tailrec def run(i: Target) = if (i.resume) run(i.value)
\end{lstlisting}

This shows that our asymmetric coroutines
can be used to simulate symmetric coroutines,
which is consistent with earlier observations
\cite{Moura:2009:RC:1462166.1462167}.

\textbf{Oz-style single-assignment variables.}
Variables in the Oz language \cite{VanRoy:2004:CTM:983087}
do not have a value when created.
Reading them suspends execution until some other thread assigns a value.
Assigning a value to the variable more than once is an error.

\begin{multicols}{2}
\begin{lstlisting}[caption={Oz-style variable read},language=scala,label=list:oz1,captionpos=t,abovecaptionskip=-\medskipamount]
@volatile var state: AnyRef = Lst()

val get = coroutine { () =>
  if (READ(state).is[Lst])
    yieldval(this)`\label{code:get-read}`
  READ(state).as[T]
}

\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Oz-style variable write},language=scala,label=list:oz2,captionpos=t]
@tailrec def set(y: T) {
  val x = READ(state)
  if (x.is[Lst]) {
    if (CAS(state, x, y))
      for (i <- x.as[Lst]) schedule(i)
    else set(y)
  } else sys.error("Assigned!") }
\end{lstlisting}
\end{multicols}

Internally, a single-assignment variable has some \texttt{state},
which is either the list of suspended threads or a value.
When \texttt{get} is called,
\texttt{state} is atomically read in line \ref{code:get-read}.
If the state is a list,
coroutine is yielded to the scheduler,
which tries to atomically replace the list with the new suspended thread (not shown).
The coroutine is resumed when the value becomes available --
method \texttt{set} tries to atomically replace the list
with the value of type \texttt{T}.
If successful, it schedules the suspended threads for execution.

\textbf{Backtracking algorithms.}
Suppose there is a coroutine that recursively evaluates different code paths
of a program \texttt{i}, as if it was traversing a tree.
Program \texttt{i} must cooperate --
each time a different path can be taken,
\texttt{i} must yield a sequence of preparation functions,
each of which is called
before executing the snapshot of the rest of the program.
We call this coroutine \texttt{backtrack}:

\begin{lstlisting}[label=list:backtrack,language=scala,mathescape,captionpos=t]
type Program = (Seq[() => Unit]) <~> Unit // An instance that yields preparation functions.
val backtrack: Program ~> (Unit, Unit) = coroutine { (i: Program) =>
  if (i.resume) for (prepare <- i.value) {
    prepare()
    backtrack(i.snapshot)
  } else yieldval(())`\label{code:code-path-end}`
}
\end{lstlisting}

When \texttt{backtrack} exhausts a code path in line \ref{code:code-path-end},
it itself yields.
This allows generator-based testing frameworks,
such as ScalaCheck \cite{scalacheck},
to use pull-style generators instead of monadic ones
\cite{Wadler:1995:MFP:647698.734146}.
Define the \texttt{Test} type as a coroutine that yields preparation functions
(calling it creates a \texttt{Program} instance defined previously).
Given a suspendable \texttt{Test} coroutine, which represents a test snippet,
the \texttt{check} method starts a coroutine instance of type \texttt{Program},
and uses it to create another coroutine instance called \texttt{exploration}
that runs the backtracking algorithm on the program.
Method \texttt{check} then resumes the \texttt{exploration}
until termination:

\begin{lstlisting}[label=list:backtrack-forever-check,language=scala,mathescape,captionpos=t]
type Test = () ~> (Seq[() => Unit], Unit) // A coroutine that yields preparation functions.
def check(test: Test) {
  val program = call(test())
  val exploration = call(backtrack(program))
  while (exploration.resume) {}
}
\end{lstlisting}

When a generator coroutine,
such as \texttt{ints} shown in Listing \ref{list:backtrack-ints},
gets asked to produce a value,
it will yield a sequence of functions that prepare the rest of execution.

\begin{multicols}{2}
\begin{lstlisting}[caption={Generator for integers},label=list:backtrack-ints,language=scala,mathescape,captionpos=t]
val ints = coroutine { (vals: Seq[Int]) =>
  var res: Int = _
  yieldval(vals.map(x => () => res = x))
  res
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={User test that checks commutativity},label=list:backtrack-test,language=scala,mathescape,captionpos=t]
check(coroutine { () =>
  val a = ints(0 until MAX_INT)
  val b = ints(0 until MAX_INT)
  assert(a * b == b * a)
})
\end{lstlisting}
\end{multicols}

The snippet in Listing \ref{list:backtrack-test}
contains a unit test example that tests commutativity.
The test invokes the \texttt{ints} coroutine directly,
which internally yields preparation functions back to its caller,
i.e. \texttt{backtrack}.
The test is then resumed from each \texttt{ints} multiple times
for different values of \texttt{a} and \texttt{b}.

Through direct coroutine calls,
basic generators such as \texttt{ints}
can be composed into generators for complex data structures,
without having to compose generators monadically
in \texttt{for}-comprehensions.

\textbf{Continuations.}
Shift-reset-style delimited continuations use the \texttt{reset} operator
to delimit regions of the program that can be transformed into a continuation
\cite{Danvy:1990:AC:91556.91622}.
The \texttt{shift} operator,
which takes a function whose input is the current continuation,
can be used inside these regions.
%To show equivalence of coroutines and continuations,
We sketch the implementation of \texttt{shift} and \texttt{reset} operators
similar to those used in Scala delimited continuations
\cite{Rompf:2009:IFP:1631687.1596596}.

\begin{lstlisting}[label=list:continuations,language=scala,mathescape,captionpos=t]
type Shift = (() => Unit) => Unit
def reset(b: () ~> (Shift, Unit)) {
  def continue(i: Shift <~> Unit) = if (i.resume) i.value(() => continue(i.snapshot))
  continue(call(b()))
}
def shift: Shift ~> (Shift, Unit) = coroutine { (b: Shift) => yieldval(b) }
\end{lstlisting}

We first introduce an alias type \texttt{Shift},
which represents continuation handlers --
functions that take continuations of the current program.
The \texttt{reset} operator takes a coroutine
that could yield a \texttt{Shift} object.
It creates a new coroutine instance and resumes it.
If this instance calls \texttt{shift} with a continuation handler,
the handler is yielded back to \texttt{reset},
which invokes the handler with the continuation --
a function that creates a snapshot of the coroutine instance, and resumes it.
The use of \texttt{snapshot} is required,
as the continuation function can be invoked multiple times.


==> phases.tex <==
\begin{tikzpicture}
  [
    frame/.style={rectangle,draw,line width=0.2mm},
    empty/.style={rectangle,draw,dashed,line width=0.2mm},
    scale=0.8,
    every node/.style={scale=0.8},
  ]
  \node(s0)  at ( 0.00, 0.00)  [frame,minimum width=30mm,minimum height=6mm] {\small AST canonicalization};
  \node(s1)  at ( 4.00, 0.00)  [frame,minimum width=30mm,minimum height=6mm] {\small CFG conversion};
  \node(s2)  at ( 8.00, 0.00)  [frame,minimum width=30mm,minimum height=6mm] {\small CFG splitting};
  \node(s3)  at (12.00, 0.00)  [frame,minimum width=30mm,minimum height=6mm] {\small AST generation};
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s0)--(s1);
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s1)--(s2);
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s2)--(s3);
  % \node(s0)  at ( 0.00, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
  % \node(s1)  at ( 0.00, 0.30)  [frame,minimum width=3mm,minimum height=3mm] {};
  % \node(s2)  at ( 0.00, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  % \node(c0)  at ( 1.50, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
  % \node(c1)  at ( 1.50, 0.30)  [empty,minimum width=3mm,minimum height=3mm] {};
  % \node(c2)  at ( 1.50, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  % \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s1) edge[bend left=+30] node[above=3.5pt,xshift=-0.5mm] {\small\lstinline$resume$} (c0);
  % \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (c0) edge[bend left=+30] node[below=2.5pt] {\small\lstinline$yieldval$} (s1);
\end{tikzpicture}


==> programming-model.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Programming Model}\label{sec:prog-model}

In this section,
we describe the proposed programming model
through a series of examples.

\textbf{Coroutine definitions.}
A subroutine is a sequence of statements that carry out a task.
The same subroutine may execute many times during execution.
When a program calls a subroutine,
execution suspends at that callsite and continues in the subroutine.
Execution at the callsite resumes only after the subroutine completes.
For example, the program in Listing \ref{list:subroutine}
declares a subroutine that doubles an integer,
and then calls it with the argument \texttt{7}.

\begin{multicols}{2}
\begin{lstlisting}[
caption={Subroutine example},language=scala,label=list:subroutine,captionpos=t,
abovecaptionskip=-\medskipamount,
belowskip=-\medskipamount
]
val dup = (x:Int) => { x + x }
dup(7)
\end{lstlisting}
\columnbreak
\begin{lstlisting}[
caption={Coroutine example},language=scala,label=list:coroutine,captionpos=t,
abovecaptionskip=-\medskipamount,
belowskip=-\medskipamount
]
val dup =
  coroutine { (x:Int) => x + x }
\end{lstlisting}
\end{multicols}
\vspace{0.2cm}

Upon calling \texttt{dup},
the subroutine does an addition, returns the result and terminates.
When the execution resumes from the callsite,
the subroutine invocation no longer exists.

\emph{Coroutines} generalize subroutines by being able to
suspend during their execution, so that their execution can be resumed later.
In our implementation, a coroutine is defined inside the \texttt{coroutine} block.
We show the coroutine equivalent of \texttt{dup}
in Listing \ref{list:coroutine}.

\textbf{Yielding and resuming.}
Once started, the \texttt{dup} coroutine from Listing \ref{list:coroutine}
runs to completion without suspending.
However, a typical coroutine will suspend at least once.
When it does, it is useful that it \emph{yields} a value
to the caller, explaining why it is suspended.

Consider the coroutine \texttt{rep} in Listing \ref{list:yield},
which takes one argument \texttt{x}.
The \texttt{rep} coroutine invokes the \texttt{yieldval} primitive
to yield the argument \texttt{x} back to its caller, twice in a row.

\begin{multicols}{2}
\begin{lstlisting}[caption={Yielding example},language=scala,label=list:yield,captionpos=t,abovecaptionskip=-\medskipamount]
val rep = coroutine { (x:Int) =>
  yieldval(x)
  yieldval(x)
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Execution states},language=scala,mathescape,label=list:exec-states,captionpos=t]
{ $_\uparrow$yieldval(7); yieldval(7) } $\Rightarrow$`\label{code:yieldval-1}`
{ yieldval(7); $_\uparrow$yieldval(7) } $\Rightarrow$`\label{code:yieldval-2}`
{ yieldval(7); yieldval(7)$_\uparrow$ } $\Rightarrow$`\label{code:yieldval-3}`
{ yieldval(7); yieldval(7)$_{\;\,}$}`\label{code:yieldval-4}`
\end{lstlisting}
\end{multicols}

Listing \ref{list:exec-states} show the states
that the coroutine undergoes during its execution for \texttt{x=7}.
The upward arrow ($\uparrow$) denotes the program counter.
After getting invoked,
the coroutine is paused in line \ref{code:yieldval-1}
before the first \texttt{yieldval}.
The caller resumes the coroutine (resuming is explained shortly),
which then executes the next \texttt{yieldval}
and yields the value \texttt{7} in line \ref{code:yieldval-2}.
The caller resumes the coroutine again,
and the coroutine executes the last \texttt{yieldval}
in line \ref{code:yieldval-3}.
The caller then resumes the coroutine the last time,
and the coroutine terminates in line \ref{code:yieldval-4}.
The termination of a coroutine is similar to a termination of a subroutine --
once the control flow reaches the end,
the invocation of the corresponding coroutine no longer exists.

\textbf{Delimited coroutines.}
As stated in the introduction,
the proposed coroutine model is \emph{delimited}.
This means that the \texttt{yieldval} keyword can only occur inside a scope
that is lexically enclosed with the \texttt{coroutine} keyword --
a free \texttt{yieldval} results in a compiler error.

By itself, this restriction could hinder composability.
Consider a hash table with closed addressing,
which consists of an array whose entries are lists of elements (buckets).
We would like a coroutine that traverses the elements of the hash table.
Given a separately implemented \texttt{bucket} coroutine
from Listing \ref{list:hash-bucket} that yields from a list,
it is handy if a hash table coroutine can reuse this existing functionality
by passing buckets from which to yield.

\begin{multicols}{2}
\begin{lstlisting}[caption={List coroutine},language=scala,label=list:hash-bucket,captionpos=t,abovecaptionskip=-\medskipamount]
val bucket = coroutine {
  (b: List[Int]) =>
  while (b != Nil) {
    yieldval(b.head)
    b = b.tail
  }
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Hash table coroutine},language=scala,mathescape,label=list:hash-table,captionpos=t]
val hashtable = coroutine {
  (t: Array[List[Int]]) =>
  var i = 0
  while (i < t.length) {
    bucket(t(i)); i += 1`\label{code:bucket}`
  }
}
\end{lstlisting}
\end{multicols}

% \begin{figure}

% \begin{center}
% \begin{tikzpicture}
%   [
%     frame/.style={rectangle,draw,line width=0.2mm},
%     empty/.style={rectangle,draw,dashed,line width=0.2mm},
%   ]
%   \node(s0)  at (-1.00, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
%   \node(s1)  at (-1.00, 0.30)  [frame,minimum width=3mm,minimum height=3mm] {};
%   \node(s2)  at (-1.00, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
%   \node(c0)  at ( 0.90, 0.45)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small A};
%   \node(c1)  at ( 0.90, 0.75)  [empty,minimum width=3mm,minimum height=3mm] {};
%   \node(c2)  at ( 0.90, 1.05)  [empty,minimum width=3mm,minimum height=3mm] {};
%   \node(d0)  at ( 2.80, 0.00)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small B};
%   \node(d1)  at ( 2.80, 0.30)  [empty,minimum width=3mm,minimum height=3mm] {};
%   \node(d2)  at ( 2.80, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
%   \node()    at (-1.20, 1.00)  [] {\small caller};
%   \node(p1)  at (-0.50, 0.85)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $1$};
%   \node()    at ( 0.90, 1.40)  [] {\small instance A};
%   \node(p2)  at ( 1.45, 1.05)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $2$};
%   \node(p3)  at ( 1.35, 0.70)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $3$};
%   \node()    at ( 1.95, 0.70)  [] {\small \lstinline$resume$};
%   \node()    at ( 3.30, 1.00)  [] {\small instance B};
%   \node(p4)  at ( 1.00,-0.42)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $4$};
%   \draw[-stealth,thick,shorten <=1.5pt,shorten >=1.5pt] (s1) edge[bend left=+20] node[above=1.5pt,xshift=1.5mm] {\small\lstinline$resume$} (c0);
%   \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (c0) edge[bend left=+20] node[above=11pt,xshift=1.3mm] {\small\lstinline$start$} (d0);
%   \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (d0) edge[bend left=+30] node[below=2.5pt] {\small\lstinline$yieldval$} (c0);
% \end{tikzpicture}

% \begin{tikzpicture}
% \node()  at (-4.20, 0.00)  [] {\small \; RESUME AND YIELD VALUE};
% \node()  at ( 0.60, 0.00)  [] {\small \; \; COROUTINE START};
% \node()  at ( 8.90, 0.00)  [] {};
% \end{tikzpicture}
% \end{center}

% \caption{Control constructs: \lstinline$yieldval$, \lstinline$start$ and direct calls}
% \label{fig:control}
% \end{figure}

\paratitle{Stackful coroutines}
To allow composing separately written coroutines,
it must be possible for one coroutine to call into another coroutine,
but retain the same yielding context.
The \texttt{hashtable} coroutine in Listing \ref{list:hash-table}
traverses the array entries,
and calls \texttt{bucket} for each entry.
The two coroutines yield values together, as if they were a single coroutine.

\begin{wrapfigure}{R}{0.3\textwidth}
\begin{minipage}{0.3\textwidth}
\begin{tikzpicture}
  [
    frame/.style={rectangle,draw,line width=0.2mm},
    empty/.style={rectangle,draw,dashed,line width=0.2mm},
  ]
  \node(s0)  at (-1.10, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s1)  at (-1.10, 0.30)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s2)  at (-1.10, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(c0)  at ( 1.20, 0.00)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small h};
  \node(c1)  at ( 1.20, 0.30)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small b};
  \node(c2)  at ( 1.20, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node()    at (-1.20, 1.00)  [] {\small caller};
  % \node(p1)  at (-0.50,-0.50)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $1$};
  \node(p2)  at ( 1.60, 0.60)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $1$};
  \node(p3)  at (-0.55, 0.80)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $2$};
  \node()    at ( 1.60, 1.00)  [align=center] {\small coroutine};
  % \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s1) edge[bend left=-30] node[below=2.5pt,xshift=1.0mm] {\small\lstinline$resume$} (c0);
  \draw[-stealth,thick,shorten <=0.5pt,shorten >=0.5pt] (c0) ++(330:2.3mm) arc (-120:75:2.3mm) --++(180:2mm) node[above=-10.5pt,xshift=9.0mm,text width=1cm] {\small \textit{direct}\\\textit{call}};
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (c1) edge[bend left=-20] node[above=-0.5pt,xshift=2.0mm] {\small\lstinline$yieldval$} (s1);
\end{tikzpicture}
\end{minipage}
\end{wrapfigure}
Similar to ordinary subroutine calls,
when the \texttt{hashtable} coroutine calls \texttt{bucket},
it must store its local variables and state.
One way to achieve this is to use a call stack.
When the program resumes the \texttt{hashtable} coroutine,
it switches from the normal program call stack
to a separate call stack that belongs to the resumed coroutine instance.
The \texttt{hashtable} coroutine then pushes its state to the stack,
and passes the control flow to the \texttt{bucket} coroutine
(\circled{1} in the figure below).
The \texttt{bucket} coroutine stores its state to the stack and
yields \emph{to the same caller that
originally resumed the \texttt{hashtable} coroutine}
(\circled{2}).

By saying that our coroutine model is \emph{stackful},
we mean that coroutines are able to call each other,
and yield back to the same resume-site \cite{Moura:2009:RC:1462166.1462167}.
In our implementation, this is enabled with an artifical call stack,
as explained in Section \ref{sec:implementation}.

Importantly, a coroutine call can only occur in a scope
that is lexically enclosed with the \texttt{coroutine} keyword
(akin to \texttt{yieldval}).
Only a coroutine body can call another coroutine --
a free call is a compiler error.
A natural questions follows:
how does a normal program create a new coroutine instance?

\paratitle{Coroutine instances}
Similar to how invoking a \emph{subroutine}
creates a running instance of that subroutine,
starting a \emph{coroutine} creates a new \emph{coroutine instance}.
A subroutine's execution is not a program value -- it cannot be observed or controlled.
However, after creating a coroutine instance,
the caller must interact with it
by reading the yielded values and resuming.
Therefore, it is necessary to treat the coroutine instance as a program value.

To distinguish between normal coroutine calls and creating a coroutine instance,
we introduce a separate \texttt{start} keyword, as a design choice.
The instance encapsulates a new call stack.
After \texttt{start} returns a new coroutine instance,
the caller can invoke \texttt{resume} and \texttt{value} on the instance.
By returning \texttt{true},
the \texttt{resume} indicates that the instance yielded,
and did not yet terminate.
In this case, invoking \texttt{value} returns the last yielded value.

\vspace{0.2cm}
\begin{multicols}{2}
\begin{lstlisting}[caption={Starting and resuming},language=scala,label=list:resume-value,captionpos=t,abovecaptionskip=-\medskipamount]
val i = hashtable.start(array)`\label{code:hashtable-start}`
var sum: Int = 0`\label{code:hashtable-sum}`
while (i.resume) sum += i.value`\label{code:hashtable-resume-value}`
\end{lstlisting}
\columnbreak
\quad\quad
\begin{tikzpicture}
  [
    frame/.style={rectangle,draw,line width=0.2mm},
    empty/.style={rectangle,draw,dashed,line width=0.2mm},
  ]
  \node(s0)  at (-1.10, 0.00)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s1)  at (-1.10, 0.30)  [frame,minimum width=3mm,minimum height=3mm] {};
  \node(s2)  at (-1.10, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node(c0)  at ( 1.60, 0.00)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small h};
  \node(c1)  at ( 1.60, 0.30)  [frame,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small b};
  \node(c2)  at ( 1.60, 0.60)  [empty,minimum width=3mm,minimum height=3mm] {};
  \node()    at (-1.20, 1.00)  [] {\small caller};
  \node(p0)  at (-1.75,-0.50)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $1$};
  \node(p1)  at (-0.30,-0.50)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $2$};
  \node(p2)  at ( 2.00, 0.60)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $3$};
  \node(p3)  at (-0.35, 0.30)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $4$};
  \node(p4)  at (-0.25, 0.95)  [circle,draw,minimum width=3mm,minimum height=3mm,inner sep=0pt] {\small $5$};
  \node()    at ( 2.00, 1.00)  [align=center] {\small instance};
  \node()    at (-1.20,-0.50)  [align=center] {\small \lstinline$start$};
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s1) edge[bend left=-30] node[below=2.5pt,xshift=1.0mm] {\small\lstinline$resume$} (c0);
  \draw[-stealth,thick,shorten <=0.5pt,shorten >=0.5pt] (c0) ++(330:2.3mm) arc (-120:75:2.3mm) --++(180:2mm) node[above=-10.5pt,xshift=9.0mm,text width=1cm] {\small \textit{direct}\\\textit{call}};
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (c1) edge[bend left=20] node[above=-0.5pt,xshift=2.0mm] {\small\lstinline$yieldval$} (s1);
  \draw[-stealth,thick,shorten <=2pt,shorten >=2pt] (s1) edge[bend left=30] node[above=-0.5pt,xshift=2.0mm] {\small\lstinline$resume$} (c1);
\end{tikzpicture}
\end{multicols}
\vspace{0.2cm}

Listing \ref{list:resume-value} shows how to use the hash table coroutine
to compute the sum of the hash table values.
A new coroutine instance is started in line \ref{code:hashtable-start}
using the \texttt{hashtable} coroutine.
In the \texttt{while} loop in line \ref{code:hashtable-resume-value},
the values are extracted from the instance
until \texttt{resume} returns \texttt{false}
(subsequent calls to \texttt{resume} result in a runtime error in our implementation).
The figure on the right shows the creation of the instance,
followed by two \texttt{resume} calls.

\paratitle{Typed coroutines}
In the example in Listing \ref{list:resume-value},
the \texttt{sum} variable in line \ref{code:hashtable-sum} is integer-typed.
Therefore, the right hand of the assignment in line \ref{code:hashtable-resume-value}
must also have the integer type.
This illustrates that it is useful to reason about the type of the yielded values.

A coroutine type encodes the types $\texttt{P}_i$ of its parameters,
the return type \texttt{R},
and the \emph{yield type} \texttt{Y} of the yielded values,
also called the \emph{output type} \cite{yield-mainstream}.
Its general form is
$\texttt{(P}_1\texttt{,}\ldots\texttt{,P}_N\texttt{)\textasciitilde>(Y,R)}$
\footnote{We note that Scala allows operator syntax, such as €\textasciitilde>€,
when declaring custom data types.}.
In the following, we annotate the \texttt{dup} coroutine
from Listing \ref{list:coroutine}:

\begin{lstlisting}[language=scala,mathescape,label=list:type-coroutine-dup,captionpos=t,numbers=none,aboveskip=0.2 \baselineskip,belowskip=-0.2 \baselineskip]
val dup: Int~>(Nothing,Int) = coroutine { (x:Int) => x + x }
\end{lstlisting}

Since this coroutine does not yield any values,
its yield type is \texttt{Nothing}, the bottom type in Scala.
A coroutine \texttt{once}, which yields its argument once,
has the yield type \texttt{Int}:

\begin{lstlisting}[language=scala,mathescape,label=list:type-coroutine-once,captionpos=t,numbers=none,aboveskip=0.2 \baselineskip,belowskip=-0.2 \baselineskip]
val once: Int~>(Int,Unit) = coroutine { (x:Int) => yieldval(x) }
\end{lstlisting}

The €bucket€ and €hashtable€ coroutines
from Listings \ref{list:hash-bucket} and \ref{list:hash-table}
have the following types:

\begin{lstlisting}[language=scala,mathescape,label=list:type-coroutine-once,captionpos=t,numbers=none,aboveskip=0.2 \baselineskip,belowskip=-0.2 \baselineskip]
val bucket: List[Int]~>(Int,Unit) = ...
val hashtable: Array[List[Int]]~>(Int,Unit) = ...
\end{lstlisting}

Coroutine instances have a separate type \texttt{Y<\textasciitilde>R},
where \texttt{Y} is the yield type, and \texttt{R} is the return type.
For example, starting \texttt{once} produces an instance with the type
\texttt{Int<\textasciitilde>Unit}:

\begin{lstlisting}[language=scala,mathescape,label=list:type-coroutine-instance,captionpos=t,numbers=none,aboveskip=0.2 \baselineskip,belowskip=-0.2 \baselineskip]
val i: Int<~>Unit = once.start(7)
\end{lstlisting}

Instances of the €bucket€ and €hashtable€ coroutines
also have the type €Int<\textasciitilde>Unit€.

\paratitle{Snapshots}
We extend standard coroutines with the \texttt{snapshot} operation,
which takes a coroutine instance
and returns a duplicated instance with exactly the same execution state.

\begin{lstlisting}[language=scala,mathescape,label=list:snapshot,captionpos=t,numbers=none]
val i1: Int<~>Unit = once.start(7)
val i2: Int<~>Unit = i1.snapshot
\end{lstlisting}

In the previous example,
the coroutine instance \texttt{i1} is duplicated to \texttt{i2}.
Subsequent coroutine operations can be called independently
on the two coroutine instances.


==> related-work.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Related Work}\label{sec:related}

We organize the related work on coroutines into several categories.
We start with the origins and previous formalization approaches,
we then contrast coroutines to similar domain-specific primitives,
and conclude with the related work on continuations.
Where appropriate, we contrast our model with alternatives.
As stated in the introduction,
many features of our model have been studied already.
However, our main novelty
is that our delimited coroutines rely only on metaprogramming,
as well as augmenting coroutines with snapshots.

\textbf{Coroutine in programming languages.}
Table \ref{tab:suspension-primitives} is a brief comparative summary
of suspension primitives in different languages.
We compare type-safety, whether suspendable code blocks are first-class objects,
whether coroutines are stackful,
and if suspendable blocks can call each other without dynamic allocation.
The scope column denotes the scope in which the primitive can be used.


\begin{table}
  \caption{Comparison of Suspension Primitives in Different Languages}
  \label{tab:suspension-primitives}
  \small
  \begin{tabular}{l@{\hskip0.1cm} c@{\hskip0.15cm} c@{\hskip0.15cm} c@{\hskip0.15cm} c@{\hskip0.15cm} c@{\hskip0.15cm} c@{\hskip0.15cm}}
    \toprule
    Name&Type-safe&First-class&Stackful&Allocation-free&Scope&Snapshots\\
    \midrule
    Enumerators (C\#)             & \cmark & \xmark & \xmark & $\varnothing$ & delimited     & \xmark\\
    Generators (Python)           & \xmark & \cmark & \cmark & \xmark        & delimited     & \xmark\\
    Async (Scala, C\#)            & \cmark & \cmark & \cmark & \xmark        & delimited     & \xmark\\
    Spawn-sync (Cilk)             & \cmark & \xmark & \cmark & \cmark        & whole program & \xmark\\
    Boost (C++)                   & \cmark & \cmark & \cmark & \cmark        & delimited     & \xmark\\
    CO2 (C++)                     & \cmark & \cmark & \xmark & $\varnothing$ & delimited     & \xmark\\
    Coroutines (Lua)              & \xmark & \cmark & \cmark & \cmark        & just-in-time  & \xmark\\
    Coroutines (Kotlin)           & \cmark & \cmark & \cmark & \xmark        & delimited     & \xmark\\
    \textbf{Coroutines (Scala)}   & \cmark & \cmark & \cmark & \cmark        & delimited     & \cmark\\
  \bottomrule
\end{tabular}
\end{table}

The Kotlin language exposes coroutines
with its \texttt{suspend} and \texttt{yield} keywords
\cite{coroutines-kotlin}.
Kotlin's implementation is delimited and CPS-based,
and it translates every call to a coroutine \texttt{c}
to an allocation of a coroutine class specific to \texttt{c}.
This coroutine-specific class holds the state of the local variables.
Instances of this class are chained and form linked-list-based callstack.
Our translation approach is different in that a coroutine call
modifies an array-based call stack, and does not require an object allocation.
Currently, Kotlin coroutines do not allow snapshots,
which makes them equivalent to one-shot continuations
\cite{Moura:2009:RC:1462166.1462167}.

In the C++ community, there are two popular coroutine libraries:
Boost coroutines \cite{coroutines-boost} and CO2 \cite{coroutines-co2}.
Boost coroutines are stackful, and they expose two separate asymmetric coroutine types:
push-based coroutines, where resuming takes an input value,
and pull-based coroutines, where resuming returns an output value.
They do not support snapshots due to problems with memory safety in copying the stack.
CO2 aims to implement fast coroutines, and reports better performance than Boost,
but it supports only stackless coroutines.

\textbf{Origins and formalizations.}
The idea of coroutines dates back to Erdwinn and Conway's work on
a tape-based Cobol compiler and its separability into modules
\cite{Conway:1963:DST:366663.366704}.
Although the original use-case is no longer relevant, other use-cases emerged.
Coroutines were investigated on numerous occasions,
and initially appeared in languages such as Modula-2 \cite{wirth1985programming},
Simula \cite{Birtwhistle:1979:SB:1096934},
and BCPL \cite{journals/spe/MoodyR80}.
A detailed classification of coroutines is given
by Moura and Ierusalimschy \cite{Moura:2009:RC:1462166.1462167},
along with a formalization of asymmetric coroutines
through an operational semantics.
Moura and Ierusalimschy observed that asymmetric first-class stackful coroutines
have an equal expressive power as one-shot continuations,
but did not investigate snapshots,
which make coroutines equivalent to full continuations.
Anton and Thiemann showed that it is possible
to automatically derive type systems
for symmetric and asymmetric coroutines
by converting their reduction semantics
into equivalent functional implementations,
and then applying existing type systems
for programs with continuations \cite{Anton2010}.
James and Sabry identified the input and output types of coroutines
\cite{yield-mainstream},
where the output type corresponds
to the \textit{yield} type described in this paper.
The input type ascribes the value passed to the coroutine when it is resumed.
As a design tradeoff, we chose not to have explicit input values in our model.
First, the input type increases the verbosity of the coroutine type,
which may have practical consequences.
Second, as shown in examples from Section \ref{sec:use-cases},
the input type can be simulated with the return type of another coroutine,
which yields a writable location, and returns its value when resumed
(e.g. the \texttt{await} coroutine from Section \ref{sec:use-cases}).
Fischer et al. proposed a coroutine-based programming model
for the Java programming language,
along with the respective formal extension of Featherweight Java
\cite{Fischer:2007:TLS:1244381.1244403}.

\textbf{Domain-specific approaches.}
The need for simpler control flow
prompted the introduction of coroutine-inspired primitives
that target specific domains.
One of the early applications was data structure traversal.
Push-style traversal with \texttt{foreach} is easy,
but the caller must relinquish control,
and many applications cannot do this
(e.g. the same-fringe benchmark from Section \ref{sec:eval}).
Java-style iterators with \texttt{next} and \texttt{hasNext}
are harder to implement than a \texttt{foreach} method,
and coroutines bridge this gap.

Iterators in CLU \cite{Liskov:1977:AMC:359763.359789} are essentially coroutines --
program sections with \texttt{yield} statements
that are converted into traversal objects.
C\# inherited this approach -- its iterator type \texttt{IEnumerator} exposes
\texttt{Current} and \texttt{MoveNext} methods.
Since enumerator methods are not first class entities,
it is somewhat harder to abstract suspendable code,
as in the backtracking example from Section \ref{sec:use-cases}.
C\# enumerators are not stackful,
so the closed addressing hash table example
from the Listing \ref{list:hash-table}
must be implemented inside a single method.
Enumerators can be used for asynchronous programming,
but they require exposing \texttt{yield} in user code.
Therefore, separately from enumerators, C\# exposes async-await primitives.
Some newer languages such as Dart
similarly expose an async-await pair of primitives.

Async-Await in Scala \cite{scala-async}
is implemented using Scala's metaprogramming facilities.
Async-await programs can compose
by expressing asynchronous components as first-class \texttt{Future} objects.
The Async-Await model does not need to be stackful,
since separate modules can be expressed as separate futures.
However, reliance on futures and concurrency makes it hard
to use Async-Await generically.
For example, iterators implemented using futures
have considerable performance overheads
due to synchronization involved in creating future values.

There exist other domain-specific suspension models.
For example,
Erlang's €receive€ statement
effectively captures the program continuation
when awaiting for the inbound message \cite{programming-erlang96}.
A model similar to Scala Async was
devised to generate Rx's \texttt{Observable} values
\cite{EPFL-CONF-188383,Meijer:2012:YMD:2160718.2160735},
and the event stream composition in the reactor model
\cite{Prokopec:2017:EBB:3133850.3133865,Prokopec:2014:CAM:2637647.2637656},
as well as callbacks usages
in asynchronous programming models based on futures and flow-pools
\cite{SIP14,prokopec12flowpools,EPFL-REPORT-181098,6264/THESES,Schlatter:198208}
can be similarly simplified.
Cilk's spawn-sync model \cite{Leiserson1997} is similar to async-await,
and it is implemented as a full program transformation.
The Esterel language defines a \texttt{pause} statement
that pauses the execution, and continues it in the next event propagation cycle
\cite{Berry:1992:ESP:147276.147279}.
Behaviour trees \cite{6907656} are AI algorithms used to simulate agents --
they essentially behave as AST interpreters with yield statements.

\textbf{Generators.}
Dynamic languages often support \emph{generators},
which are essentially untyped asymmetric coroutines.
A Python generator instance \cite{pep-generators}
exposes only the \texttt{next} method (an equivalent of \texttt{resume}),
which throws a \texttt{StopIteration} error when it completes.
In practice, Python generators are mostly used for \emph{list comprehensions},
as programmers find it verbose to handle \texttt{StopIteration} errors.
Newer Python versions allow stackful generators \cite{pep-delegation}
with the \texttt{yield from} statement,
which is implemented as syntactic sugar around basic generators
that chains the \texttt{resume} points instead of using call stacks.
ECMAScript 6 generators are similar to Python's generators.
Lua coroutines bear the most similarity
with the coroutine formulation in this paper \cite{moura.04.jucs},
with several differences.
First, Lua coroutines are not statically typed.
While this is less safe,
it has the advantage of reduced syntactic burden.
Second, Lua coroutines are created from function values dynamically.
This is convenient, but requires additional JIT optimizations to be efficient.

\textbf{Transformation-based continuations.}
Continuations are closely related to coroutines,
and with the addition of \texttt{snapshot}
the two can express the same programs.
Scheme supports programming with continuations via the \texttt{call/cc} operator,
which has a similar role as \texttt{shift}
in shift-reset delimited continuations
\cite{Danvy:1990:AC:91556.91622,Asai:2017:SCT:3175493.3162069}.
In several different contexts,
it was shown that continuations subsume other control constructs
such as exception handling, backtracking, and coroutines.
Nonetheless, most programming languages do not support continuations today.
It is somewhat difficult to provide an efficient implementation of continuations,
since the captured continuations must be callable more than once.
One approach to continuations is to transform the program
to continuation-passing style \cite{Sussman:1998:SIE:609145.609186}.
Scala's continuations \cite{Rompf:2009:IFP:1631687.1596596}
implement delimited shift-reset continuations with a CPS transform.
The downside of CPS is the risk of stack overflows
in runtimes in the absence of tail-call optimization, which is the case of JVM.

Optimizing compilers tend to be tailored to the workloads that appear in practice.
For example, it was shown that optimizations such as
inlining, escape analysis, loop unrolling and devirtualization
make most collection programs run nearly optimally
\cite{Prokopec:2017:MCO:3136000.3136002,7092728,Prokopec:196627,Sujeeth:2013:CRC:2524984.2524988,prokopec11}.
However, abstraction overheads associated with coroutines are somewhat new,
and are not addressed by most compilers.
For this reason, compile-time transformations of coroutine-heavy workloads
typically produce slower programs compared to their runtime-based counterparts.
We postulate that targeted high-level JIT optimizations
could significantly narrow this gap.

\textbf{Runtime-based continuations.}
There were several attempts to provide runtime continuation support for the JVM,
ranging from Ovm implementations \cite{LAMP-CONF-2007-002}
based on \texttt{call/cc},
to JVM extensions \cite{Stadler:2009:LCJ:1596655.1596679},
based on the \texttt{capture} and \texttt{resume} primitives.
While runtime continuations are not delimited and can be made very efficient,
maintenance pressure and portability requirements
prevented these implementations from becoming a part of official JVM releases.
An alternative, less demanding approach relies only on stack introspection facilities
of the host runtime \cite{Pettyjohn:2005:CGS:1090189.1086393}.
There exists a program transformation that relies on exception-handling
to capture the stack \cite{Sekiguchi:2001:PIC:647332.722736}.
Here, before calling the continuation,
the saved state is used in method calls to rebuild the stack.
This works well for continuations,
where the stack must be copied anyway,
but may be too costly for coroutine \texttt{resume}.
Bruggeman et al. observed that many use cases
call the continuation only once and can avoid the copying overhead,
which lead to \textit{one-shot continuations}
\cite{Bruggeman:1996:RCP:231379.231395}.
One-shot continuations are akin to coroutines without snapshots.

\textbf{Other related constructs.}
Coroutines are sometimes confused with \emph{goroutines},
which are lightweight threads in the Go language.
While coroutines can be used to encode goroutines,
the converse encoding is not as efficient,
as goroutines involve message passing.


==> subtyping-rules.tex <==

\begin{minipage}[t]{1.6cm}
\small
$\quad \texttt{S<:S} \,$
\\
\hspace{5mm}
\textsc{(S-Refl)}
\noindent
\end{minipage}
\begin{minipage}{2.4cm}
\small
\infrule[\textsc{S-Trans}]
{ \texttt{S<:U} \quad \texttt{U<:T}
}
{ \texttt{S<:T}
}
\noindent
\end{minipage}
\begin{minipage}{2.4cm}
\small
\infrule[\textsc{S-Arrow}]
{ \texttt{T}_1\texttt{<:S}_1 \quad \texttt{S}_2\texttt{<:T}_2
}
{ \texttt{S}_1\texttt{=>S}_2\texttt{<:T}_1\texttt{=>T}_2
}
\noindent
\end{minipage}
\begin{minipage}{3.2cm}
\small
\infrule[\textsc{S-Instance}]
{ \quad \texttt{S}_1\texttt{<:T}_1 \quad \texttt{S}_2\texttt{<:T}_2
}
{ \texttt{S}_1\leftrightsquigarrow\texttt{S}_2
\texttt{<:T}_1\leftrightsquigarrow\texttt{T}_2
}
\noindent
\end{minipage}
\begin{minipage}{4.0cm}
\small
\infrule[\textsc{S-Coroutine}]
{ \texttt{T}_1\texttt{<:S}_1 \quad
\texttt{S}_y\texttt{<:T}_y \quad
\texttt{S}_2\texttt{<:T}_2
}
{ \texttt{S}_1 \overset{\texttt{S}_y}{\rightsquigarrow} \texttt{S}_2
\texttt{<:T}_1 \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2
}
\noindent
\end{minipage}


==> transformation-discussion.tex <==

\section{Transformation of $\lambda_\leadsto$ to simply typed lambda calculus with references}
\label{sec:simply-typed-coroutines-transformation}

In this section, we analyze the formal transformation rules
shown in Fig. \ref{fig:appendix-transformation}.
As stated in the main paper,
the transformation is a delimited CPS transform,
where the translation of each term assumes the existence
of a continuation of the body of the current coroutine,
represented by the type
$
\varkappa\texttt{[T},\texttt{T}_y,\texttt{T}_r\texttt{]}
\triangleq
\texttt{T=>Out[T}_y,\texttt{T}_r\texttt{]}
$.

The key idea in the described CPS transformation is
to separate the return type (and the transformation) of the coroutine
from the return type of its caller.
This way, the coroutine does not need to be compiled
with the knowledge about the return type of the enclosing program,
and does not need to be polymorphic in the return type of the enclosing program.
To accomplish this separation,
we define a special \emph{store function type}
$
\sigma\texttt{[T}_y,\texttt{T}_r\texttt{]}
\triangleq
\varkappa\texttt{[Unit},\texttt{T}_y,\texttt{T}_r\texttt{]=>Unit}
$ --
a function that knows how to store the coroutine's continuation.

Each term inside a coroutine is then translated
to a function that takes a store function,
and the continuation of the current term.
The input type \texttt{T} of the continuation of type
$\varkappa\texttt{[T},\texttt{T}_y,\texttt{T}_r\texttt{]=>Unit}$
must correspond to the type of the value that the term evaluates to
(which is usually the same as the type of that term in the source language,
but of course differs if the original term was a coroutine or a coroutine instance).
The abbreviation for the transformed term is
$
\xi(\texttt{[T}_y,\texttt{T}_r,\texttt{T},\texttt{t})
\triangleq
\tau(
\texttt{(s:}\sigma\texttt{[T}_y,\texttt{T}_r\texttt{]}\texttt{)=>}
\texttt{(k:}\varkappa\texttt{[T},\texttt{T}_y,\texttt{T}_r\texttt{]}\texttt{)=>}
\texttt{t}
)
$.
The source term may itself mention types from the source language.
Therefore, the type substitution $\tau$
serves to replace the coroutine and coroutine instance types
that are mentioned in the source term,
and is defined as:
$
\tau(\texttt{t})
\triangleq
\forall \texttt{T}_1,\texttt{T}_y,\texttt{T}_2
[
\texttt{(x:T}_1\texttt{)} \overset{\texttt{T}_y}{\rightsquigarrow} \texttt{T}_2
\mapsto
\gamma\texttt{[T}_1,\texttt{T}_y,\texttt{T}_2\texttt{]}
]
[
\texttt{T}_y \leftrightsquigarrow \texttt{T}_2
\mapsto
\rho\texttt{[T}_y,\texttt{T}_2\texttt{]}
]
\texttt{t}
$.

Note, finally,
that a coroutine of type
$\texttt{T}_1\overset{\texttt{T}_y}{\rightsquigarrow}\texttt{T}_2$
translates to the $\gamma$ value in the target language,
whose type is defined as follows:
$
\gamma\texttt{[T}_1,\texttt{T}_y,\texttt{T}_r\texttt{]}
\triangleq
\sigma\texttt{[T}_y,\texttt{T}_r\texttt{]=>T}_1
\texttt{=>Out[T}_y\texttt{,T}_r\texttt{]}
$.
This means that a coroutine can be invoked when provided
with a store function (so that it knows how to store its state),
and it will return an \texttt{Out} value,
which models either a yield or a return.
In the same spirit,
a coroutine instance of type
$\texttt{T}_y\leftrightsquigarrow\texttt{T}_2$
is translated into a $\rho$ value,
whose type is defined as follows:
$
\rho\texttt{[T}_y,\texttt{T}_r\texttt{]}
\triangleq
\texttt{Ref[}\varkappa\texttt{[Unit},\texttt{T}_y,\texttt{T}_r\texttt{]]}
$.

Before going through the transformation rules,
we introduce several additional definitions:

\begin{definition}\label{def:output-transformer-type}
The function type
$
\varphi\texttt{[T}_y,\texttt{T}_r,\texttt{T}_q\texttt{]}
\triangleq
\texttt{Out[T}_y\texttt{,T}_r\texttt{]=>}
\texttt{Out[T}_y\texttt{,T}_q\texttt{]}
$
is called the \emph{output transformer type}.
\end{definition}

The output transformer functions are used
in the translation of coroutine calls,
and serve to modify the return type of the continuation.
We additionally define two auxiliary abbreviations,
which will be used when storing the evaluation state.

\begin{definition}\label{def:helper-functions}
The \emph{output transformer} $\Phi$
is a function that,
for a given continuation value \texttt{k} of type
$\varkappa\texttt{[T}_r,\texttt{T}_y,\texttt{T}_q\texttt{]}$,
maps a value of type
$\texttt{Out[T}_y\texttt{,T}_r\texttt{]}$
to a value of type
$\texttt{Out[T}_y\texttt{,T}_q\texttt{]}$,
and is defined as follows:

{
\centering
\small
$
\Phi(\texttt{T}_y, \texttt{T}_r, \texttt{T}_q, \texttt{k})
$
\normalsize
$
\triangleq
$

\small
$
\texttt{(x:Out[T}_y\texttt{,T}_r\texttt{])=>}
\texttt{x match\{case Ret(x)=>k(x);case Yield(x)=>Yield(x);case Term=>Term\}}
$
\normalsize

}

The \emph{store function constructor} $\psi$
is a function that
maps a reference \texttt{x} of type
$\rho\texttt{[T}_y,\texttt{T}_r\texttt{]}$
to a store function of type
$\sigma\texttt{[T}_y,\texttt{T}_r\texttt{]}$,
and is defined as follows:

{
\centering
\small
$
\psi(\texttt{T}_y, \texttt{T}_r, \texttt{x})
$
\normalsize
$
\triangleq
$
\small
$
\texttt{(x:}\rho\texttt{[T}_y,\texttt{T}_r\texttt{]}\texttt{)=>}
\texttt{(k:}\varkappa\texttt{[Unit},\texttt{T}_y,\texttt{T}_r\texttt{])=>x:=k}
$
\normalsize

}

\qed
\end{definition}

Next, we make the typing rules shorter by dropping $\Sigma$ from the typing relation:

\begin{definition}
The abbreviated typing relation is:
$\Gamma \vdash \texttt{t:T} | \texttt{T}_y$
$\triangleq$
$\forall \Sigma, \Sigma | \Gamma \vdash \texttt{t:T} | \texttt{T}_y$.
\qed
\end{definition}

\begin{definition}[Transformation relation]
The \emph{transformation relation} is a five place relation
$\Gamma \vdash \texttt{T}_y | \texttt{T}_r | \texttt{t} \rightarrow \texttt{t}'$,
where $\Gamma$ is the typing context,
$\texttt{T}_y$ is the yield type of the current term,
$\texttt{T}_r$ is the return type of the enclosing coroutine,
$\texttt{t}$ is the term in the source language,
and $\texttt{t}'$ is the term in the target language.
When $\texttt{T}_y \neq \bot$ and $\texttt{T}_r \neq \bot$,
this relation is inductively defined
according to Figures \ref{fig:appendix-transformation}
and \ref{fig:appendix-transformation-outside}.
\qed
\end{definition}


\begin{figure}[t]
\small
\centering
\hspace*{-1.2cm}
\input{transformation-rules.tex}
\caption{
Transformation of coroutines in $\lambda_\leadsto$
to a simply typed lambda calculus with references
}
\label{fig:appendix-transformation}
\end{figure}

We now describe the rules in Fig. \ref{fig:appendix-transformation}.
All of these rules assume that we are inside a body of some coroutine,
which has the yield type $\texttt{T}_y$ and a return type $\texttt{T}_r$
(outside of a body of a coroutine, as we show shortly,
there is no need for a CPS transform).
Consider the two simplest rules, \textsc{X-Var} and \textsc{X-Unit}.
The transformed term simply calls the continuation by passing the value,
either a variable or a \texttt{Unit} value, to the continuation.
The \textsc{X-App} rule assumes that the
subterm $\texttt{t}_1$ evaluates to a function $\texttt{t}_1'$,
and $\texttt{t}_2$ evaluates to $\texttt{t}_2'$.
Consider what happens after both $\texttt{t}_1'$ and $\texttt{t}_2'$
produce values $\texttt{x}_1$ and $\texttt{x}_2$, respectively.
The next step in the evaluation is to simply apply
$\texttt{x}_1$ to $\texttt{x}_2$.
However, the application $\texttt{x}_1\texttt{(x}_2\texttt{)}$
is a continuation for the term $\texttt{t}_2'$,
whose evaluation is itself a continuation for $\texttt{t}_1'$.
The transformation of $\texttt{t}_1\texttt{(t}_2\texttt{)}$
requires chaining these continuations together
as described in the \textsc{X-App} rule.

Next, consider the \textsc{X-Coroutine} rule,
which relies on the assumption that the coroutine body \texttt{t}
translates to a function $\texttt{t}'$
under the extended typing context $\Gamma , \texttt{x:T}_1$.
The transformed term has the $\gamma$ type --
it takes a store function and an argument.
The store function is passed to $\texttt{t}'$,
along with a continuation that
stores a terminated continuation \texttt{()=>Term},
and wraps the result of $\texttt{t}'$
into a $\texttt{Ret}$ value.
The resulting $\gamma$ value is then passed
to the continuation of the definition site of the coroutine
(which is itself assumed to be inside another coroutine).

A coroutine created this way is, by rule \textsc{X-Start}, \emph{called}
by first allocating a reference \texttt{x} for the evaluation state
(term $\texttt{q}_1$),
then assigning the continuation of the coroutine
into the reference \texttt{x} (term $\texttt{q}_2$),
and finally, passing the reference \texttt{x}
to the continuation \texttt{k} (term $\texttt{p}$).
Note that the abbreviation $\psi$ is used to construct
the store function -- this is just a store function that assigns
the continuation to the reference.

Consider now the \textsc{X-Yield} rule.
This rule continues the evaluation of the subterm $\texttt{t}$
by passing the current continuation \texttt{k}
(whose type must be $\gamma\texttt{[Unit},\texttt{T}_y,\texttt{T}_r\texttt{]}$,
since \texttt{yield} reduced to a \texttt{Unit} value)
to the store function.
As we just saw with the \textsc{X-Start} rule,
the store function could, for example, store the continuation into a reference
(but it can do other things too, as we show shortly).
The transformation of the \texttt{yield} then returns a \texttt{Yield} value.

We are now ready to take a look at the \textsc{X-AppCor} rule.
A transformed coroutine application
first constructs a mapping \texttt{f}
between output type of the callee coroutine
and the output type of the caller coroutine (term $\texttt{q}_1$),
whose type is defined as follows:
$
\varphi\texttt{[T}_y,\texttt{T}_r,\texttt{T}_q\texttt{]}
\triangleq
\texttt{Out[T}_y\texttt{,T}_r\texttt{]=>}
\texttt{Out[T}_y\texttt{,T}_q\texttt{]}
$.
This mapping is defined by the abbreviation $\Phi$
(defined in \ref{def:helper-functions},
which just forwards \texttt{Yield} values.
However, if the callee returns a \texttt{Ret(x)} value,
then the wrapped value \texttt{x} is passed
to the continuation \texttt{k} of the callee
(which itself must return the correctly typed \texttt{Ret} value).

Next, the coroutine application must
create a new store function $\texttt{s}'$
with the appropriate type (term $\texttt{q}_2$).
This new store function
$\texttt{s}'$ passes a modified continuation to
the store function $\texttt{s}$ of the callee,
such that the modified continuation calls
the callee's continuation $\texttt{k}'$,
and then adapts the result using the mapping \texttt{f}.
Finally,
the transformed coroutine $\texttt{x}_1$
is invoked with the new store function $\texttt{s}'$,
and the result transformed using \texttt{f}
(term $\texttt{q}_3$).

Having seen \textsc{X-AppCor},
rules \textsc{X-Snapshot} and \textsc{X-Resume} should be self-explanatory.
The \texttt{snapshot} term
translates to the cloning the $\rho$ reference,
and the \texttt{resume} term
translates to dereferencing the continuation from the $\rho$ reference,
invoking it, and calling the correct handler, case-wise.

We deliberately left \textsc{X-Abs} as the last rule in our discussion.
Recall that the standard abstraction term effectively \emph{resets} the yield type
back to $\bot$ --
the standard abstraction term \emph{cannot} yield back to its callsite.
For this reason, the \textsc{X-Abs} rule
transforms the body of an abstraction term
under the assumption that the enclosing yield and return types are both $\bot$.
However, the fineprint present in each transformation rule
is that the $\texttt{T}_y$ \emph{must not} be $\bot$ --
the transformation rules shown so far cannot translate such a term!

The conclusion is that we need a second set of rules
that govern the transformation \emph{outside} of coroutines.
Naturally, these rules do not require a CPS transform,
and they leave most of the program as is --
they deal with coroutine definitions
and handling coroutine instances.
In particular, there is no analogue for the \textsc{X-AppCor}
and \textsc{X-Yield} rules --
a well-typed user program cannot yield or call coroutines
outside of a lexical scope of a coroutine.

\begin{figure}[t]
\small
\centering
\hspace*{-1.2cm}
\input{transformation-rules-outside.tex}
\caption{
Transformation of non-yielding terms in $\lambda_\leadsto$
to a simply typed lambda calculus with references
}
\label{fig:appendix-transformation-outside}
\end{figure}

The rules in Fig. \ref{fig:appendix-transformation-outside},
whose name starts with \textsc{X-Free},
transform non-yielding terms.
They are analogous to the coroutine transformation rules.
When the yield and return types are $\bot$,
the transformation produces a normal term instead of a $\xi$ expression --
the logic inside each translated coroutine-related operation stays the same,
but the value is not being passed to a continuation.
To switch to the CPS transform from Fig. \ref{fig:appendix-transformation},
the transformation must apply the \textsc{X-FreeCoroutine} rule.

Note, finally, that the only terms that are different
after the transformation are those that mention
elements of the $\lambda_\leadsto$ calculus syntax.
Any term that makes no mention of
$\lambda_\leadsto$-specific terms is left unchanged.
This shows that the transformation is both selective,
and that it does not require the recompilation of legacy programs
that use coroutines.
This was one of the design goals mentioned in the introduction.
Furthermore,
a selective metaprogramming API \cite{Burmako:2013:SML:2489837.2489840}
is a good implementation vehicle for this type of a transformation,
since the transformation can be applied to delimited parts of the program,
without a full program transformation.


==> use-case-implementations.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Additional coroutine-based implementations}

In Section \ref{sec:use-cases},
we showed how coroutines simplify actors and Rx streams.
In this section, we show the coroutine-based implementations for these use-cases.

\textbf{Actors.}
Since JVM does not have continuations,
actor frameworks are unable to implement exact Erlang-style semantics,
in which the €receive€ statement can be called anywhere in the actor.
Instead, frameworks like Akka expose a top-level €receive€ method \cite{akka},
which returns a partial function used to handle messages.
This function can be swapped during the actor lifetime
with the €become€ statement.
In the example from Listing \ref{list:actor-erlang},
we used a €receive€ statement
that suspends in the middle of the actor and awaits a message.
We now show its implementation using coroutines.

The core idea is to implement a €recv€ coroutine
(we call it €recv€ to disambiguate from Akka's €receive€ function),
which yields a partial function that represents the continuation of the actor.
The resume-site can then call €become€
to hot-swap Akka's top-level €receive€ handler
with the yielded partial function.

In Listing \ref{list:erlang-impl},
we first define an auxiliary type €Rec€,
which describes a partial function that can take €Any€ message objects.
The method €act€ declares an Erlang-style actor --
it takes a coroutine that may yield
partial functions of the €Rec€ type,
which describe how to process the next message.
The €act€ method starts an instance of the input coroutine,
and resumes it inside a recursive €loop€ function.
The instance potentially calls the €recv€ method, which yields.
When this happens,
€act€ extends the yielded partial function with the €andThen€ combinator
which recursively resumes the coroutine instance.
This chained partial function is passed to €become€,
which tells Akka to run the chained function when a message arrives.

The €recv€ is a coroutine that yields the €Rec€ function
and returns a message of type €Any€ -- the actor definition must then match this value.
The implementation of €recv€
declares a local variable €res€ in which the incoming message is stored
by the yielded partial function.
After €recv€ gets resumed, €act€ will have already called the yielded function,
which will have written the message to €res€,
so that it can be returned to the actor that invoked €recv€.

\begin{lstlisting}[label=list:erlang-impl,caption={Erlang-style actor implementation},language=scala,mathescape,captionpos=t]
type Rec = PartialFunction[Any, Unit]
def act(c: () ~> (Rec, Unit)) = Actor { self =>
  val i = c.start()
  def loop() =
    if (i.resume) self.become(i.value.andThen(loop))
    else self.stop()
  loop()
}
val recv: () ~> (Rec, Any) = coroutine { () =>
  var res: Any = _
  yieldval({ case x => res = x })
  res
}
\end{lstlisting}


\textbf{Event streams.}
Event streams expose the €onEvent€ method,
similar to €onSuccess€ on futures.
The €onEvent€ method takes a callback
that is invoked when the next event arrives.
As shown in Listing \ref{list:events-coroutines}, it is much more convenient 
to extract an event in the direct-style by invoking a €get€ statement,
instead of installing a callback.

In Listing \ref{list:reactors},
we implement the method €get€ on the event stream of type €Events[T]€.
We declare a type alias €Install€
that represents a function that installs a callback to the event stream.
When an €Install€ function is invoked with a function €f€,
the function €f€ is passed as a callback to some event stream.

The €react€ method is similar to the €act€ method for actors --
it delimits the suspendable part of the event-driven program.
The €react€ method starts and resumes the coroutine.
When the coroutine yields an €Install€ function,
the €react€ method uses the €Install€ function
to install a callback that recursively resumes the coroutine.

The €get€ method is called by the users to extract
the next event out of a reactor's event stream.
Its implementation yields an €Install€ function that installs the callback
on the event stream by calling €onEvent€.
The event stream callback sets the result variable
and invokes the continuation function €f€.
This technique is similar to the actor use-case,
but the difference is that it abstracts over what €become€ is.

\begin{lstlisting}[label=list:reactors,caption={Direct-style event streams},language=scala,mathescape,captionpos=t]
type Install = (() => Unit) => Unit
def react(c: () ~> (Install, Unit)) = {
  val i = c.start()
  def loop(): Unit = if (i.resume) i.value(loop)
  loop()
}
def get[T](e: Events[T]): () ~> (Install, T) = coroutine { () =>
  var res: T = _
  val install = (f: () => Unit) => e.onEvent(x => {
    res = x
    f()
  })
  yieldval(install)
  res
}
\end{lstlisting}

We note that, in this example,
it might have been more natural to yield an event stream directly,
instead of yielding €Install€ functions.
However, the event stream is parametric in the type of events,
and the coroutine would always have to yield event streams
of the same event type.
The €Install€ function hides the event type inside the €get€ function,
and allows a more flexible event stream API.


==> use-cases.tex <==
%!TEX root = coroutines-ecoop.tex

\section{Use Cases}\label{sec:use-cases}

Having explained what type-safe, delimited and stackful means,
we motivate our design choices with observations and concrete examples.
The goal of this section is to show how specific primitives
help express other kinds of suspendable computations.

\begin{observation}
Stackful coroutines allow composing suspendable software modules.
\end{observation}

The hash table example from Listings \ref{list:hash-bucket} and \ref{list:hash-table}
demonstrated why composing different modules is useful,
and the remaining examples in this section reinforce this.

\begin{observation}
Stackful coroutines simplify the interaction with recursive data types.
\end{observation}

\paratitle{Iterators}
Data structure iterators are one of the earliest applications of coroutines
\cite{Liskov:1977:AMC:359763.359789}.
We can implement an iterator coroutine \texttt{it} for binary trees
as shown in Listing \ref{list:iterator}:

\begin{multicols}{2}
\begin{lstlisting}[caption={Tree iterator implementation},language=scala,mathescape,label=list:iterator,captionpos=t]
val it = coroutine { (t:Tree) =>
  if (t.fst != null) it(t.fst)
  yieldval(t.element)
  if (t.snd != null) it(t.snd) }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Symmetric coroutine},label=list:symmetric-run,language=scala,captionpos=t,abovecaptionskip=-\medskipamount,belowskip=-0.4 \baselineskip]
type Sym[R] = Sym[R] <~> R
def run(i: Sym[R]): R =
  if (i.resume) run(i.value)
  else i.result
\end{lstlisting}
\end{multicols}

% In Section \ref{sec:eval}, we implement and benchmark similar iterators
% for graph data structures.

\begin{observation}
Asymmetric coroutines can be used to express symmetric coroutines.
\end{observation}

\paratitle{Symmetric coroutines}
In a programming model with symmetric coroutines,
there is no \texttt{resume} primitive.
Instead, a symmetric coroutine always yields the next coroutine instance
from which to continue.
As shown in Listing \ref{list:symmetric-run},
a symmetric coroutine instance can be expressed
with the recursive type \texttt{Sym[R]}.
This was observed before \cite{Moura:2009:RC:1462166.1462167}.

\begin{observation}
Coroutine calls and coroutine return values,
together with the \texttt{yieldval} primitive,
allow encoding alternative forms of suspension primitives.
\end{observation}

The core idea is to express a suspension primitive as a special coroutine.
This coroutine yields a value that allows the resume-site to communicate back.
Once resumed, the coroutine \emph{returns another value} to its caller coroutine.
We show several examples of this pattern.

\paratitle{Async-await}
A future is an entity that initially does not hold a value,
but may asynchronously attain it at a later point.
Future APIs are usually callback-based --
the code that handles the future value is provided as a function.
In Scala, type \texttt{Future} exposes the \texttt{onSuccess} method,
which takes a callback and calls it once the value is available,
and \texttt{value}, which can be used to access the future value if available.
\texttt{Promise} is the future's writing end, and it exposes \texttt{success},
which sets the value of the corresponding future at most once \cite{SIP14}.

\begin{multicols}{2}
\begin{lstlisting}[caption={Callback-style API},language=scala,label=list:future-callback,captionpos=t,abovecaptionskip=-\medskipamount]
val token: Future[Token] =
  authenticate()
token.onSuccess { t =>
  val session: Future[Session] =
    sessionFor(t)
  session.onSuccess(useSession)
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Async-await-style API},language=scala,label=list:future-async,captionpos=t]
async {
  val token: Token =
    await { authenticate() }
  val session: Session =
    await { sessionFor(token) }
  useSession(session)
}
\end{lstlisting}
\end{multicols}

In Listing \ref{list:future-callback},
the \texttt{authenticate} method returns a future
with a \verb$Token$ value.
Once the token arrives,
the callback function (passed to the \verb$onSuccess$ method)
calls \verb$sessionFor$ to obtain a session future.
The program continues in the \verb$useSession$ callback.
The direct-style async-await version,
shown in Listing \ref{list:future-async},
relies on the \texttt{async} statement, which starts asynchronous computations,
and the \texttt{await}, which suspends until a value is available.

We use coroutines to replicate Scala's Async framework \cite{scala-async}.
The \texttt{await} method emulates the suspension primitive --
it creates a coroutine that yields a future and returns its value.
It assumes that the resume-site
invokes \texttt{resume} only \emph{after} the future is completed.

\begin{lstlisting}[caption={The \texttt{await} primitive},language=scala,mathescape,label=list:async-await,captionpos=t]
def await[T]: Future[T] ~> (Future[T], T) =
  coroutine { (f: Future[T]) => yieldval(f); f.value }
\end{lstlisting}

The \texttt{async} method interacts with \texttt{await}
from the resume-site.
For a given computation \texttt{b},
it starts an instance, and executes it asynchronously in a \texttt{Future}.
Whenever the computation \texttt{b} yields a future,
a callback is recursively installed.
If \texttt{resume} returns \texttt{false},
the resulting future is completed with the evaluation result of \texttt{b}
(\texttt{async} itself must return a future).

\begin{lstlisting}[caption={The \texttt{async} primitive},language=scala,mathescape,label=list:async-await,captionpos=t]
def async[R](b: () ~> (Future[Any], R)): Future[R] = {
  val i = b.start()
  val p = new Promise[R]
  @tailrec def loop(): Unit =
    if (i.resume) i.value.onSuccess(loop) else p.success(i.result)
  Future { loop() }
  p.future
}
\end{lstlisting}

\paratitle{Erlang-style actors}
Actor frameworks for the JVM are unable to implement exact Erlang-style semantics,
in which the \texttt{receive} statement can be called anywhere in the actor
\cite{Haller:2009:SAU:1496391.1496422}.
For example, Akka exposes a top-level \texttt{receive} method \cite{akka},
which returns a partial function used to handle messages.
This function can be swapped with the \texttt{become} statement.

Listing \ref{list:actor-akka} shows
a minimal Akka actor example that implements a server.
The server starts its execution in the \texttt{receive} method,
which awaits a password from the user.
If the password is correct,
the top-level event-handling loop becomes the \texttt{loggedIn} method,
which accepts GET requests.
When the \texttt{Logout} message arrives, the actor stops.
Listing \ref{list:actor-erlang} shows an equivalent Erlang-style actor,
in which the control flow is more apparent.
The \texttt{receive} method has the role of a suspension primitive --
it pauses the actor until a message arrives.

\begin{multicols}{2}
\begin{lstlisting}[caption={Akka-style actor},language=scala,label=list:actor-akka,captionpos=t,abovecaptionskip=-\medskipamount]
class Server extends Actor {
  def receive = {
    case Login(pass) =>
      assert(isCorrect(pass))
      become(loggedIn) }
  def loggedIn = {
    case Get(url) => serve(url)
    case Logout() => stop() } }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Erlang-style actor},language=scala,label=list:actor-erlang,captionpos=t]
def server() = {
  val Login(pass) = receive()
  assert(isCorrect(pass))
  while (true) receive() match {
    case Get(url) => serve(url)
    case Logout() => stop()
  }
}
\end{lstlisting}
\end{multicols}

As shown in the appendix,
the \texttt{receive} coroutine follows a similar pattern as async-await --
\texttt{receive} yields an object into which
the top-level loop can insert the message.

\paratitle{Event streams}
First-class Rx-style event streams \cite{Meijer:2012:YMD:2160718.2160735}
expose a set of declarative transformation combinators.
As an example, consider how to collect a sequence of points when dragging the mouse.
The mouse events are represented as an event stream value.
Dragging starts when the mouse is pressed down, and ends when released.
In Listing \ref{list:events-rx},
the \texttt{after} combinator removes a prefix of events,
and \texttt{until} removes a suffix.
The first drag event's \texttt{onEvent} callback
creates a \texttt{Curve} object, and the last event saves the curve.

\begin{multicols}{2}
\begin{lstlisting}[caption={Rx-style streams},language=scala,label=list:events-rx,captionpos=t,abovecaptionskip=-\medskipamount]
val drag = mouse.after(_.isDown)
  .until(_.isUp)
drag.first.onEvent { e =>
  val c = new Curve(e.x, e.y)
  drag.onEvent(
    e => c.add(e.x, e.y))
  drag.last.onEvent(
    e => saveCurve(c)) }
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Direct-style streams},language=scala,label=list:events-coroutines,captionpos=t]
var e = mouse.get
while (!e.isDown) e = mouse.get
val c = new Curve(e.x, e.y)
while (e.isDown) {
  e = mouse.get
  c.add(e.x, e.y)
}
saveCurve(c)
\end{lstlisting}
\end{multicols}

The equivalent direct-style program in Listing \ref{list:events-coroutines}
uses the \texttt{get} coroutine to suspend the program until an event arrives.
We show the implementation of \texttt{get} in the appendix.

\paratitle{Oz-style single-assignment variables}
A variable in the Oz language \cite{VanRoy:2004:CTM:983087}
can be assigned only once.
Reading a single-assignment variable
suspends execution until some other thread assigns a value.
Assigning a value to the variable more than once is an error.

\begin{multicols}{2}
\begin{lstlisting}[caption={Oz-style variable read},language=scala,label=list:oz1,captionpos=t,abovecaptionskip=-\medskipamount]
@volatile var state: AnyRef =
  List.empty()

val get = coroutine { () =>
  if (READ(state).is[List])
    yieldval(this)`\label{code:get-read}`
  READ(state).as[ElemType]
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Oz-style variable write},language=scala,label=list:oz2,captionpos=t]
@tailrec def set(y: ElemType) {
  val x = READ(state)
  if (x.is[List]) {
    if (CAS(state, x, y))
      for (i <- x.as[List])
        schedule(i)
    else set(y)
  } else throw Reassigned }
\end{lstlisting}
\end{multicols}

Internally, a single-assignment variable has some \texttt{state},
which is either the list of suspended threads or a value.
When \texttt{get} from the Listing \ref{list:oz1} is called,
\texttt{state} is atomically read in line \ref{code:get-read}.
If the state is a list,
coroutine is yielded to the scheduler,
which atomically adds the new suspended thread to the list (not shown).
The coroutine is resumed when the value becomes available --
method \texttt{set} in Listing \ref{list:oz2}
tries to atomically replace the list
with the value of type \texttt{ElemType}.
If successful, it schedules the suspended threads for execution.

\begin{observation}
Snapshots enable backtracking and allow emulating full continuations.
\end{observation}

\paratitle{Backtracking}
Testing frameworks such as ScalaCheck \cite{scalacheck}
rely on backtracking to systematically explore the test parameter space.
ScalaCheck uses a monadic-style API to compose the parameter generators.
Listing \ref{list:scalacheck-monadic} shows a ScalaCheck-style test
that first creates a generator for number pairs
in a Scala \texttt{for}-comprehension,
and then uses the generator in a commutativity test.
The \texttt{pairs} generator is created from the intrinsic
\texttt{ints} generator.

In the direct-style variant in Listing \ref{list:scalacheck-direct},
the \texttt{ints} generator
is a coroutine that yields and captures the execution snapshot.
Therefore, it can be called from anywhere inside the test.

\begin{multicols}{2}
\begin{lstlisting}[caption={Monadic ScalaCheck test},language=scala,label=list:scalacheck-monadic,captionpos=t,abovecaptionskip=-\medskipamount,showlines=true]
val pairs =
  for {
    x <- ints(0 until MAX_INT)
    y <- ints(0 until MAX_INT)
  } yield (x, y)

forAll(pairs) { pair =>
  val (a, b) = pair
  assert(a * b == b * a)
}

\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Direct-style ScalaCheck test},language=scala,label=list:scalacheck-direct,captionpos=t,showlines=true,belowskip=-0.15 \baselineskip]
test {
  val a = ints(0 until MAX_INT)
  val b = ints(0 until MAX_INT)
  assert(a * b == b * a)
}
\end{lstlisting}
\begin{lstlisting}[caption={Positive-definite matrix test},language=scala,label=list:scalacheck-modularized,captionpos=t,showlines=true,aboveskip=-0.15 \baselineskip]
val pd = coroutine { (m:Mat) =>
  val x = nonZeroVector(m.size)
  assert(x.t * m * x > 0)
}
\end{lstlisting}
\end{multicols}

Moreover, generator late-binding allows modularizing the properties.
Listing \ref{list:scalacheck-modularized}
shows a modular \emph{positive-definite} matrix property \texttt{pd}:
given a matrix $M$, value $x^T M x$ is positive for any non-zero vector $x$.
The \texttt{pd} coroutine can be called from within other tests.
Importantly, note that the vector \texttt{x}
is generated \emph{from within} the test.
This is hard to achieve in the standard ScalaCheck tests,
since their generators require prior knowledge about the vector \texttt{x}.

Consider implementing the \texttt{test} and the \texttt{ints} primitives
from Listing \ref{list:scalacheck-direct}.
The key idea is as follows:
each time a test calls a generator,
it suspends and yields a list of environment setters.
Each environment setter is a function
that prepares a value to return from the generator.
The resume-site runs each environment setter,
creates a snapshot and resumes it.

\begin{multicols}{2}
\begin{lstlisting}[caption={Direct-style ScalaCheck},label=list:backtrack,language=scala,mathescape,captionpos=t]
type Test =
  () ~> (List[() => Unit], Unit)

type Instance =
  List[() => Unit] <~> Unit

def backtrack(i: Instance) = {
  if (i.resume)
    for (setEnv <- i.value) {
      setEnv()
      backtrack(i.snapshot)
    }
}
\end{lstlisting}
\columnbreak
\begin{lstlisting}[caption={Direct-style ScalaCheck, cont.},label=list:backtrack-cont,language=scala,mathescape,captionpos=t]
val ints = coroutine {
  (xs: List[Int]) =>
  var env: Int = _
  val setEnvs =
    xs.map(x => () => env = x)
  yieldval(setEnvs)
  env
}

def test(t: Test) = {
  val instance = t.start()
  backtrack(instance)
}
\end{lstlisting}
\end{multicols}

In Listing \ref{list:backtrack},
we first declare two type aliases \texttt{Test} and \texttt{Instance},
which represent a test coroutine and a running test instance.
Their yield type is a list of environment setters \texttt{List[() => Unit]}.
The \texttt{backtrack} subroutine takes a running test instance, and resumes it.
If the instance yields, then the test must have called a generator,
so \texttt{backtrack} traverses the environment setters
and recursively resumes a snapshot for each of them.
Thus, each recursive call to \texttt{backtrack}
represents a node in the respective backtracking tree.

The \texttt{ints} generator in Listing \ref{list:backtrack-cont}
is a coroutine that takes a list of integers \texttt{xs} to choose from.
It starts by creating a local variable \texttt{env},
and a list of functions that set \texttt{env} (one for each integer in \texttt{xs}).
The generator then yields this list.
Each time \texttt{ints} gets resumed,
the \texttt{env} variable is set to a proper value,
so it is returned to the test that called it.

\paratitle{Continuations}
Shift-reset-style delimited continuations use the \texttt{reset} operator
to delimit program regions for the CPS-transform
\cite{Danvy:1990:AC:91556.91622}.
The \texttt{shift} operator,
which takes a function whose input is the continuation,
can be used inside these regions.
%To show equivalence of coroutines and continuations,
We sketch the implementation of \texttt{shift} and \texttt{reset}
similar to those in Scala delimited continuations
\cite{Rompf:2009:IFP:1631687.1596596}.

\begin{lstlisting}[label=list:continuations,language=scala,mathescape,captionpos=t]
type Shift = (() => Unit) => Unit
def reset(b: () ~> (Shift, Unit)): Unit = {
  def continue(i: Shift <~> Unit) =
    if (i.resume) i.value(() => continue(i.snapshot))
  continue(b.start())
}
def shift: Shift ~> (Shift, Unit) =
  coroutine { (b: Shift) => yieldval(b) }
\end{lstlisting}

The type alias \texttt{Shift} represents continuation handlers --
functions that take continuations of the current program.
The \texttt{reset} operator takes a coroutine
that can yield a \texttt{Shift} value.
It starts a new coroutine instance and resumes it.
If this instance calls \texttt{shift} with a continuation handler,
the handler is yielded back to \texttt{reset},
which creates an instance snapshot and uses it to create a continuation.
The continuation is passed to the continuation handler.
The use of \texttt{snapshot} is required,
as the continuation can be invoked multiple times.

